Mobility Data in Operations: The Facility Location Problem

The recent large scale availability of mobility data, which captures individual mobility patterns, poses novel operational problems that are exciting and challenging. Motivated by this, we introduce and study a variant of the (cost-minimization) facility location problem where each individual is endowed with two locations (hereafter, her home and work locations), and the connection cost is the minimum distance between any of her locations and its closest facility. We design a polynomial-time algorithm whose approximation ratio is at most 2.497. We complement this positive result by showing that the proposed algorithm is at least a 2.428-approximation, and there exists no polynomial-time algorithm with approximation ratio $2-\epsilon$ under UG-hardness. We further extend our results and analysis to the model where each individual is endowed with K locations. Finally, we conduct numerical experiments over both synthetic data and US census data (for NYC, greater LA, greater DC, Research Triangle) and evaluate the performance of our algorithms.

==> EC-submission/EC-macros.tex <==
\usepackage[parfill]{parskip}
% \usepackage[letterpaper, left=1in, right=1in, top=1in, bottom=1in]{geometry}


% \usepackage[boxed]{algorithm2e}

\usepackage{pgfplots}
\pgfplotsset{compat=1.18}
\usepackage{tikz}

\usetikzlibrary{patterns}

\usepackage{amsmath}
% \PassOptionsToPackage{numbers, compress}{natbib}
% \usepackage{tcolorbox}
\usepackage{xcolor}
\usepackage{bbm}
\usepackage{multicol}



\usepackage{natbib}
% \bibliographystyle{plainnat}
\bibpunct{(}{)}{;}{a}{,}{,}
 
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage[usenames,dvipsnames]{xcolor}
% \usepackage[colorlinks=true, linkcolor=blue!70!black, citecolor=blue!70!black,urlcolor=black,breaklinks=true]{hyperref}

\usepackage{hyperref}

\usepackage{comment}

\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\usepackage{mathtools, amsthm, bm}

\usepackage[frak=mma]{mathalfa}
\usepackage{soul}

\allowdisplaybreaks

\usepackage{csquotes}
\makeatletter
%Take the original environment definition and change the leftmargin to 1cm
\renewenvironment*{displayquote}
  {\begingroup\setlength{\leftmargini}{1cm}\csq@getcargs{\csq@bdquote{}{}}}
  {\csq@edquote\endgroup}
\makeatother
% \usepackage{amsthm}


% \usepackage{algorithm} 
% \usepackage{algorithmic}  
% \usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e} 

% \usepackage[lined,boxed,ruled,norelsize,algo2e,linesnumbered,noend]{algorithm2e}
\newcommand{\algcomment}[1]{\textcolor{blue!70!black}{{\texttt{\textbf{#1}}}}}
\newcommand\mycommfont[1]{\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}

\usepackage{subcaption}
\usepackage{multirow}
\usepackage{float}
\usepackage{xspace}

\usepackage{enumitem}

\usepackage{xfrac}

\usepackage{cleveref}


\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]

\usepackage{thm-restate}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}% reset theorem numbering for each chapter

% \newenvironment{numberedtheorem}[1]{%
% \renewcommand{\thetheorem}{#1}%
% \begin{theorem}}{\end{theorem}\addtocounter{theorem}{-1}}

% \newenvironment{numberedlemma}[1]{%
% \renewcommand{\thetheorem}{#1}%
% \begin{lemma}}{\end{lemma}\addtocounter{theorem}{-1}}


\newtheorem{informal}{Informal Theorem}


\theoremstyle{plain}
\newtheorem{definition}{Definition}[section] % definition numbers are dependent on theorem numbers
\newtheorem{example}[definition]{Example}
% \newtheorem{assumption}[definition]{Assumption} 
\newtheorem{remark}[definition]{Remark} 
\newtheorem{conjecture}[definition]{Conjecture} 
\newtheorem{task}[definition]{Task} 
\newtheorem{observation}[definition]{Observation}

\theoremstyle{plain}

\newenvironment{numbereddefinition}[1]{%
\renewcommand{\thedefinition}{#1}%
\begin{definition}}{\end{definition}\addtocounter{definition}{-1}}


\newtheorem{assumption}{Assumption}
% \newtheorem{assumption}[definition]{Assumption} 


\newenvironment{numberedassumption}[1]{%
\renewcommand{\thedefinition}{#1}%
\begin{assumption}}{\end{assumption}\addtocounter{definition}{-1}}

\newenvironment{myprocedure}[1][htb]
{ \renewcommand{\algorithmcfname}{Procedure} %Update algorithm name
\begin{algorithm2e}[#1]%
}{\end{algorithm2e}}



	\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
	\newcommand{\reals}{\mathbb{R}}
	\newcommand{\positivereals}{\tiny \reals_{+}}
	\newcommand*{\R}{\mathbb{R}}



\makeatletter
\newcommand{\subalign}[1]{%
  \vcenter{%
    \Let@ \restore@math@cr \default@tag
    \baselineskip\fontdimen10 \scriptfont\tw@
    \advance\baselineskip\fontdimen12 \scriptfont\tw@
    \lineskip\thr@@\fontdimen8 \scriptfont\thr@@
    \lineskiplimit\lineskip
    \ialign{\hfil$\m@th\scriptstyle##$&$\m@th\scriptstyle{}##$\hfil\crcr
      #1\crcr
    }%
  }%
}
\makeatother



\allowdisplaybreaks


% 	\DeclareMathOperator{\argmax}{argmax}
% 	\DeclareMathOperator{\argmin}{argmin}
	\DeclareMathOperator{\OPT}{\texttt{OPT}}
	\DeclareMathOperator{\MC}{\textrm{MaxCut}}
	\newcommand{\SDP}{\texttt{OPT-SDP}}
	\newcommand{\Ws}{\sum_{(i,j)\in E}w_{ij}}
	\newcommand{\OBJ}{\texttt{OBJ}}
	\newcommand{\Ycal}{\mathcal{Y}}
	\newcommand{\Ecal}{\mathcal{E}}
	\newcommand{\Zcal}{\mathcal{Z}}

	\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
	\DeclarePairedDelimiter{\card}{\lvert}{\rvert}
	\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
	\providecommand{\given}{}
	\DeclarePairedDelimiterX{\set}[1]\{\}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
	\let\Pr\relax
	\DeclarePairedDelimiterXPP{\Pr}[1]{\mathbb{P}}[]{}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
	\DeclarePairedDelimiterXPP{\Ex}[1]{\mathbb{E}}[]{}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
	\DeclarePairedDelimiter{\dotp}{\langle}{\rangle}
	\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
	\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}


	

	%%%-----------------Macros for this paper ------------------

	\newcommand{\YF}[1]{\textcolor{blue}{ (\em Yiding: \bf#1)}}



\newcommand{\durationpdf}{g}
\newcommand{\durationcdfi}{\bar{\durationdistribution}}
\newcommand{\inventorydistribution}{\mathcal H}
\newcommand{\inventorycdf}{\inventorydistribution}
\newcommand{\inventorycdfi}{{\bar{\inventorycdf}}}
\newcommand{\magicprob}{\eta}

\newcommand{\bench}[1]{\textbf{OPT}\left[#1\right]}
\newcommand{\tpre}{t'}
	\newcommand{\opt}{^{\star}}
	\newcommand{\primed}{^\dagger}
	\newcommand{\doubleprimed}{^{\ddagger}}
	\newcommand{\pprimed}{\doubleprimed}


	\newcommand{\Z}{\mathbb{Z}}
	\newcommand{\inventory}{c}
	\newcommand{\mininventory}{{\inventory_{\min}}}%{\underaccent{\bar}{\inventory}}

	\newcommand{\xit}{x_i(t)}
	\newcommand{\yit}{y_i(t)}
	\newcommand{\rit}{r_i(t)}
	\newcommand{\xitp}{x_i(t')}
	\newcommand{\fit}{f_i(t)}
	\newcommand{\fitp}{f_i(t')}
	\newcommand{\fitm}{f_i(t^-)}
	\newcommand{\yitm}{y_i(t^-)}
	\newcommand{\fitpm}{f_i((t')^-)}
	\newcommand{\yitp}{y_i(t')}
	\newcommand{\yitpm}{y_i((t')^-)}
	\newcommand{\ritp}{r_i(t')}
	\newcommand{\yst}{y_S(t)}
	\newcommand{\ystp}{y_S(t')}
	\newcommand{\feasibleset}{\mathcal F}
	\newcommand{\lit}{\lambda_i(t)}
	\newcommand{\litp}{\lambda_i(t')}
	\newcommand{\tht}{\theta(t)}
% 	\newcommand{\thit}{\theta_i(t)}
	\newcommand{\thitp}{\theta_i(t')}
	\newcommand{\lt}{\lambda(t)}
	\newcommand{\totaltime}{T}
	\newcommand{\reward}{r}
	\newcommand{\rewards}{\mathbf \reward}
	\newcommand{\choice}{\phi}
	\newcommand{\pen}{\Psi}
	%\newcommand{\choices}{\boldsymbol{\choice}}
	\newcommand{\durationdistribution}{G}
	\newcommand{\durationdistributions}{{\mathbf{\durationdistribution}}}
	\newcommand{\assortment}{S}
	\newcommand{\assortmentspace}{\mathcal{S}}
	\newcommand{\duration}{d}
	\newcommand{\typedistribution}{F}

	\newcommand{\inventorydual}{\theta}
	\newcommand{\inventoryduali}{\inventorydual_{i, k,t}}
	\newcommand{\probdual}{\lambda}
	\newcommand{\probduali}{\probdual_{t}}
\newcommand{\probdualtype}{\lambda_{t,\type_t}}
	\newcommand{\typesequence}{\{\type_t\}_{t = 1}^\totaltime}
	\newcommand{\inversetypesequence}{\{\type_t\}_{t = 1}^\totaltime}
	\newcommand{\typedistributionsequence}{\{\typedistribution_t\}_{t = 1}^\totaltime}

\newcommand{\EAR}{\text{EAR}}
\newcommand{\EARPrime}{\text{EAR}\primed}
% 	\newcommand{\EAR}[2][]{\text{\bf Expected-LP}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
% 	\newcommand{\EARPrime}[2][]{\text{\bf Expected-LP}^{\dagger}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
	\newcommand{\algo}{\mathcal{A}}

    \newcommand{\Profit}[2][]{\text{\bf Profit}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
    \newcommand{\Cost}[2][]{\text{\bf COST}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}

	\newcommand{\Rev}[2][]{\text{\bf Rev}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
	\newcommand{\MargRev}[1]{\mathbf{MargRev}[#1]}

	
    \newcommand{\Obj}[2][]{\text{\bf OBJ}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
    
    \newcommand{\SFRP}[1]{\text{\hyperref[eq:strongly factor-revealing quadratic program]{$\mathcal{P}_{\texttt{SFR}}(#1)$}}}
    \newcommand{\WFRP}[1]{\text{\hyperref[eq:weakly factor-revealing program]{$\mathcal{P}_{\texttt{FR}}(#1)$}}}

    \newcommand{\SFRPMFLP}[1]{\text{\hyperref[eq:strongly factor-revealing program MFLP]{$\mathcal{P}_{\texttt{SFR-MFLP}}(#1)$}}}
    \newcommand{\WFRPMFLP}[1]{\text{\hyperref[eq:weakly factor-revealing program MFLP]{$\mathcal{P}_{\texttt{FR-MFLP}}(#1)$}}}



	\newcommand{\alloc}{x}
	\newcommand{\curalloc}{\alloc_{\indexnew, t}}
	\newcommand{\curalloctype}{\alloc_{\assortment, t, \type_t}}
	\newcommand{\curalloctypeopt}{\alloc^*_{\assortment, t, \type_t}}
	\newcommand{\curexantetype}{X_{\assortment, t, \type_t}}
	\newcommand{\curchoice}{\choice_{t}(\assortment, i)}
	\newcommand{\curreward}{\reward_i^{\type_t}}
	\newcommand{\price}{P}
	\newcommand{\curprice}{\price_{i, t}^{\type_t}}
	\newcommand{\curdurationdistribution}{\durationdistribution_i^{\type_t}}
	\newcommand{\curinventorya}{I_{i, t}}
	\newcommand{\curinventoryb}{I_{i, t}}
	\newcommand{\curpseudoinventory}{{\tilde{I}_{i, t}}}
	\newcommand{\curpenA}{\pen\left(\curinventorya/\inventory_i\right)}
	\newcommand{\curpenB}{\pen\left(\curinventoryb/\inventory_i\right)}
	\newcommand{\curpena}{\pen_i(t^-)}
	\newcommand{\curpenb}{\pen_i(t)}
	\newcommand{\previous}{^\prime}
	\newcommand{\prealloc}{\alloc_{\indexnew, \tpre}}
	\newcommand{\prechoice}{\choice_{\tpre}(\assortment, i)}
	%\newcommand{\curchoicetype}{\choice^{\type_t}(\assortment, i)}


	% accents for using with newagentvar
	% (must take a single argument)
	\newcommand{\ironed}{\bar}
	\newcommand{\constrained}{\hat}
	\newcommand{\optconstrained}{\composed{\optimized}{\constrained}}
	\newcommand{\optimized}[1]{#1\opt}
	\newcommand{\differentiated}[1]{#1'}
	\newcommand{\fortype}{\tilde}
	\newcommand{\tagged}[2]{{#2}^{#1}}


	\newcommand{\starred}[1]{#1^\star}
	\newcommand{\primedarg}[1]{#1\primed}
	\newcommand{\noaccents}[1]{#1}
	% compose accents on the fly
	\newcommand{\composed}[3]{#1{#2{#3}}}
	\newcommand{\newagentvar}[3][\noaccents]{%
		\expandafter\newcommand\expandafter{\csname #2\endcsname}{#1{#3}}%
		\expandafter\newcommand\expandafter{\csname #2s\endcsname}{#1{\boldsymbol{#3}}}%
		\expandafter\newcommand\expandafter{\csname #2smi\endcsname}[1][i]{#1{\boldsymbol{#3}}_{-##1}}%
		\expandafter\newcommand\expandafter{\csname #2i\endcsname}[1][i]{#1{#3}\agind[##1]}%
		\expandafter\newcommand\expandafter{\csname #2ith\endcsname}[1][i]{#1{#3}_{(##1)}}%
	}
	\newagentvar{typespace}{{\cal Z}}
	\newagentvar{typesubspace}{S}
	\newcommand{\extypes}[1][\exquant]{\typesubspace^{#1}\!}
	\newagentvar{type}{z}
	\newagentvar{othertype}{s}
	\newagentvar{val}{v}
	\newagentvar{hval}{\bar \val}
	\newagentvar{hbudget}{\bar \wealth}
	\newagentvar{budget}{B}
	\newagentvar{lbudget}{\underaccent{\bar}{ \wealth}}
	\newagentvar{lowestval}{0}
	\newagentvar{cumval}{V}
	\newagentvar{cumprice}{P}
	\newagentvar{welcurve}{W}
	\newagentvar{revcurve}{R}
	\newagentvar{outcome}{w}
	\newagentvar{outcomespace}{{\cal W}}
	\newcommand{\nulloutcome}{\emptyset}
	


	
	\newcommand{\distance}{d}
\newcommand{\flow}{\tau}
\newcommand{\flowi}{\flow_{ij}}
\newcommand{\flows}{\{\flowi\}}
\newcommand{\pop}{N}
\newcommand{\popi}{\pop_i}
\newcommand{\popj}{\pop_j}
\newcommand{\pops}{\{\popi\}}
\newcommand{\emp}{E}
\newcommand{\empi}{\emp_i}
\newcommand{\empj}{\emp_j}
\newcommand{\emps}{\{\empi\}}
\newcommand{\stores}{\SOL}
\newcommand{\home}{h}
\newcommand{\workplace}{w}
% \newcommand{\distance}{d}
\newcommand{\opencost}{f}
\newcommand{\opencosti}{\opencost_i}
\newcommand{\opencosts}{\{\opencosti\}}
\newcommand{\serveradius}{R}

\newcommand{\servingpopulation}{\texttt{Service}}
\newcommand{\servingpopulationand}{\servingpopulation_\land}
\newcommand{\servingpopulationor}{\servingpopulation_\lor}

\newcommand{\data}{D}
\newcommand{\mobilitydata}{\data_{M}}
\newcommand{\partialdata}{\data_{L}}
\newcommand{\datas}{\mathcal{\data}}
\newcommand{\mobilitydatas}{\datas_{M}}
\newcommand{\allmobilitydatas}{\bar\datas_{M}}


\newcommand{\population}{\emp}
\newcommand{\employee}{\pop}
% \newcommand{\flow}{\tau}
\newcommand{\flowbf}{\boldsymbol{\flow}}
% \newcommand{\flowi}{\flow_{ij}}

\newcommand{\instance}{I}
\newcommand{\instances}{\mathcal{\instance}}
\newcommand{\observeinstance}{D}
\newcommand{\SOL}{\texttt{SOL}}
\renewcommand{\OPT}{\texttt{OPT}}
\newcommand{\voi}{\Gamma}
\newcommand{\voior}{\voi_\lor}
\newcommand{\voiand}{\voi_\land}



% \newcommand{\OPT}{\texttt{OPT}}
\newcommand{\approxratio}{\Gamma}
\newcommand{\SFRapproxratio}{\approxratio_{\texttt{SFR}}(\discountfactor)}
\newcommand{\WFRapproxratio}{\approxratio_{\texttt{FR}}(\discountfactor)}

\newcommand{\SFRMFLPapproxratio}{\approxratio_{\texttt{SFR-MFLP}}}
\newcommand{\WFRMFLPapproxratio}{\approxratio_{\texttt{FR-MFLP}}}


\newcommand{\connectioncost}{c}
\newcommand{\sol}{\Psi}

\newcommand{\distanceHat}{{\distance}}
\newcommand{\costHat}{{\opencost}}
\newcommand{\distanceHatStar}{{\connectioncost}}
\newcommand{\muHat}{{\alpha}}
\newcommand{\dualapproxHat}{\hat{\dualapprox}}


\DeclareRobustCommand{\rchi}{{\mathpalette\irchi\relax}}
\newcommand{\irchi}[2]{\raisebox{\depth}{$#1\chi$}}
\newcommand{\permuspace}{\mathbb{\chi}}
\newcommand{\permu}{\chi}

\newcommand{\greedyapprox}{\text{3.103}}
\newcommand{\greedyapproxMFLP}{\text{1.819}}




\newcommand{\TWOLFLP}{2-LFLP}
\newcommand{\edge}{e}
\newcommand{\edgehome}{\edge_h}
\newcommand{\edgework}{\edge_w}
\newcommand{\flowe}{\flow_\edge}
\newcommand{\ALG}{\texttt{ALG}}

\newcommand{\plus}[1]{{\left( #1 \right)^+}}

\newcommand{\dual}{\mu}
\newcommand{\currentset}{U}
\newcommand{\starinstance}{S}
\newcommand{\pendingset}{W}
\newcommand{\N}{\mathbb{N}}
\newcommand{\edgeindex}{\eta}

\newcommand{\frcone}{\texttt{FRC-1}}
\newcommand{\frctwo}{\texttt{FRC-2}}
\newcommand{\frcthree}{\texttt{FRC-3}}
\newcommand{\frcfour}{\texttt{FRC-4}}
\newcommand{\frcfive}{\texttt{FRC-5}}
\newcommand{\frcsix}{\texttt{FRC-6}}

\newcommand{\greedycounter}{\alpha}
\newcommand{\firstchanceset}{U}
\newcommand{\secondchanceset}{U^{(2)}}
\newcommand{\secondchancesetwork}{\secondchanceset_w}
\newcommand{\secondchancesethome}{\secondchanceset_h}
\newcommand{\connectmapping}{\psi}
\newcommand{\Edge}{E}
\newcommand{\config}{\sigma}
% \newcommand{\config}{\mathfrak{H}}
\newcommand{\confige}{{\config(\edge)}}
\newcommand{\configi}{\confige}
\newcommand{\timeindex}{t}
\newcommand{\cost}{c}
\newcommand{\coststar}{\cost(\starinstance)}
\newcommand{\allocstar}{\alloc(\starinstance)}
\newcommand{\duale}{\dual(\edge)}
\newcommand{\starspace}{\mathcal{S}}
\newcommand{\singlecountedgeset}{\Edge^{(1)}}
\newcommand{\doublecountedgeset}{\Edge^{(2)}}
\newcommand{\singlecountedgesetHat}{\hat{\singlecountedgeset}}
\newcommand{\doublecountedgesetHat}{\hat{\doublecountedgeset}}
\newcommand{\mHat}{{m}}
\newcommand{\nHat}{{n}}
\newcommand{\qHat}{{q}}
\newcommand{\dualapprox}{\Gamma}



\newcommand{\qHatBf}{\mathbf{q}}
\newcommand{\muHatBf}{\boldsymbol{\muHat}}
\newcommand{\distanceHatBf}{{\mathbf{\distance}}}
\newcommand{\distanceHatStarBf}{{\mathbf{\connectioncost}}}
\newcommand{\zerobf}{\mathbf{0}}

\newcommand{\naturals}{\mathbb{N}}


\newcommand{\yHat}{\hat{y}}



\newcommand{\discountfactor}{\gamma}
\newcommand{\nullsymbol}{\bot}
\newcommand{\hwset}{\{h,w\}}

\newcommand{\normalizefactor}{K}
\newcommand{\SFRCmonotonicity}{\texttt{(SFR.i)}}
\newcommand{\SFRCtriangleineq}{\texttt{(SFR.ii)}}
\newcommand{\SFRCcontribution}{\texttt{(SFR.iii)}}
\newcommand{\SFRCcontributionstronger}{\texttt{(SFR.iii.0)}}
\newcommand{\SFRCdistance}{\texttt{(SFR.iv)}}
\newcommand{\SFRCconnectcost}{\texttt{(SFR.v)}}
\newcommand{\SFRCtotalcost}{\texttt{(SFR.vi)}}
\newcommand{\SFRCdensity}{\texttt{(SFR.vii)}}

\newcommand{\WFRCtriangleineq}{\texttt{(FR.i)}}
\newcommand{\WFRCcontribution}{\texttt{(FR.ii)}}
\newcommand{\WFRCconnectcost}{\texttt{(FR.iii)}}
\newcommand{\WFRCtotalcost}{\texttt{(FR.iv)}}

\newcommand{\EdgeTilde}{\tilde{\Edge}}
\newcommand{\edgetoellmapping}{\kappa}
\newcommand{\edgetoellmappingconfig}{\edgetoellmapping_{\config}}

\newcommand{\empattract}{\rho}
\newcommand{\flowconstructionfactor}{\iota}
\newcommand{\costconstructionfactor}{\bar{\opencost}}
\newcommand{\zhvi}{z}
\newcommand{\CFAlg}{\texttt{2-GR}}
\newcommand{\CFAlgP}{\texttt{2-GRP}}
\newcommand{\GDH}{\texttt{GR-H}}
\newcommand{\GDW}{\texttt{GR-W}}

\newcommand{\candidatecosttext}{candidate cost}



\newcommand{\KLFLP}{$K$-LFLP}
\newcommand{\RelaxSFRapproxratio}{\approxratio_{\texttt{SFR-Relax}}}
\newcommand{\RelaxSFRP}[1]{\text{\hyperref[eq:relax strongly factor-revealing quadratic program]{$\mathcal{P}_{\texttt{SFR-Relax}}(#1)$}}}

\newcommand{\LBLP}[1]{\text{\hyperref[eq:lower bound LP]{$\mathcal{P}_{\texttt{LB}}(#1)$}}}


==> Notes/LP-relxation.tex <==
% \section{LP Relaxation}

==> Notes/conjunctive-model.tex <==
\section{Conjunctive Model}
\label{sec:conjunctive}

==> Notes/disjunctive-model.tex <==
\section{Disjunctive Model}
\label{sec:disjunctive}

\newcommand{\WH}{Work Heuristic}
\newcommand{\OPTP}{Optimal Policy}
\newcommand{\wc}{\gamma}
\newcommand{\downtownoverlapcnt}{\zeta}
\newcommand{\bpb}{\rho}
\newcommand{\bpbd}{\bpb_d}
\newcommand{\bpbs}{\bpb_s}
\newcommand{\locationsubset}{T}
\newcommand{\downtown}{\locationsubset_d}
\newcommand{\suburb}{\locationsubset_s}
\newcommand{\rev}{R}
\newcommand{\oneed}{^{(1)}}
\newcommand{\twoed}{^{(2)}}
\newcommand{\threeed}{^{(3)}}
\newcommand{\revd}{\rev_d}
\newcommand{\revdone}{\revd\oneed}
\newcommand{\revdtwo}{\revd\twoed}
\newcommand{\revone}{\rev\oneed}
\newcommand{\revtwo}{\rev\twoed}
\newcommand{\revthree}{\rev\threeed}
\newcommand{\revs}{\rev_s}
\newcommand{\revsone}{\revs\oneed}
\newcommand{\revstwo}{\revs\twoed}
\newcommand{\mapping}{\sigma}
\newcommand{\downtowntilde}{\tilde\downtown}

\subsection{Data-driven Simulation in 
Disjunctive Model}
\label{sec:empirical result or}

\subsection{Approximation Guarantee of 
Work Heuristic}
\label{sec:theoretical result or}
In this subsection, we establish two 
theoretical results on the approximation guarantee
of \WH, which provides qualitative insights 
on the performance of \WH\ observed 
in our data-driven simulation (\Cref{sec:empirical result or}).

As we discussed in \Cref{sec:empirical result or},
for cities (e.g., NYC, DC, Bay area) where 
\WH\ achieves a near-optimal profit as \OPTP,
employments are concentrated, i.e., 
there exists a subset of locations 
(denoted as \emph{downtown})
which contains majority of the employments,
and their bang-per-buck are 
strictly higher than 
the bang-per-buck of the remaining locations
(denoted as \emph{suburb}). 
Here we formalize this intuition by introducing
the following parameterized assumption on 
a partial data $\partialdata$,
and \Cref{thm:wh or}.
\begin{assumption}
Partial data $\partialdata = ([n], \distance, \pops, \emps,  \opencosts, \serveradius)$ 
is \emph{$(\wc, \downtownoverlapcnt, \bpbd, \bpbs)$-employments concentrated}
if there exists a partition $(\downtown, \suburb)$
of all locations $[n]$ such that
\begin{itemize}
    \item opening all locations in downtown $\downtown$
    serves $\wc$-fraction of total employees,
    i.e.,
    \begin{align*}
        \sum_{i\in[n]}
        \empi \cdot 
        \indicator{\exists
        k\in\downtown:
        \distance(i,k) \leq 
        \serveradius}
        = \wc \cdot 
        \sum_{i\in[n]}
        \empi
    \end{align*}
    \item for every location $i\in \downtown$, 
    the number of other locations in downtown which overlap\footnote{We say two locations overlap if their distance is less or equal to $2\serveradius$.}
    with location $i$ is at most $\downtownoverlapcnt$, i.e., 
    \begin{align*}
        \left|
        \{j\in\downtown\backslash\{i\}:\distance(i,j) \leq 2\serveradius\}
        \right| \leq \downtownoverlapcnt
    \end{align*}
    \item for every location $i\in\downtown$,
    \begin{align*}
        \sum_{j\in[n]}\empj \cdot 
        \indicator{
        \distance(i,j) \leq 
        \serveradius}
        \geq 
        \bpbd \cdot \opencost_i
    \end{align*}
    \item for every location $i\in\suburb$,
    \begin{align*}
        \sum_{j\in[n]}(\popj+ \empj) \cdot 
        \indicator{
        \distance(i,j) \leq 
        \serveradius}
        \cdot \indicator{
        \forall k\in \downtown:\distance(j,k) > \serveradius
        }
        \leq 
        \bpbs \cdot \opencost_i
    \end{align*}
\end{itemize}
\end{assumption}

\begin{lemma}
\label{lem:open downtown cost}
In the disjunctive model,
for partial data $\partialdata$
that is $(\wc, \downtownoverlapcnt, \bpbd, \bpbs)$-employments concentrated,
the cost of opening stores in all locations in downtown $\downtown$
satisfies 
$$\sum_{i\in\downtown}\opencost_i\leq 
\frac{\downtownoverlapcnt + 1}{\bpbd}\cdot \wc \cdot 
        \sum_{i\in[n]}
        \empi$$
\end{lemma}
\proof{\textsl{Proof.}}
Without loss of generality, we assume $\downtown = [k]$
and $c_i$ is decreasing in $i\in[k]$.
To show the statement, we first construct
subset $\downtowntilde\subseteq[k]$
and 
mapping $\mapping:[k]\rightarrow[k]$ as follows:
(i) initialize $\downtowntilde \gets \emptyset$;
(ii) for each location $i\in[k]$, 
if location $i$ does not overlap with any location $j\in\downtowntilde$
(i.e., $\forall j\in\downtowntilde$ $\distance(i, j) > 2\serveradius$),
add location $i$ into $\downtowntilde$
(i.e., $\downtowntilde\gets \downtowntilde\cup\{i\}$)
and set $\mapping(i) \gets i$;
otherwise
set $\mapping(i) \gets \min\{j\in\downtowntilde:\distance(i,j)\leq 2\serveradius\}$.

By construction, for each location $i$,
$\mapping(i) \leq i$ for each location $i\in[k]$,
and $|\{j\in[k]:\mapping(j) = i\}|\leq \downtownoverlapcnt + 1$. 
Thus,
\begin{align*}
        \sum_{i\in[k]}\opencost_i
        &\leq
        \sum_{i\in[k]}\opencost_{\mapping(i)}
        \leq 
        \sum_{i\in\downtowntilde} (\downtownoverlapcnt + 1)\cdot \opencost_i
        \\&
        \overset{}{\leq}
        (\downtownoverlapcnt + 1)
        \sum_{i\in\downtowntilde} 
        \frac{1}{\bpbd}\sum_{j\in[n]}\empj \cdot 
        \indicator{
        \distance(i,j) \leq 
        \serveradius}
        \\&
        \overset{(a)}{\leq}
        \frac{\downtownoverlapcnt + 1}{\bpbd}
        \sum_{j\in[n]}
        \empi \cdot 
        \indicator{\exists
        i\in[k]:
        \distance(i,j) \leq 
        \serveradius}
        =
        \frac{\downtownoverlapcnt + 1}{\bpbd}
        \cdot 
        \wc \cdot 
        \sum_{i\in[n]}
        \empi
\end{align*}
where inequality~(a) uses the fact that location $i$ and $j$ do not overlap
for any $i, j\in \downtowntilde$.
\hfill\halmos
\endproof

\begin{theorem}
\label{thm:wh or}
In the disjunctive model,
for partial data $\partialdata$
that is $(\wc, \downtownoverlapcnt, \bpbd, \bpbs)$-employments concentrated,
its value of mobility data $\voi(\partialdata)$ is at most 
\begin{align*}
\voi(\partialdata)
     \leq 
    \frac{
    \wc +  \left(1-\frac{1}{\bpbs}\right)^+
        (1-\wc)
    }{
    \left(1-\frac{\downtownoverlapcnt + 1}{\bpbd}\right)^+\wc 
    }
\end{align*}
\end{theorem}
\proof{\textsl{Proof.}}
For our analysis, we introduce the following 
partition which divides all individuals into three groups:
(1) individuals who can be served due to their employment 
by opening stores in 
all locations in downtown $\downtown$;
(2) individuals who can be served due to their residency 
by opening stores in 
all locations in downtown $\downtown$ (after excluding individuals from 
group (1));
(3) all remaining individuals.

Fix an arbitrary optimum solution $\OPT$
when mobility data $\mobilitydata$ is available.
Its revenue (i.e., individual served by $\OPT$) can 
be decomposed into $\revone$, $\revtwo$ and $\revthree$,
which corresponds to individuals served in aforementioned group (1), (2), (3)
respectively. 
% $\revd$ is the number of individuals 
% who are served by stores in solution $\OPT$ in
% downtown $\downtown$ (i.e., $\OPT\cap\downtown$);
% and $\revs$
% is the number of individuals
% who are served by stores in solution $\OPT$ in
% suburb $\suburb$ (i.e., $\OPT\cap\suburb$),
% after excluding individuals from $\revd$.
% We can further decompose $\revd$
% into $\revdone$ and $\revdtwo$
% where $\revdone$
% considers individuals who can be served by opening stores 
% in all locations in downtown $\downtown$
% due to their employments,
% and $\revdtwo$ considers the remaining individuals from $\revd$
% after excluding $\revdone$.
% Similarly, we can further decompose $\revs$
% into $\revsone$ and $\revstwo$
% where $\revsone$
% considers individuals who cannot be served by opening stores 
% in all locations in downtown $\downtown$,
% and $\revstwo$ considers the remaining individuals from $\revs$
% after excluding $\revsone$.
The profit from the optimum solution $\OPT$
can thus be upperbounded by 
\begin{align*}
    \Profit{\OPT} 
    \leq 
    \revone + \revtwo + \revthree - \frac{1}{\bpbs}\revthree
\end{align*}
where we lowerbound the cost for serving individuals in
$\revone$ and $\revtwo$ by 0,
and the cost for serving individuals in $\revthree$ 
by $\frac{1}{\bpbs}\revthree$.

When only partial data $\partialdata$ is available, 
consider the solution $\SOL$ which opens stores in all locations in downtown $\downtown$.
Invoking \Cref{lem:open downtown cost},
we can lowerbound its profit by 
\begin{align*}
    \Profit{\SOL} 
    \geq 
        \wc \cdot \sum_{i\in[n]}
        \empi 
        + \revtwo
        - 
        \frac{\downtownoverlapcnt + 1}{\bpbd}\cdot 
        \wc \cdot \sum_{i\in[n]}
        \empi 
\end{align*}
Thus, the approximation between $\SOL$ and $\OPT$ is at most 
\begin{align*}
    \frac{\Profit{\OPT}}{\Profit{\SOL}}
    &\leq 
    \frac{
    \revone + \revtwo + \revthree - \frac{1}{\bpbs}\revthree
    }{
    \wc \cdot \sum_{i\in[n]}
        \empi 
        + \revtwo
        - 
        \frac{\downtownoverlapcnt + 1}{\bpbd}\cdot 
        \wc \cdot \sum_{i\in[n]}
        \empi 
    }
    \leq 
    \frac{
    \revone + \revthree - \frac{1}{\bpbs}\revthree
    }{
    \wc \cdot \sum_{i\in[n]}
        \empi 
        - 
        \frac{\downtownoverlapcnt + 1}{\bpbd}\cdot 
        \wc \cdot \sum_{i\in[n]}
        \empi 
    }
\end{align*}
Here we also know that 
\begin{align*}
    \revone  &\leq \wc \cdot \sum_{i\in[n]} \empi
        % \\
        \quad 
        \mbox{and}
        \quad
     \revtwo + \revthree 
    %  &
     \leq (1 - \wc) \cdot \sum_{i\in[n]} \empi
\end{align*}
Thus, the value of mobility data is at most 
\begin{align*}
    \voi(\partialdata) 
    &\leq 
    \frac{
    \wc \cdot \sum_{i\in[n]}
        \empi 
        +
        \left(1-\frac{1}{\bpbs}\right)^+
        (1-\wc) \cdot \sum_{i\in[n]}
        \empi 
    }{
    \wc \cdot \sum_{i\in[n]}
        \empi 
        - 
        \frac{\downtownoverlapcnt + 1}{\bpbd}\cdot 
        \wc \cdot \sum_{i\in[n]}
        \empi 
    }
    % \\
    % &
    =
    \frac{
    \wc +  \left(1-\frac{1}{\bpbs}\right)^+
        (1-\wc)
    }{
    \left(1-\frac{\downtownoverlapcnt + 1}{\bpbd}\right)\wc 
    }
\end{align*}
We conclude the proof by also considering the trivial solution that opens no store 
if $\left(1-\frac{\downtownoverlapcnt + 1}{\bpbd}\right) < 0$ 
when only partial data $\partialdata$ is available.
\hfill\halmos
\endproof


\begin{theorem}
\label{thm:wh or v2}
In the disjunctive model,
for any partial data $\partialdata$
and any solution $\SOL\subseteq[n]$, we have 
\begin{align*}
    \max_{\mobilitydata}
    \frac
    {
    \Profit[(\partialdata,\mobilitydata)]{\OPT(\partialdata,\mobilitydata)}}
    {\Profit[(\partialdata,\mobilitydata)]{\SOL}}
    \leq 
    \frac{A}{B}
\end{align*}
where $A$ is the optimal value of 
\begin{align*}
    \begin{array}{lll}
    \max\limits_{\mathbf x,\mathbf y,\mathbf z }~
    &
    \displaystyle\sum\nolimits_{i\in[n]} z_i -
    \sum\nolimits_{i\in[n]} \opencost_i x_i 
    ~&
    \text{s.t.} 
    \vspace{1mm}
    \\
    &
    y_i \leq \displaystyle\sum\nolimits_{j\in[n]}
    x_j \cdot \indicator{\distance(i, j)\leq \serveradius}
    &
    i\in[n]
    \vspace{1mm}
    \\
    &
    z_i \leq 
    y_i \cdot \left(
    \emp_i
    +
    \pop_i\cdot \indicator{\forall j\in\SOL:
    \distance(i,j) > \serveradius}
    \right)
    ~&
    i\in[n]
    \vspace{1mm}
    \\
    &
    \displaystyle\sum\nolimits_{i\in[n]}z_i \leq 
    \displaystyle\sum\nolimits_{i\in[n]}\empi
    &
    \vspace{1mm}
    \\
    &
    x_i \in\{0, 1\},~ y_i \in\{0, 1\},
    ~z_i\in\reals_+
    &
    i\in[n]
    \end{array}
\end{align*}
and 
\begin{align*}
    B = \displaystyle\sum\nolimits_{i\in[n]} \empi \cdot 
    \indicator{\exists j \in \SOL: \distance(i, j) \leq \serveradius}
    -
    \displaystyle\sum\nolimits_{i\in\SOL}\opencost_i
\end{align*}
\end{theorem}

==> Notes/facility-location-greedy.tex <==
\section{Greedy}
In this section, we revisit the greedy algorithm (\Cref{alg:greedy})
introduced
in \citet{JMMSV-02},
where authors show a 1.861-approximation of 
\Cref{alg:greedy} for metric facility location problem.
Since the connection cost in our model is not a 
metric, in \Cref{claim:log(n) bound} we show that 
\Cref{alg:greedy} is a $\Omega(\log(n))$-approximation 
in our model. 
On the other side, we show a modified version
of the greedy algorithm (\Cref{alg:greedy modified})
is a $3.722$-approximation.

\newcommand{\plus}[1]{{\left( #1 \right)^+}}

\newcommand{\dual}{\alpha}
\newcommand{\currentset}{U}
\newcommand{\starinstance}{S}
\newcommand{\pendingset}{W}
\newcommand{\N}{\mathbb{N}}
\newcommand{\permu}{\sigma}


We use $\plus{x}$
to denote $\max\{x, 0\}$.

\begin{algorithm2e}[H]
 	\caption{GREEDY \citep{JMMSV-02}}
 	\label{alg:greedy}
 	\vspace{2mm}
 	
 	Initialize $\dual(j) \gets 0$ for each individual $j\in[n]$
 	
 	\vspace{1mm}
 	
 	Initialize $\currentset \gets [n]$
 	
 	\While{$U \not= \emptyset$}{ 
 	    \vspace{1mm}
 	    
 	    Continuously increase $\dual(j)$
 	    with the same rate 
 	    for all individuals $j\in \currentset$
 	    
 	    \While{there exists an unopened store $i$ s.t.\
 	    $\sum_{j\in \currentset} 
 	    \plus{\dual(j) - \connectioncost(i, j)} = \opencost(i)$
 	    }{
 	    \vspace{1mm}
 	    
 	    Open store $i$
 	    
 	    \vspace{1mm}
 	    
 	    \For{each individual $j\in \currentset$}{
 	    \vspace{1mm}
 	    \If{$\dual(j) - \connectioncost(i, j)\geq 0$}{
 	    \vspace{1mm}
 	    
 	    Connect individual $j$ with store $i$
 	    
 	    \vspace{1mm}
 	    Remove $j$ from $\currentset$, i.e., 
 	    $\currentset \gets \currentset \backslash \{j\}$
 	  %  \vspace{1mm}
 	    }
 	    }
 	    }
 	    
 	    \While{there exists an individual $j\in \currentset$ 
 	    s.t.\ $\dual(j) = \connectioncost(i, j)$ 
 	    for some opened store $i$
 	    }
 	    {
 	    \vspace{1mm}
 	    
 	    Connect individual $j$ with store $i$
 	    and remove $j$ from $\currentset$ 
 	    
 	  %  \vspace{1mm}
 	    }
 	    
 	    \vspace{1mm}
 	}
\end{algorithm2e}

\begin{theorem}[\citealp{JMMSV-02}]
In metric facility location problem,
\Cref{alg:greedy} is a $1.861$-approximation.
\end{theorem}

\begin{claim}
\label{claim:log(n) bound}
In home-workplace facility location problem,
\Cref{alg:greedy} is a $\Omega(\log(n))$-approximation.
\end{claim}
\begin{proof}{\textsl{Proof.}}
Consider the following instance of home-workplace facility 
location problem.
There are $n$ individuals and $n + 1$ possible locations for 
stores.

All individual have the same home location
which is also the location of store $n + 1$.
The workplace of each individual $j\in [n]$ 
is also the location of store $j$.
The distance between any two stores is at least $1+\epsilon$
where $\epsilon > 0$ is a sufficiently small constant.
Note that in this instance, for each individual $j\in[n]$,
$$\connectioncost(i, j) \geq (1 + \epsilon)\cdot \indicator{i\not= j}
\;\;\mbox{for every $i\in[n]$; and }
\connectioncost(n + 1, j) = 0
$$

The opening cost $\opencost(i) = \frac{1}{n - i + 1} - \epsilon$
for each store $i \in [n]$;
and $\opencost(n + 1) = 1$.

The optimal solution is opening store $n + 1$ (with total cost 1);
while \Cref{alg:greedy}
opens the first $n$ stores (with total cost $\sum_{i\in [n]}(\frac{1}{i}-\epsilon) = 
\Omega(\log(n))$.
 \ 
\end{proof}

\subsection{Modified GREEDY}
The main idea behind the modified greedy algorithm 
(\Cref{alg:greedy modified})
is that once we remove an individual $j$ from $\currentset$
(suppose we connect home $\home(j)$ to some store $i$),
we will leave $j$ a chance to connect her workplace 
$\workplace(j)$ to some store later.
See \Cref{alg:greedy modified} for a formal description.

\begin{theorem}
\label{thm:greedy modified}
In home-workplace facility location problem, 
\Cref{alg:greedy modified}
is a 3.722-approximation.
\end{theorem}

\begin{algorithm2e}[H]
 	\caption{Modified GREEDY}
 	\label{alg:greedy modified}
 	\vspace{2mm}
 	
 	Initialize $\dual(j) \gets 0$ for each individual $j\in[n]$
 	
 	\vspace{1mm}
 	
 	Initialize $\currentset \gets [n]$
 	
 	\vspace{1mm}
 	
 	Initialize $\pendingset \gets \emptyset$
 	
 	\While{$U \not= \emptyset$}{ 
 	    \vspace{1mm}
 	    
 	    Continuously increase $\dual(j)$
 	    with the same rate 
 	    for all individuals $j\in \currentset$
 	    
 	    \While{there exists an unopened store $i$ s.t.\
 	    $\sum_{j\in \currentset} 
 	    \plus{\dual(j) - \connectioncost(i, j)}
 	    +
 	    \sum_{\ell \in \pendingset}
 	    \plus{\alpha(\ell) - \distance(i,\ell)}
 	    = \opencost(i)$
 	    }{
 	    
 	    \vspace{1mm}
 	    
 	    \tcc{ we abuse the notation and define $\dual(\home(j)) = 
\dual(\workplace(j)) \triangleq \dual(j)$
for every individual $j\in[n]$}
 	    
 	    \vspace{1mm}
 	    
 	    Open store $i$
 	    
 	    \vspace{1mm}
 	    
 	    \For{each location $\ell\in \pendingset$}{
 	    \vspace{1mm}
 	    \If{$\dual(\ell) - \distance(i, \ell)\geq 0$}{
 	    
 	    \vspace{1mm}
 	    
 	    Connect location $\ell$ with store $i$
 	    
 	    \vspace{1mm}
 	    Remove $\ell$ from $\pendingset$, i.e., 
 	    $\pendingset \gets \pendingset \backslash \{\ell\}$
 	    }
 	    }
 	    
 	    \vspace{1mm}
 	    
 	    \For{each individual $j\in \currentset$}{
 	    \vspace{1mm}
 	    \If{$\dual(j) - \connectioncost(i, j)\geq 0$}{
 	    
 	    \vspace{1mm}
 	    \tcc{without loss of generality, 
 	    assume $\distance(i, \home(j)) \leq 
 	    \distance(i, \workplace(j))$}
 	    
 	    \vspace{1mm}
 	    
 	    Connect location $\home(j)$ with store $i$
 	    
 	    \vspace{1mm}
 	    Remove $j$ from $\currentset$, i.e., 
 	    $\currentset \gets \currentset \backslash \{j\}$
 	    \vspace{1mm}
 	    
 	    Add $\workplace(j)$ into $\pendingset$, i.e.,
 	    $\pendingset\gets \pendingset\cup\{\workplace(j)\}$
 	    }
 	    }
 	    }
 	    
 	    \While{there exists a location $\ell\in \pendingset$ 
 	    s.t.\ $\dual(\ell) = \distance(i, \ell)$ 
 	    for some opened store $i$
 	    }
 	    {
 	    \vspace{1mm}
 	    
 	    Connect location $\ell$ with store $i$
 	    and remove $\ell$ from $\pendingset$ 
 	    
 	  %  \vspace{1mm}
 	    }
 	    
 	    \While{there exists an individual $j\in \currentset$ 
 	    s.t.\ $\dual(j) = \connectioncost(i, j)$ 
 	    for some opened store $i$
 	    }
 	    {
 	    
 	    \vspace{1mm}
 	    \tcc{without loss of generality, 
 	    assume $\distance(i, \home(j)) \leq 
 	    \distance(i, \workplace(j))$}
 	    
 	    \vspace{1mm}
 	    
 	    Connect location $\home(j)$ with store $i$
 	    
 	    \vspace{1mm}
 	    Remove $j$ from $\currentset$, i.e., 
 	    $\currentset \gets \currentset \backslash \{j\}$
 	    \vspace{1mm}
 	    
 	    Add $\workplace(j)$ into $\pendingset$, i.e.,
 	    $\pendingset\gets \pendingset\cup\{\workplace(j)\}$
 	    }
 	    
 	    \vspace{1mm}
 	}
\end{algorithm2e}

\newcommand{\timeindex}{t}
\newcommand{\cost}{c}

\subsection{Analysis of \Cref{alg:greedy modified}}


Similar to \citet{JMMSV-02},
we define a \emph{star} $\starinstance = (i, L)$
as a pair of one store $i$ and a subset $L$ of locations.\footnote{
We only consider stars which consist 
subset of location where every individual 
has at most one corresponding location (i.e., home or workplace) in it.}
For every star $\starinstance=(i, L)$,
let $\cost(\starinstance) = \opencost(i) + \sum_{\ell\in L}
\distance(i, \ell)$.
It is easy to see that the optimal solution is lowerbounded by\footnote{In all programs, we omit the non-negativity 
constraints of variables for writing simplicity.}
\begin{align}
\label{eq:lp relaxtion}\tag{$\mathcal{P}$}
    \begin{array}{llll}
    \min     & 
    \sum_{\starinstance}
    \cost(\starinstance)\alloc(\starinstance)
    & \text{s.t.}&\\
         &
         \sum_{\starinstance:\home(j) \in \starinstance}
         \alloc(\starinstance)
         +
         \sum_{\starinstance:\workplace(j) \in \starinstance}
         \alloc(\starinstance)
         \geq 1 
         &
         j\in[n],
         ~~~~~
         &
         \langle\dual(j)\rangle
         \\
         \\
    \max     & 
    \sum_{j\in[n]}\dual(j)
    & \text{s.t.}&\\
         &
         \sum_{\ell\in L}\alpha(\ell) \leq \cost(\starinstance)
         ~~~~~
         &
         \starinstance=(i, L),
         &
         \langle\alloc(\starinstance)\rangle
    \end{array}
\end{align}
where we abuse the notation and define $\dual(\home(j)) = 
\dual(\workplace(j)) \triangleq \dual(j)$
for every individual $j\in[n]$.

\begin{claim}
\label{claim:optimal upperbound}
The optimal total cost is lowerbounded by 
program \eqref{eq:lp relaxtion}.
\end{claim}


Now, we consider $\{\dual(j)\}$ 
(or $\{\dual(\ell)\}$ equivalently)
constructed from \Cref{alg:greedy modified}.

\begin{claim}
\label{claim:greedy upperbound}
The total cost of \Cref{alg:greedy modified}
is at most $2\cdot \sum_{j\in[n]} \dual(j)$.
\end{claim}

Due to \Cref{claim:greedy upperbound},
if we show that the dual constraints in \eqref{eq:lp relaxtion}
is satisfied when its left hand side 
is scaling down by $\gamma = 1.861$,
then we finish the proof of \Cref{thm:greedy modified}.

Let $\timeindex(\ell)$
be the time stamp when location $\ell$
is connected to some store in \Cref{alg:greedy modified}.
If location $\ell$ does not get connected to any
store at the end, we set $\timeindex(\ell) = \infty$.

\begin{claim}
For every location $\ell$,
$\timeindex(\ell) \geq \dual(\ell)$.
\end{claim}

Without loss of generality, 
we assume $\timeindex(\ell)$ is weakly increasing
in $\ell$.
Next, we establish two lemmas to characterize 
$\{\dual(\ell)\}$ as follows.

\begin{lemma}
For every store $i\in [m]$, every 
pair of locations $\ell$ and 
$\ell\primed$,
if $\timeindex(\ell) < \timeindex(\ell\primed)$,
then 
\begin{align*}
    \dual(\ell\primed) \leq 
\dual(\ell) + \distance(i,\ell) 
+ \distance(i, \ell\primed).
\end{align*}
\end{lemma}
\begin{proof}
Let $i\primed$ be the store which location $\ell$
is
connected to (since $\timeindex(\ell) < \timeindex(\ell\primed) \leq \infty$, such store $i$ exists).
Note that \Cref{alg:greedy modified} ensures that 
\begin{itemize}
    \item $\dual(\ell)\geq \distance(i\primed, \ell)$
    \item store $i$ is opened weakly before time $\timeindex(\ell) < \timeindex(\ell\primed)$, 
    and thus $\dual(\ell\primed) \leq \distance(i\primed,\ell\primed)$
\end{itemize}
Hence, by triangle inequality,
\begin{align*}
    \dual(\ell\primed) \leq \distance(i\primed, \ell\primed)
    \leq 
    \distance(i\primed, \ell) + 
    \distance(i, \ell) +
    \distance(i, \ell\primed)
    \leq 
    \dual(\ell) + 
    \distance(i, \ell) +
    \distance(i, \ell\primed).
     \ 
\end{align*}
\end{proof}


\begin{lemma}
For every star $\starinstance = (i, L)$, and 
every location $\ell\in L$, 
\begin{align*}
    \sum_{\ell\primed\in L: \ell\primed \geq \ell} 
    \plus{\min\{\dual(\ell), \dual(\ell\primed)\} - \distance(i,\ell\primed)} 
    \leq
    \opencost(i).
\end{align*}
\end{lemma}
\begin{proof}
By contradiction, suppose there exists 
a star $\starinstance = (i, L)$, and 
a location $\ell\in L$
such that 
\begin{align}
\label{eq:contradiction}
    \sum_{\ell\primed\in L: \ell\primed \geq \ell} 
    \plus{\min\{\dual(\ell), \dual(\ell\primed)\} - \distance(i,\ell\primed)} 
    >
    \opencost(i).
\end{align}
Now consider the time stamp $\timeindex(\ell)$.
By definition, 
every location $\ell\primed\in L$ such that $\ell\primed \geq \ell$
is not connected to any store 
and its dual assignment is at least 
$\min\{\timeindex(\ell),\dual(\ell\primed)\}$
at this moment $\timeindex(\ell)$.
Therefore, we can conclude that store $i$
is opened strictly before time stamp $\timeindex(\ell)$,
since
\begin{align*}
    \opencost(i) < 
    \sum_{\ell\primed\in L: \ell\primed \geq \ell} 
    \plus{\min\{\dual(\ell), \dual(\ell\primed)\} 
    - \distance(i,\ell\primed)} 
    \leq 
    \sum_{s\in L: s \geq \ell} 
    \plus{\min\{\timeindex(\ell), \dual(\ell\primed)\} 
    - \distance(i,\ell\primed)} 
\end{align*}
On the other hand, 
\eqref{eq:contradiction} also implies that
there exists at least one location $\ell^* \in L$
such that $\ell^* \geq \ell$ and 
$\min\{\timeindex(\ell), \dual(\ell^*)\} - \distance(i,\ell^*) > 0$.
By the construction of \Cref{alg:greedy modified},
$\ell^*$ should be connected to location $i$ (or some other store)
strictly before time stamp 
$\timeindex(\ell)$ (i.e., $\timeindex(\ell^*) < \timeindex(\ell)$), which leads to a contradiction. 
\end{proof}

Using two lemmas above, we can upperbound $\gamma$ by the 
following factor revealing program parameterized by
a natural number $k\in \N_{\geq 1}$,
\begin{align}
\label{eq:factor revealing program}\tag{$\mathcal{F}_k$}
    \begin{array}{lll}
    \max     & 
    \frac{\sum_{\ell\in [k]} \dual(\ell)}
    {\opencost + \sum_{\ell\in [k]} \distance(\ell)}
    & \text{s.t.} \\
         &
         \dual(\ell\primed) \leq \dual(\ell) + \distance(\ell)
         +
         \distance(\ell\primed)
         \qquad&
         \ell,\ell\primed\in[k], \ell < \ell\primed
         \\
         &
    \sum_{\ell\primed\in [\ell:k]} 
    \plus{\min\{\dual(\ell), \dual(\ell\primed)\} - \distance(\ell\primed)} 
    \leq
    \opencost
    \qquad
    &
    \ell\in[k]
    \end{array}
\end{align}
where for each dual constraint corresponded to 
star $\starinstance=(i, L)$, 
we can consider $k\gets |L|$,
$\opencost\gets \opencost(i)$,
$\distance(\ell) \gets \distance(i,\ell)$
and $\dual(\ell) \gets \in \dual(\ell)$;
and two constraints correspond to two 
characterization lemmas above.
\YF{This part is a little bit informal since the first lemma
also requires $\timeindex(\ell) < \timeindex(\ell\primed)$. However, it
can be verified that this factor revealing program is 
indeed correct.}

To rewrite program \eqref{eq:factor revealing program}
as a linear program, we 
consider all possible permutation $\permu$
for $[k]$ and define 
\begin{align}
\label{eq:factor revealing LP}\tag{$\mathcal{F}_{k,\permu}$}
    \begin{array}{lll}
    \max     & 
    \sum_{\ell\in [k]} \dual(\ell)
    & \text{s.t.} \\
    &
     \opencost + \sum_{\ell\in [k]} \distance(\ell) \leq 1
     &
    \\
    &
    \dual(\ell) \leq \dual(\ell\primed)
    &
    \ell,\ell\primed\in[k], \permu(\ell) <  \permu(\ell\primed)
    \\
         &
         \dual(\ell\primed) \leq \dual(\ell) + \distance(\ell)
         +
         \distance(\ell\primed)
         \qquad&
         \ell,\ell\primed\in[k], \ell < \ell\primed
         \\
         &
    \sum_{\ell\primed\in [\ell:k]} 
    \xi(\ell, \ell\primed)
    \leq
    \opencost
    \qquad
    &
    \ell\in[k]
    \\
    &
    \xi(\ell, \ell\primed)\geq \dual(\ell) - \distance(\ell\primed)
    &
    \ell,\ell\primed\in[k],
    \ell\leq \ell\primed,
    \permu(\ell) < \permu(\ell\primed)
    \\
    &
    \xi(\ell, \ell\primed)\geq \dual(\ell\primed) - \distance(\ell\primed)
    &
    \ell,\ell\primed\in[k],
    \ell\leq \ell\primed,
    \permu(\ell) > \permu(\ell\primed)
    \end{array}
\end{align}
\YF{The factor revealing LP \eqref{eq:factor revealing LP}
requires a parameter $\sigma$ 
to handle $\min\{\dual(\ell),\dual(\ell\primed)\}$.
Intuitively speaking, LP \eqref{eq:factor revealing LP}
should attain its worst ratio when $\sigma = (1, 2, \dots, k)$,
i.e., when
$\dual(\ell)$ is weakly increasing in $\ell$.
I numerically verified this intuition for $k \leq 8$
and it seems to be correct.
However, I cannot come up with a formal argument to proof 
this intuition at this moment. 
}
\YF{When $\sigma = (1, 2, \dots, k)$,
this is exactly the same LP in \citet{JMMSV-02}.}

==> Notes/facility-location-information.tex <==
\section{Value of Information}



In this subsection, we present a framework to 
discuss the value 
of mobility data in our home-workplace facility location problem.

To simplify the notation, we redefine the 
home-workplace facility location problem as follows.
There are $m$ locations.
Each location $i$ has $\population_i$
residents and $\employee_i$
employees.
The mobility data $\flowbf = \{\flowi\}$ specifies the home-workplace 
flow where $\flowi$
is the number of residents in location $i$
who work in location $j$.
Similar to \Cref{sec:facility model},
we denote the opening cost for a store in location $i$
as $\opencost(i)$; and the distance between location $i$
and location $j$ as $\distance(i, j)$.

\begin{remark}
Given $\{\population_i, \employee_i\}$,
a mobility data $\flowbf$ is feasible
if and only if 
$\sum_{j}\flowi = \population_i$ for every location $i$
and 
$\sum_{i}\flowi = \employee_j$ for every location $j$.
\end{remark}

\begin{remark}
Given $\{\population_i,\employee_i\}$
and $\flowbf$,
we can construct a home-workplace facility location 
problem instance using notation in \Cref{sec:facility model},
i.e., pin down 
the number of individual $n$, home location $h(j)$ and workplace location $w(j)$ for each individual $j$.
\end{remark}

We now ask the following informal research question 
about the value of the mobility data 
in this 
subsection:
% 
% \smallskip
% \begin{displayquote}
\emph{In
the home-workplace facility location problem,
how large the ratio of total cost can be
for a planner with/without the knowledge of mobility data $\flowbf$?}
% \end{displayquote}
% \smallskip

Fix an arbitrary problem instance 
$\instance = (m, \{\population_i, 
\employee_i\}, \flowbf, \distance, \opencost)$
for the home-workplace facility location problem.
A planner without the knowledge of mobility data $\flowbf$
only observes data $\phi(\instance) = (m, \{\population_i, 
\employee_i\}, \distance, \opencost)$,
i.e., everything except $\flowbf$.
Given two problem instances $\instance$ and $\instance'$
such that $\phi(\instance) = \phi(\instance')$,
a planner without the knowledge of $\flowbf$
cannot distinguish these two instances, 
and
thus will make the same decision $\SOL$
for both instances.
On the other hand, it is possible that the optimal 
decisions for the two problem instances
are different.
Thus, given any observable data $\observeinstance = (m, \{\population_i, 
\employee_i\}, \distance, \opencost)$,
we measure value 
of mobility data 
$\Gamma(\observeinstance)$ 
as the gap between 
the planners with/without the knowledge of mobility data as follows,
\begin{align*}
    \Gamma(\observeinstance) =
    \min_{\SOL}
    \max_{\instance:\phi(\instance) = \observeinstance}
    \frac{\SOL(\instance)}{\OPT(\instance)}
\end{align*}
where $\SOL\subseteq[m]$ is a feasible solution 
given the observed data $\observeinstance$,
and $\SOL(\instance)$ is the 
cost of solution $\SOL$ 
for problem instance $\instance$,
and $\OPT(\instance)$
is the optimum cost for problem instance $\instance$.

\begin{remark}
In our definition, the value of mobility data $\Gamma(\observeinstance)$
given observed data $\observeinstance$ 
characterizes a theoretical information barrier
--
no solution $\SOL$ can obtain
approximation factor better than $\Gamma(\observeinstance)$
in the worst case.
\end{remark}

In the remaining of this subsection,
we impose  
various real-world-motivated assumptions on
observed data $\observeinstance$ and discuss the 
induced value of mobility data $\Gamma(\observeinstance)$.

\subsection{General Case}
We first impose a simple assumption that the opening cost 
are identical.
\begin{assumption}
\label{asp:identical opening cost}
The opening costs are identical,
i.e., $\opencost(i) = 1$ for every location $i$.
\end{assumption}
\begin{proposition}
\label{prop:voi general}
Under \Cref{asp:identical opening cost},
there exists an observed data $\observeinstance$
with $\Gamma(\observeinstance) = m$.
\end{proposition}
\begin{proof}{{\textsl{Proof.}}}
Consider the following $\observeinstance$.
There are $m$ locations
where $\population_i = \employee_i = 1$ 
for every location $i\in[m - 1]$
and $\population_m = \employee_m = m - 1$.
The distance between any two pair of locations is infinite,
i.e., $\distance(i, j) = \infty$ for every $i \not = j$.

Fix any solution $\SOL \not= [m]$.
Consider an instance $\instance$ such that 
$\flow_{ii} = \population_i = \employee_i$ for every location $i$.
Note that $\SOL(\instance) = \infty$ and $\OPT(\instance) = m$.

Fix the solution $\SOL = [m]$.
Consider an instance $\instance$
such that $\flow_{im} = \flow_{mi} = 1 $ for every location $i\in[m-1]$.
Note that $\SOL(\instance) = m$ and $\OPT(\instance) = 1$.
 \ 
\end{proof}

In the proof of 
\Cref{prop:voi general},
we consider an observed data $\observeinstance$
whose (i) distances between different locations are infinite;
and (ii) different locations have heterogeneous 
populations and employments.
Next we will introduce additional assumptions 
to exclude (i) and (ii) by considering
two more real-world-motivated regimes
(i.e., \emph{urban regime} and \emph{rural regime}).


\begin{proposition}
\label{prop:voi general upperbound}
For any observed data $\observeinstance$
under \Cref{asp:identical opening cost},
$\Gamma(\observeinstance) = O(m)$.
\end{proposition}
\begin{proof}{\textsl{Proof.}}
Note that $\SOL = [m]$
guarantees that 
$\frac{\SOL(\instance)}{\OPT(\instance)} \leq m$
for all $\instance$ such that $\phi(\instance) = \observeinstance$.
 \ 
\end{proof}



\newcommand{\distanceupperbound}{C}
\subsection{Urban Regime}
In the urban regime, we impose the assumption
that the distance of different locations are upperbounded.
\begin{assumption}
\label{asp:distance upper bound}
There exists $\distanceupperbound\geq 0$ such that 
$\distance(i, j) \leq \distanceupperbound$ 
for every pair of locations $(i, j)$.
\end{assumption}

\begin{proposition}
Under \Cref{asp:identical opening cost}
and \Cref{asp:distance upper bound},
there exists an observed data $\observeinstance$
with $\Gamma(\observeinstance) \geq 
\min\{m, \sqrt{n\cdot \distanceupperbound}\}$,
where $n = \sum_{i\in[m]} \population_i$ is the total population.
\end{proposition}
\begin{proof}{\textsl{Proof.}}
We first focus on the parameter regime where
$m \leq \sqrt{n\cdot \distanceupperbound}$.
In this regime, consider
the following $\observeinstance$ similar to 
the one in \Cref{prop:voi general}.
There are $m$ locations.
For each location $i \in [m-1]$,
$\population_i = \employee_i = \frac{n}{2(m - 1)}$;
and $\population_m = \employee_m = \frac{n}{2}$.
The distance between every pair of locations $(i, j)$
equals to $\distanceupperbound$,
i.e., $\distance(i, j) = \distanceupperbound$.

In the other parameter regime where
$m >\sqrt{n\cdot \distanceupperbound}$,
let $m\primed = \sqrt{n \cdot \distanceupperbound}$.
Now consider the following $\observeinstance$.
There are $m$ locations. 
For each location $i \in [m\primed-1]$,
$\population_i = \employee_i = \frac{n}{2(m\primed - 1)}$;
for each location $i\in [m\primed:m - 1]$,
$\population_i = \employee_i = 0$;
and $\population_m = \employee_m = \frac{n}{2}$.
The distance between every pair of locations $(i, j)$
equals to $\distanceupperbound$,
i.e., $\distance(i, j) = \distanceupperbound$.
With the similar argument as the first regime ($m\leq \sqrt{n\cdot C}$),
we can conclude that for any solution $\SOL$, 
there exists $\instance$ such that $\frac{\SOL(\instance)}{\OPT(\instance)} \geq m\primed = \sqrt{n\cdot \distanceupperbound}$,
which finishes the proof.
 \ 

% Fix any $\SOL \subseteq[m]$.
% Let $i\primed = \min~\SOL$
% and $i\doubleprimed = \min~([m]\backslash\SOL)$.
% Consider an instance $\instance_{\SOL}$ where 
% (i)
% $\flow_{j i \primed} = \flow_{i\primed j} = \population_j$
% for every location $j\in \SOL\backslash\{i\primed\}$;
% (ii)
% $\flow_{j i\doubleprimed} = 
% \flow_{i\doubleprimed j} = \population_j$
% for every location $j\in
% [m]\backslash\SOL
% \backslash\{i\doubleprimed\}$;
% (iii) 
% $\flow_{i\primed i\primed} = \population_{i\primed} - 
% \sum_{j \in  \SOL\backslash\{i\primed\}} 
% \population_j>0$;
% and
% (iv) 
% $\flow_{i\doubleprimed i\doubleprimed} 
% = \population_{i\doubleprimed} - 
% \sum_{j \in  [m]\backslash\SOL
% \backslash\{i\doubleprimed\}}
% \population_j>0$.
% Under this instance $\instance_{\SOL}$, $\OPT = \{i\primed, i\doubleprimed\}$
% and $\OPT(\instance_{\SOL}) = 2$.
% On the other hand, $\SOL(\instance_{\SOL}) = |\SOL| + \sum_{i\in[m]\backslash\SOL} \population_i \cdot \distanceupperbound$.
% Hence,
% \begin{align*}
%     \Gamma(\observeinstance) \geq 
%     \min_{\SOL\subseteq[m]}
%     \frac{\SOL(\instance_{\SOL})}{\OPT(\instance_{\SOL})}
%     \geq 
%     \min_{k\in [0:m]}
%     \frac{k + n\cdot \distanceupperbound\cdot 
%     \left(
%     \frac{1}{2^k} - \frac{1}{2^m}
%     \right)}{2}
%     \overset{(a)}{=} 
%     \Theta\left(
%     m,
%     \log(n\cdot \distanceupperbound)
%     \right)
% \end{align*}
% where equality holds by taking 
% $k = \min\{m, \log(n\cdot \distanceupperbound) + o(n\cdot \distanceupperbound)\}$.
%  \ 
\end{proof}

\begin{proposition}
For any observed data $\observeinstance$
under \Cref{asp:identical opening cost}, \Cref{asp:distance upper bound}
and 
$\distance(i,j) \geq \sqrt{\distanceupperbound/n}\cdot \indicator{i\not = j}$,
$\Gamma(\observeinstance) = 
O(\min\{m,\sqrt{n\cdot C} + 1\})$.
\end{proposition}
\begin{proof}{\textsl{Proof.}}
Fix any observed data $\observeinstance$.
Due to \Cref{prop:voi general upperbound},
it is sufficient to show 
$\Gamma(\observeinstance) = 
O(\sqrt{n\cdot \distanceupperbound})$.
Let $\SOL = 
\{1\}\cup
\{i\in[m]:
\population_i \cdot \distanceupperbound
\geq \sqrt{n\cdot \distanceupperbound}\}
\cup
\{i\in[m]:
\employee_i \cdot \distanceupperbound
\geq \sqrt{n\cdot \distanceupperbound}\}$.
Note that by construction, 
(i) $1 \leq |\SOL| \leq 2 \sqrt{n\cdot \distanceupperbound} + 1$;
and 
(ii)
for every location $i\not\in \SOL$,
$\population_i\cdot \distanceupperbound < 
\sqrt{n\cdot\distanceupperbound}$
and 
$\employee_i\cdot \distanceupperbound < 
\sqrt{n\cdot\distanceupperbound}$.

Now consider an arbitrary instance $\instance$
such that $\phi(\instance) = \observeinstance$.
Denote the optimal solution for this instance as 
$\OPT \subseteq[m]$.
By definition, $\OPT\backslash\SOL$
is the set of location where
stores are opened in solution $\OPT$
but not in solution $\SOL$.
Similarly, $[m]\backslash\SOL\backslash\OPT$
is the set of location 
where stores are not opened in neither $\OPT$ or $\SOL$. 
Let $\population_A$ be the number of individuals 
who reside or work in $\OPT\backslash\SOL$;
and $\population_B$ be the number of individuals 
who both reside and work in $[m]\backslash\SOL\backslash\OPT$.
We highlight that $\population_A \cdot \distanceupperbound\leq 
2\sqrt{n\cdot \distanceupperbound}\,|\OPT\backslash\SOL|$. 
Note that 
\begin{align*}
    \SOL(\instance) &\leq 
    \underbrace{|\SOL|}_{\text{opening costs}}
    +
    \underbrace{\distanceupperbound\cdot \population_A}_{
    \text{
    % upper bound of 
    connection costs upperbound for $\population_A$}}
    +
    \underbrace{\distanceupperbound\cdot \population_B}_{
    \text{
    % upper bound of 
    connection costs upperbound for $\population_B$}}
    \\
    \OPT(\instance) &\geq 
        \underbrace{|\OPT|}_{\text{opening costs}}
    +
    \underbrace{
    \sqrt{
    % \frac
    {\distanceupperbound}/{n}}
    \cdot \population_B}_{
    \text{
    % upper bound of 
    connection costs lowerbound for $\population_B$}}
\end{align*}
Thus,
% Let $\SOL(\instance,i)$
% (resp.\ $\OPT(\instance, i)$)
% be the cost 
% related to location $i\in[m]$
% (i.e., the opening cost for the store at location $i$
% if applicable, and the connection cost for 
% population $\population_i$)
% in solution $\SOL$ (resp.\ $\OPT$).
% By definition, $\SOL(\instance) = \sum_{i\in[m]}\SOL(\instance,i)$
% and $\OPT(\instance) 
% = \sum_{i\in[m]}\OPT(\instance,i)$.
% Note that
\begin{align*}
    \frac{\SOL(\instance)}
    {\OPT(\instance)}
    =
     \frac{2\SOL(\instance)}
    {2\OPT(\instance)}
    \leq 
    \max\left\{
    \frac{2|\SOL|}
    {
    \OPT(\instance)
    }
    ,
    \frac{2\distanceupperbound\cdot \population_A}{|\OPT|},
    \frac{2\distanceupperbound\cdot \population_B}{
        \sqrt{
    % \frac
    {\distanceupperbound}/{n}}
    \cdot \population_B}
    \right\}
\end{align*}
where 
\begin{align*}
    \frac{|\SOL|}
    {
    \OPT(\instance)
    }
    &\leq
    \frac{|\SOL|}{1} 
    \leq 
    2\sqrt{n\cdot \distanceupperbound} + 1
    \\
    \frac{\distanceupperbound\cdot \population_A}{|\OPT|}
    &\leq 
    \frac{\distanceupperbound\cdot \population_A}{|\OPT\backslash\SOL|}
    \leq 
   2\sqrt{n\cdot \distanceupperbound}
 \ 
\end{align*}
% and for every $j\not\in\SOL$
% \begin{align*}
%     \frac{\SOL(\instance,j)}{\OPT(\instance,j)}
% \end{align*}
\end{proof}


\begin{comment}
\begin{proposition}
Under \Cref{asp:identical opening cost}
and \Cref{asp:distance upper bound},
there exists an observed data $\observeinstance$
with $\Gamma(\observeinstance) = 
\Theta(\min\{m, \log(n\cdot \distanceupperbound)\})$,
where $n = \sum_{i\in[m]} \population_i$ is the total population.
\end{proposition}
\begin{proof}{\textsl{Proof.}}
Consider the following $\observeinstance$.
There are $m$ locations.
For each location $i \in [2:m]$,
$\population_i = \employee_i = \frac{n}{2^i}$;
and $\population_1 = \employee_1 = n - \sum_{i\in[2:m]}\population_i = \frac{n}{2} + \frac{n}{2^m}$.
The distance between every pair of locations $(i, j)$
equals to $\distanceupperbound$,
i.e., $\distance(i, j) = \distanceupperbound$.

Fix any $\SOL \subseteq[m]$.
Let $i\primed = \min~\SOL$
and $i\doubleprimed = \min~([m]\backslash\SOL)$.
Consider an instance $\instance_{\SOL}$ where 
(i)
$\flow_{j i \primed} = \flow_{i\primed j} = \population_j$
for every location $j\in \SOL\backslash\{i\primed\}$;
(ii)
$\flow_{j i\doubleprimed} = 
\flow_{i\doubleprimed j} = \population_j$
for every location $j\in
[m]\backslash\SOL
\backslash\{i\doubleprimed\}$;
(iii) 
$\flow_{i\primed i\primed} = \population_{i\primed} - 
\sum_{j \in  \SOL\backslash\{i\primed\}} 
\population_j>0$;
and
(iv) 
$\flow_{i\doubleprimed i\doubleprimed} 
= \population_{i\doubleprimed} - 
\sum_{j \in  [m]\backslash\SOL
\backslash\{i\doubleprimed\}}
\population_j>0$.
Under this instance $\instance_{\SOL}$, $\OPT = \{i\primed, i\doubleprimed\}$
and $\OPT(\instance_{\SOL}) = 2$.
On the other hand, $\SOL(\instance_{\SOL}) = |\SOL| + \sum_{i\in[m]\backslash\SOL} \population_i \cdot \distanceupperbound$.
Hence,
\begin{align*}
    \Gamma(\observeinstance) \geq 
    \min_{\SOL\subseteq[m]}
    \frac{\SOL(\instance_{\SOL})}{\OPT(\instance_{\SOL})}
    \geq 
    \min_{k\in [0:m]}
    \frac{k + n\cdot \distanceupperbound\cdot 
    \left(
    \frac{1}{2^k} - \frac{1}{2^m}
    \right)}{2}
    \overset{(a)}{=} 
    \Theta\left(
    m,
    \log(n\cdot \distanceupperbound)
    \right)
\end{align*}
where equality holds by taking 
$k = \min\{m, \log(n\cdot \distanceupperbound) + o(n\cdot \distanceupperbound)\}$.
 \ 
\end{proof}
\end{comment}

\newcommand{\populationupperbound}{\Delta}
\newcommand{\distancelouwerbound}{C}

\subsection{Rural Regime}
In the rural regime, we impose the assumption that 
heterogeneity of 
the populations and employments 
in different locations are bounded.
Specifically, 
there exists a constant $\populationupperbound$
such that $\frac{\population_i}{ \population_j}\leq \populationupperbound_N$
and $\frac{\employee_i}{\employee_j}\leq \populationupperbound_E$
for every location $i, j$.
Additionally, we impose another assumption
that the distance of different location are lowerbounded.
Specifically, there exists a constant $\distancelouwerbound$ such that 
$\distance(i, j) \geq \distancelouwerbound$ 
for every location $i\not= j$.

\begin{assumption}
\label{asp:distance lower bound}
There exists $\distanceupperbound\geq 0$ such that 
$\distance(i, j) \geq \distancelouwerbound$ 
for every pair of locations $(i, j)$.
\end{assumption}

\begin{assumption}
\label{asp:population ratio bound}
There exists $\populationupperbound\geq 1$
% and $\populationupperbound_E \geq 1$ 
such that 
$\frac{\population_i}{\population_j} \leq \populationupperbound$
and 
$\frac{\population_i}{\population_j} \leq \populationupperbound$
for every pair of locations $(i, j)$.
\end{assumption}

\begin{comment}
\begin{proposition}
There exists an observed data $D$ with $\Gamma(D)=  \sqrt{\populationupperbound_N \populationupperbound_E}+1. $
\end{proposition}
\begin{proof}{\textsl{Proof.}}
Suppose $C\rightarrow \infty$.
Note that any
$\SOL$ that  does not open all locations will have $\SOL(I)/OPT(I) \rightarrow \infty$ for some problem instance. Consider such $\SOL$, which has $\SOL(I)=m$ for all problem instances.

Suppose the problem data is such that 
we have two set of nodes $L$ (``leafs'') and $L^c$ such that for any $i\in L^c$ we have $N_i=\populationupperbound_N$ and $E_i= \alpha \populationupperbound_E $ and for $i\in L$ we have $N_i=1$ and $E_i=\alpha$.
Here, we assume $\alpha = (|L| + |L^c| \populationupperbound_N )/(|L|+ |L^c| \populationupperbound_E) $  so that the total number of jobs and people match.
Suppose that $\tau_{ij}=1/|L^c|$ for $i\in L$, $j\in L^c$ and
$\tau_{ij}=1/|L|$ for $i\in L^c$ and $j\in L$. For all other $i,j$ we have $\tau_{ij}=0$. Note that opening only $L^c$ we obtain a solution with cost $L^c$.
Thus, it follows that $\Gamma (D)=(|L|| +|L^c| )  / |L^c|= |L|/|L^c|+1$.

Note that by construction of $\tau_{ij}$, we have:
\begin{align}
    \populationupperbound_{E} |L^c| \alpha&= |L| \alpha\\
    \populationupperbound_{N} |L^c|&= |L|
\end{align}
Multiplying these equalities yields $
|L|/|L^c|=
\sqrt{\populationupperbound_E \populationupperbound_N}  $. Thus, it follows that $\Gamma(D) =\sqrt{\populationupperbound_E \populationupperbound_N} +1 $ as claimed. 
\hfill  \ 
\end{proof}
Note that in our construction for this result we have $m= |L| + |L^c| = |L^c| (\sqrt{\populationupperbound_E\populationupperbound_N} +1)$. So there is no need to take the minimum of the bound in the proposition and $m$. 
\end{comment}


\begin{proposition}
\label{prop:voi rural lowerbound}
Under \Cref{asp:identical opening cost},
\Cref{asp:distance lower bound}
and \Cref{asp:population ratio bound},
there exists an observed data $\observeinstance$
with 
\begin{align*}
    \Gamma(\observeinstance) = 
    \left\{
    \begin{array}{ll}
      m   
      &\qquad
      \text{if $\populationupperbound+1\geq m$}
      \\
      &
      \\
%       \max_{\alpha\in[\populationupperbound + 1, m]}
%       \frac{
%       \frac{\populationupperbound}{\populationupperbound + 1}\alpha 
%     + 1
%     +
%   {\distancelouwerbound}
%     (\alpha - \populationupperbound - 1)\frac{n}{2m}
%       }{
%       1
%     +
%   {\distancelouwerbound}
%     (\alpha - \populationupperbound - 1)\frac{n}{m}
%       }
\max\left\{\populationupperbound + 1,
      \frac{
      \frac{\populationupperbound}{\populationupperbound + 1}m 
    + 1
    +
  {\distancelouwerbound}
    (m - \populationupperbound - 1)\frac{n}{2m}
      }{
      1
    +
  {\distancelouwerbound}
    (m - \populationupperbound - 1)\frac{n}{m}
      }
\right\}
       &\qquad
       \text{if $\populationupperbound + 1\leq m$}
    \end{array}
    \right.
\end{align*}
where $n = \sum_{i\in[m]} \population_i$ is the total population.
\end{proposition}
As a sanity check, \Cref{prop:voi rural lowerbound}
implies that 
% for observed data $\observeinstance$ such that 
% $\populationupperbound +1 \leq m$, 
% $\Gamma(\observeinstance)\geq \populationupperbound + 1$ 
% by taking $\alpha = \populationupperbound + 1$;
while holding all other parameters fixed, 
as
$\distancelouwerbound$ goes to zero,
we have $\Gamma(\observeinstance) 
\geq \frac{\populationupperbound}{\populationupperbound+1}m + 1
\geq \populationupperbound + 1$ if $\populationupperbound + 1 \leq m$.
Additionally, when $\populationupperbound = o(m)$,
and $\distancelouwerbound =
\Omega(\frac{m}{n\populationupperbound})$,
$\Gamma(\observeinstance) = \Omega(\populationupperbound)$.

\begin{proof}{\textsl{Proof of \Cref{prop:voi rural lowerbound}}.}
We first focus on the parameter regime where 
$\populationupperbound + 1\geq m$.
In this regime, note that the observed data $\observeinstance$
constructed in \Cref{prop:voi general}
satisfies \Cref{asp:identical opening cost},
\Cref{asp:distance lower bound}
and \Cref{asp:population ratio bound}, and guarantees 
$\Gamma(\observeinstance) = m$.

In the other parameter regime where $\populationupperbound + 1\leq m$,
let $\alpha$ be an arbitrary number between 
$[\populationupperbound + 1,m]$.
Consider the following observed data $\observeinstance$.
There are $m$ locations. 
All locations can be partitioned into 
$ \frac{m}{\alpha}~(\triangleq\ell)$ 
sets $\{L_1, \dots, L_{\ell}\}$.\footnote{For simplicity, 
we allows fractional number of locations in each set $L_j$.}
The distance between any two locations $i, j$ such that $i\in L_a$,
$ j\in L_b$ and $a \not = b$ are infinite, i.e., $\distance(i, j) = \infty$. All sets $\{L_a\}_{a\in[\ell]}$ 
will be symmetric and thus we just describe 
the construction of $L_1$.
$L_1$ contains $\alpha$ locations.
Let 
$k = 
\frac{\alpha}
{\populationupperbound + 1}$,
and $x = \frac{1}{2}
\frac{\populationupperbound+1}{\populationupperbound}
\frac{n}{m}$.
For every location $i\in [k]$, 
$\population_i = \employee_i = \populationupperbound \cdot x$;
and 
for each location $i\in[k + 1: \alpha]$,
$\population_i = \employee_i = x$.
As a sanity check,
the total population in $L_1$ 
is 
\begin{align*}
    k\cdot \populationupperbound\cdot x + (\alpha - k)
    \cdot x
    &=
    \frac{\alpha}{\populationupperbound + 1}
    \cdot \populationupperbound \cdot 
\frac{1}{2}
\frac{\populationupperbound+1}{\populationupperbound}
\frac{n}{m}
+
\frac{\alpha\cdot \populationupperbound}{\populationupperbound + 1}
\cdot 
\frac{1}{2}
\frac{\populationupperbound+1}{\populationupperbound}
\frac{n}{m}
=
\frac{\alpha\,n}{m}
=
\frac{n}{\ell}
\end{align*}
The distance between any two locations $i, j$ in $L_1$ is as follows,
\begin{align*}
    \distance(i, j) = \left\{
    \begin{array}{ll}
    \distancelouwerbound     &
    \qquad\text{if $i \in [k], j\in [k]$}\\
    \infty     &
    \qquad\text{otherwise}
    \end{array}
    \right.
\end{align*}
Due to the symmetricity of all sets ${L_a}_{a\in[\ell]}$, 
it is sufficient to consider $\SOL$ for $L_1$.
Note that for any $\SOL$ that does not open all locations in 
$[k + 1:\alpha]$ and one location in $[k]$,
there exists an instance $\instance$
where $\flow_{ii} = \population_i = \employee_i$ 
for every location $i\in L_1$ 
such that $\SOL(\instance) = \infty$
and $\OPT(\instance) \leq \alpha$.
Now, consider $\SOL = [k+1:\alpha]\cup\{1\}$.
Consider the following instance $\instance$
where $\flow_{ij}= \flow_{ji} = \population_j~(=x)$ for 
every location $i\in [k]$ and location $j\in[k + 1:\alpha]$.
By construction, $\OPT$ opens location 1 only and thus
\begin{align*}
    \SOL(\instance) &= \alpha - k + 1 + 
    \sum_{i \in [2:k]}\distancelouwerbound\cdot \population_i
    =
    \frac{\populationupperbound}{\populationupperbound + 1}\alpha 
    + 1
    +
   {\distancelouwerbound}
    (\alpha - \populationupperbound - 1)\frac{n}{2m}
    \\
    \OPT(\instance) &= 1 + 2\sum_{i\in[2:k]}
    \distancelouwerbound\cdot \population_i =
    1 +  {\distancelouwerbound}
    (\alpha - \populationupperbound - 1)\frac{n}{m}
\end{align*}
which finihes the proof.
 \ 
\end{proof}

\begin{proposition}
For any observed data $\observeinstance$
under \Cref{asp:identical opening cost}, \Cref{asp:population ratio bound},
and 
\Cref{asp:distance lower bound} with 
$\distancelouwerbound$ goes to $\infty$,
$\Gamma(\observeinstance) = 
% O(
\min\{\populationupperbound + 1,m\}$.
\end{proposition}

\begin{proof}{\textsl{Proof.}}
Fix any observed data $\observeinstance$.
Due to \Cref{prop:voi general upperbound},
it is sufficient to show 
$\Gamma(\observeinstance) \leq \populationupperbound + 1$.
Consider a solution $\SOL = [m]$, 
we will show 
that for any instance $\instance$ such that
$\phi(\instance) = \observeinstance$,
$\OPT(\instance) = |\OPT|
% \Omega\left(
\frac{m}{\populationupperbound + 1}
% \right)
=
% \Omega\left(
\frac{\SOL(\instance)}{\populationupperbound + 1}
% \right)$.
$.

Note that the assumption \Cref{asp:distance lower bound}
with $\distancelouwerbound$ goes to $\infty$
ensures that for every individual, either 
her home location or her workplace has an 
opened store in $\OPT$. 
Thus, we have 
\begin{align*}
    \sum_{i\in\OPT} \employee_i \geq 
    \sum_{i\in[m]\backslash\OPT} \population_i
\end{align*}
Combining with the fact that 
$\sum_{i\in[m]}\population_i =
\sum_{i\in[m]}\employee_i$,
\begin{align*}
    \sum_{i\in\OPT} 
    (\employee_i + \population_i)
    \geq 
    \sum_{i\in[m]\backslash\OPT} 
    (\employee_i + 
    \population_i)
\end{align*}
which implies 
\begin{align*}
    |\OPT| \cdot 
    \populationupperbound\cdot 
    \left(\min_i \population_i + 
    \min_i \employee_i 
    \right)
    \geq 
    (m - |\OPT|) \cdot 
    \left(\min_i \population_i + 
    \min_i \employee_i 
    \right)
\end{align*}
thus $\OPT(\instance) = |\OPT| = \frac{m}{\populationupperbound + 1}$,
which finishes the proof.
 \ 
\end{proof}

\begin{proposition}
\label{prop:voi rural upperbound}
For any observed data $\observeinstance$
under \Cref{asp:identical opening cost}, \Cref{asp:population ratio bound}
with $\populationupperbound + 1 \leq 2 m$,
and 
\Cref{asp:distance lower bound} with 
$\distancelouwerbound = 
\frac{\populationupperbound + 1}{\populationupperbound}\cdot n$,
then
$\Gamma(\observeinstance) \leq \frac{\populationupperbound}{\populationupperbound + 1}m$.
% \min\{\populationupperbound + 1,m\})$.
\end{proposition}

To interpret \Cref{prop:voi rural upperbound}, 
consider $\SOL = [m]$, i.e., opening stores 
in all locations. To show $\Gamma(\observeinstance) \leq \frac{\populationupperbound}{\populationupperbound + 1}m$,
it is necessary to show for every instance $\instance$ 
such that
$\phi(\instance) = \observeinstance$ the optimal cost
$\OPT(\instance)$ is at least $1 + \frac{1}{\populationupperbound}$.


\begin{proposition}
For any observed data $\observeinstance$
under \Cref{asp:identical opening cost}, \Cref{asp:population ratio bound}
% with $\populationupperbound + 1 \leq 2 m$,
and 
\Cref{asp:distance lower bound} with 
$\distancelouwerbound = 
\frac{m}{n\populationupperbound}$,
then
$\Gamma(\observeinstance) = O(\Delta)$.
\end{proposition}
\begin{proof}{\textsl{Proof.}}
Fix an arbitrary observed data $\observeinstance$.
Let $\SOL = [m]$.
For any instance $\instance$ such that 
$\phi(\instance) = \observeinstance$.
Suppose $\OPT$ is the optimal solution 
for instance $\instance$.
Let $x \triangleq |\SOL|$.
Denote by $\population_A$  
the number of individuals 
who reside or work in $\OPT$,
and let $\population_B = n - \population_A$.
Due to \Cref{asp:population ratio bound},
we have 
\begin{align*}
    \frac{\population_A}{2x} \leq 
    \populationupperbound\cdot 
    \frac{\population_B}{m - 2x}
\end{align*}
which implies 
\begin{align*}
    \population_B \geq 
    \left(
    1 - \frac{2\populationupperbound x}
    {m + 2(\populationupperbound - 1)x}
    \right)n
\end{align*}
Combining with \Cref{asp:distance lower bound}
with $\distancelouwerbound = \frac{m}{n\populationupperbound}$,
we have
\begin{align*}
    \OPT \geq x + 
    \population_B \cdot 
    \distancelouwerbound
    \geq 
    x + \frac{m}{\populationupperbound}
    \left(
    1 - \frac{2\populationupperbound x}
    {m + 2(\populationupperbound - 1)x}
    \right)
\end{align*}
where the right-hand side is first decreasing and 
then increasing in $x$ with the minimum attained 
at $x = \frac{\sqrt{2} - 1}{2(\populationupperbound - 1)}m$
if $\populationupperbound > 1$, and $x = m$ otherwise.
To see this,
consider its derivative with respect to $x$,
\begin{align*}
    &1 - 
    \frac{m}{\populationupperbound}
    \frac{2\populationupperbound}{m + 2(\populationupperbound - 1)x}
    +
    \frac{m}{\populationupperbound}
    \frac{4\populationupperbound(\populationupperbound - 1)x}
    {(m + 2(\populationupperbound - 1)x)^2}
\intertext{whose sign does not change by multiplying
$(m + 2(\populationupperbound - 1)x)^2$, i.e., }
&\populationupperbound(m + 2(\populationupperbound - 1)x)^2
-
2m\populationupperbound(m + 2(\populationupperbound - 1)x)
+
m(4\populationupperbound(\populationupperbound - 1)x)
\intertext{After simplification, it becomes }
&4(\populationupperbound - 1)^2x^2 + 
4(\populationupperbound - 1)mx - m^2
\end{align*}
% \intertext{
which finishes the argument 
that the minimum is attained at 
$x = \frac{\sqrt{2} - 1}{2(\populationupperbound - 1)}m$.

Putting all pieces together, $\Gamma(\observeinstance) \leq \frac{m}{\frac{\sqrt{2} - 1}{2(\populationupperbound - 1)}m} = O(\populationupperbound)$.
\hfill \ 
\end{proof}

\subsection{Approximation for 
Minimax Solution}
In practice, a common robust approach 
when social planners face uncertainty (e.g., 
knowledge of $\flowbf$) is to consider the 
minimax solution. 
In particular, given observed data $\observeinstance$,
social planners may implement 
\begin{align*}
    \SOL\primed =
    \argmin\limits_{\SOL}
    \max\limits_{\instance:\phi(\instance) = \observeinstance}
    \SOL(\instance).
\end{align*}
Here we show that this minimax solution is at least 
a $m$-approximation.
\begin{proposition}
For any observed data $\observeinstance$
under \Cref{asp:identical opening cost},
the minimax solution $\SOL\primed$
is a $m$-approximation, i.e., 
\begin{align*}
    \max_{\instance:\phi(\instance)= \observeinstance}
    \frac{\SOL\primed(\instance)}{\OPT(\instance)}
    \leq m
\end{align*}
\end{proposition}
\begin{proof}{\textsl{Proof.}}
Consider solution $\SOL_0 = [m]$ which opens 
stores in all location.
By definition, the minimax solution $\SOL\primed$
satisfies that 
\begin{align*}
    \max\limits_{\instance:\phi(\instance)=\observeinstance}
    \SOL\primed(\instance) 
    \leq 
    \max\limits_{\instance:\phi(\instance)=\observeinstance}
    \SOL_0(\instance) = m
\end{align*}
Thus, for every instance $\instance$
such that $\phi(\instance) = \observeinstance$,
we have $\SOL\primed(\instance) \leq m$.
Combining with the fact that $\OPT(\instance) \geq 1$
finishes the proof.
\hfill \ 
\end{proof}

\newpage

% \begin{lemma}
\vspace{1mm}
\noindent \textbf{Tasks.} 
\begin{itemize}
    \item Impose additional constraints on the flow.
    \begin{itemize}
    \item Suppose two types of locations $L$,$H$.
    \item We have 
    \begin{itemize}
        \item $\sum_{i\in L} N_i > \rho_1 \sum_{i} N_i$
        \item $\sum_{i\in H} E_i > \rho_2 \sum_{i} E_i$
        \item  $\sum_{j\in H} \tau_{ij}> \rho_3  N_i$ for each $i$
        \begin{itemize}
        \item weaker version:
        $\sum_{i\in H}\sum_{j\in H}\tau_{ij} \geq \rho_3 
        \sum_{j\in H} N_j$.
        \end{itemize}
    \end{itemize}
    for some $\rho_1,\rho_2,\rho_3>1/2$.
    \item 
    
    % \item  $\sum_{j\in H}\tau_{ij} > \rho N_i$ for some $\rho>1/2$.
        % \item $N_i$ is arbitrary
        % \item Each location $i$ has attractiveness $a_i$. Let $A=\sum_i a_i$
        % \item $\tau_{ij}= N_i \times a_j/A $
    \end{itemize}
    \item Explore having planarity requirement
\end{itemize}


\noindent \textbf{Related papers:}
\begin{itemize}
    \item \url{https://pubsonline.informs.org/doi/pdf/10.1287/opre.43.4.623}
\end{itemize}
% \end{lemma}
\newpage
\subsection{A Sufficient Condition 
for Approximately Optimality for Work Heuristic}

Fix an arbitrary problem instance $\instance$.
Suppose the optimal solution $\OPT(\instance)$
satisfies the following two assumptions.

\begin{assumption}
Let $N_w$ be the number of individuals 
whose workplace is within the serving radius $R$
of $\OPT(\instance)$,
and $N$ be the number of individuals whose
workplace or home
is within the serving radius $R$ of $\OPT(\instance$ 
(i.e., $\servingpopulation(\OPT(\instance))$.
Then $\frac{N_w}{N} \geq \gamma$.
\end{assumption}

\begin{assumption}
Suppose $
{\displaystyle\sum_{i\in\OPT(\instance)}\opencosti}
\leq \zeta\cdot {\servingpopulation(\OPT(\instance))}$.
\end{assumption}

\begin{theorem}
Let $\SOL$ be the solution computed from 
work heuristic.
Under Assumption C.8 and C.9,
$\Profit[\instance]{\SOL} \geq (\gamma - \zeta)
\cdot 
\Profit[\instance]{\OPT(\instance)}$
\end{theorem}

\newpage 

==> Notes/facility-location-model.tex <==


\section{Model}
\label{sec:facility model}
Here we consider 
the home-workplace facility location problem.

\begin{itemize}
\item A city consists of $n$ individuals $[n]$. 
Each individual $j$ has 
home location $\home(j)$ and workplace location $\workplace(j)$.
We use index $\ell$ to denote a location from 
$\{\home(j):j\in [n]\}\cup\{\workplace(j):j\in [n]\}$.

\item A brand has $m$ possible locations $[m]$ for stores.
Each store $i$ has an opening cost $\opencost(i)$.

\item The connection cost between store $i$ to individual $j$
is 
$$\connectioncost(i, j) = \min\{\distance(i, \home(j)), \distance(i, \workplace(j))\}$$
where $\distance(\cdot,\cdot)$ is a metric (e.g., 
Euclidean distance).
Note that $\connectioncost(\cdot,\cdot)$ is not
necessarily a metric.

\item The goal of the brand
is find a subset $\sol \subseteq[m]$ to minimize
$$
\sum_{i\in \sol} \opencost(i) + \sum_{j\in[n]} \connectioncost(\sol, j)
\;\;
\mbox{where}
\;\;
\connectioncost(\sol,j) = \min_{i\in \sol} \connectioncost(i, j)
$$
\end{itemize}




==> Notes/factor-revealing-program.tex <==
\section{Simplification of Factor Revealing Program}
\label{apx:factor-revealing program}
\begin{comment}
\subsection{Approach I: Towards 3.08-Approximation}

% For Program~\ref{eq:factor revealing program}
% parameterized by $\mHat,\singlecountedgesetHat,\doublecountedgesetHat$, we can straightforwardly show that 

% \begin{align*}
    
% \end{align*}

\paragraph{Reformulation as linear program}
% Given any $\mHat\in\N_{\geq 1}$,
% let onsider any permutation $\permu:[\mHat]\rightarrow[\mHat]$.
For Program~\ref{eq:factor revealing program}
parameterized by $\mHat,\singlecountedgesetHat,\doublecountedgesetHat$,
there exists a permutation $\permu:[\mHat]\rightarrow[\mHat]$
such that 
Program~\ref{eq:factor revealing program} is 
at most Program~\ref{eq:factor revealing program 1}
parameterized by $\mHat,\singlecountedgesetHat,\doublecountedgesetHat,\permu$ as follows.

\newcommand{\xHat}{\hat{x}}

\begin{align*}
\label{eq:factor revealing program 1}
\tag{$\mathcal{P}_{\texttt{FR-1}}$}
    \arraycolsep=5.4pt\def\arraystretch{1}
    &\begin{array}{clll}
    \max\limits_{\substack{\costHat,
    \{\xHat(\ell,\ell')\}_{\ell,\ell'\in[\mHat]}
    \\
    \{\muHat(\ell),\distanceHat(\ell),
\distanceHatStar(\ell)\}_{\ell\in[\mHat]}}} &
    \displaystyle\sum\nolimits_{\ell\in\singlecountedgesetHat}
     \muHat(\ell) 
     +
     \displaystyle\sum\nolimits_{\ell\in\doublecountedgesetHat}
     2\muHat(\ell) - \distanceHatStar(\ell)
    & \text{s.t.} & \\
    \langle\frcone\rangle
    & 
    \muHat(\ell') \leq \distanceHatStar(\ell) 
    + \distanceHat(\ell) + \distanceHat(\ell')
     & 
     \ell,\ell'\in[\mHat], \ell < \ell'
     &
     \\
    \langle\frctwo\rangle
     &
     \displaystyle\sum\nolimits_{\ell'\in[\ell:\mHat]}
     \xHat(\ell,\ell')
     \leq 
     \costHat
     &
     \ell\in[\mHat]
     &
     \\
    \langle\frcthree\rangle
     &
     \costHat 
     +
     \displaystyle\sum\nolimits_{\ell\in[\mHat]}
     \distanceHat(\ell)
     \leq 1
     &
     \\
    \langle\frcfour\rangle
     &
     \distanceHatStar(\ell) \leq \muHat(\ell)
     &
     \ell\in[\mHat]
     &
     \\
     &
     \xHat(\ell,\ell') \geq \muHat(\ell) - \distanceHat(\ell')
     &
     \ell,\ell'\in[\mHat],\permu(\ell) \leq \permu(\ell')
     \\
     &
     \xHat(\ell,\ell') \geq \muHat(\ell') - \distanceHat(\ell')
     &
     \ell,\ell'\in[\mHat],\permu(\ell) > \permu(\ell')
     \\
    \langle\frcfive\rangle
     &
     \costHat\geq 0, \dualapproxHat\geq 0
     &&
     \\
    \langle\frcsix\rangle
     &
     \muHat(\ell) \geq 0, 
     \distanceHat(\ell)\geq 0,
     \distanceHatStar(\ell) \geq 0
     &
     \ell\in[\mHat]
     &
     \\
     &
     \xHat(\ell,\ell') \geq 0
     &
     \ell,\ell'\in[\mHat]
    \end{array}
\end{align*}

\paragraph{Removing parameter $\singlecountedgesetHat$}
Program~\ref{eq:factor revealing program 1}
parameterized by $\mHat,\singlecountedgesetHat,\doublecountedgesetHat,\permu$
is at most program~\ref{eq:factor revealing program 2}
parameterized by $\mHat,\permu$.

\begin{align*}
\label{eq:factor revealing program 2}
\tag{$\mathcal{P}_{\texttt{FR-2}}$}
    \arraycolsep=5.4pt\def\arraystretch{1}
    &\begin{array}{clll}
    \max\limits_{\substack{\costHat,
    \{\xHat(\ell,\ell')\}_{\ell,\ell'\in[\mHat]}
    \\
    \{\muHat(\ell),\distanceHat(\ell),
\distanceHatStar(\ell)\}_{\ell\in[\mHat]}}} &
     \displaystyle\sum\nolimits_{\ell\in[\mHat]}
     2\muHat(\ell) - \distanceHatStar(\ell)
    & \text{s.t.} & \\
    \langle\frcone\rangle
    & 
    \muHat(\ell') \leq \distanceHatStar(\ell) 
    + \distanceHat(\ell) + \distanceHat(\ell')
     & 
     \ell,\ell'\in[\mHat], \ell < \ell'
     &
     \\
    \langle\frctwo\rangle
     &
     \displaystyle\sum\nolimits_{\ell'\in[\ell:\mHat]}
     \xHat(\ell,\ell')
     \leq 
     \costHat
     &
     \ell\in[\mHat]
     &
     \\
    \langle\frcthree\rangle
     &
     \costHat 
     +
     \displaystyle\sum\nolimits_{\ell\in[\mHat]}
     \distanceHat(\ell)
     \leq 1
     &
     \\
    \langle\frcfour\rangle
     &
     \distanceHatStar(\ell) \leq \muHat(\ell)
     &
     \ell\in[\mHat]
     &
     \\
     &
     \xHat(\ell,\ell') \geq \muHat(\ell) - \distanceHat(\ell')
     &
     \ell,\ell'\in[\mHat],\permu(\ell) \leq \permu(\ell')
     \\
     &
     \xHat(\ell,\ell') \geq \muHat(\ell') - \distanceHat(\ell')
     &
     \ell,\ell'\in[\mHat],\permu(\ell) > \permu(\ell')
     \\
    \langle\frcfive\rangle
     &
     \costHat\geq 0, \dualapproxHat\geq 0
     &&
     \\
    \langle\frcsix\rangle
     &
     \muHat(\ell) \geq 0, 
     \distanceHat(\ell)\geq 0,
     \distanceHatStar(\ell) \geq 0
     &
     \ell\in[\mHat]
     &
     \\
     &
     \xHat(\ell,\ell') \geq 0
     &
     \ell,\ell'\in[\mHat]
    \end{array}
\end{align*}
\end{comment}

\begin{comment}
\paragraph{Upper-bound with relaxed program}
Let $\permu_I$ be the identity permutation,
Program~\ref{eq:factor revealing program 2}
parameterized by $\mHat,\permu_I$
is at most Program~\ref{eq:factor revealing program 3}
parameterized by $\mHat$.

\begin{align*}
\label{eq:factor revealing program 3}
\tag{$\mathcal{P}_{\texttt{FR-3}}$}
    \arraycolsep=5.4pt\def\arraystretch{1}
    &\begin{array}{clll}
    \max\limits_{\substack{\costHat,
    \{\xHat(\ell,\ell')\}_{\ell,\ell'\in[\mHat]}
    \\
    \{\muHat(\ell),\distanceHat(\ell),
\distanceHatStar(\ell)\}_{\ell\in[\mHat]}}} &
     \displaystyle\sum\nolimits_{\ell\in[\mHat]}
     2\muHat(\ell) - \distanceHatStar(\ell)
    & \text{s.t.} & \\
    \langle\frcone\rangle
    & 
    \muHat(\ell') \leq \distanceHatStar(\ell) 
    + \distanceHat(\ell) + \distanceHat(\ell')
     & 
     \ell,\ell'\in[\mHat], \ell < \ell',
     \ell\not= 1
     &
     \\
    \langle\frctwo\rangle
     &
     \displaystyle\sum\nolimits_{\ell'\in[\ell+1:\mHat]}
     \xHat(\ell,\ell')
     \leq 
     \costHat
     &
     \ell\in[\mHat]
     &
     \\
    \langle\frcthree\rangle
     &
     \costHat 
     +
     \displaystyle\sum\nolimits_{\ell\in[\mHat]}
     \distanceHat(\ell)
     \leq 1
     &
     \\
    \langle\frcfour\rangle
     &
     \distanceHatStar(\ell) \leq \muHat(\ell)
     &
     \ell\in[\mHat]
     &
     \\
     &
     \xHat(\ell,\ell') \geq \muHat(\ell) - \distanceHat(\ell')
     &
     \ell,\ell'\in[\mHat],\ell \leq \ell'
     \\
    \langle\frcfive\rangle
     &
     \costHat\geq 0, \dualapproxHat\geq 0
     &&
     \\
    \langle\frcsix\rangle
     &
     \muHat(\ell) \geq 0, 
     \distanceHat(\ell)\geq 0,
     \distanceHatStar(\ell) \geq 0
     &
     \ell\in[\mHat]
     &
     \\
     &
     \xHat(\ell,\ell') \geq 0
     &
     \ell,\ell'\in[\mHat]
    \end{array}
\end{align*}

\newcommand{\nHat}{\hat{n}}
\newcommand{\qHat}{\hat{q}}
\newcommand{\muHatPrimed}{\muHat\primed}
\newcommand{\distanceHatPrimed}{\distanceHat\primed}
\newcommand{\distanceHatStarPrimed}{\distanceHatStar\primed}
\newcommand{\naturals}{\mathbb{N}}

\subsection{Approach II: Towards $>$ 3.55-Approximation}

Fixing a parameter $\mHat$,
the worst objective value of Program~\ref{eq:factor revealing program 2} over all permutation $\permu$ 
is upperbounded by 
the worst objective value of Program~\ref{eq:factor revealing program loss}
parameterized by $\nHat$ and $\mHat$ over all $\nHat\in[\mHat]$.
\begin{align*}
\label{eq:factor revealing program loss}
\tag{$\mathcal{P}_{\texttt{FR-Loss}}$}
    \arraycolsep=5.4pt\def\arraystretch{1}
    &\begin{array}{clll}
    \max\limits_{\substack{\costHat,
    \{\qHat(\ell)\}_{\ell\in[\nHat]}
    \\
    \{\muHat(\ell),\distanceHat(\ell),
\distanceHatStar(\ell)\}_{\ell\in[\nHat]}\\
 \{\muHatPrimed(\ell),\distanceHatPrimed(\ell)\}_{\ell\in[\nHat]}}} &
     \displaystyle\sum\nolimits_{\ell\in[\nHat]}
     2\muHat(\ell) - \distanceHatStar(\ell)
     +
     2\qHat(\ell)\cdot \muHatPrimed(\ell)
    & \text{s.t.} & \\
    \langle\frcone\rangle
    & 
    \muHat(\ell') \leq \distanceHatStar(\ell) 
    + \distanceHat(\ell) + \distanceHat(\ell')
     & 
     \ell,\ell'\in[\nHat], \ell < \ell'
     &
     \\
    \langle\frcone\primed\rangle
    & 
    \muHatPrimed(\ell') \leq \distanceHatStar(\ell) 
    + \distanceHat(\ell) + \distanceHatPrimed(\ell')
     & 
     \ell,\ell'\in[\nHat], \ell \leq \ell'
     &
     \\
    \langle\frctwo\rangle
     &
     \displaystyle\sum\nolimits_{\ell'\in[\ell + 1:\nHat]}
    %  \left(
     \plus{\muHat(\ell) - \distanceHat(\ell')}
     +
     \qHat(\ell')\cdot
     \plus{\muHat(\ell) - \distanceHatPrimed(\ell')}
    %  \right)
     & \\
     &\qquad\qquad\qquad
     +
     \plus{\muHat(\ell) - \distanceHat(\ell)}
     +
     \qHat(\ell)\cdot
     \plus{\muHatPrimed(\ell) - \distanceHatPrimed(\ell)}
     \leq 
     \costHat
     &
     \ell\in[\nHat]
     &
     \\
    \langle\frcthree\rangle
     &
     \costHat 
     +
     \displaystyle\sum\nolimits_{\ell\in[\nHat]}
     \distanceHat(\ell)
     +
     \qHat(\ell)\cdot\distanceHatPrimed(\ell)
     \leq 1
     &
     \\
    \langle\frcfour\rangle
     &
     \distanceHatStar(\ell) \leq \muHat(\ell)
     &
     \ell\in[\nHat]
     &
     \\
     &
     \muHat(\ell - 1) \leq \muHatPrimed(\ell) \leq \muHat(\ell) 
     &
     \ell\in[\nHat]
     \\
    \langle\frcfive\rangle
     &
     \costHat\geq 0
     &&
     \\
    \langle\frcsix\rangle
     &
     \muHat(\ell) \geq 0, 
     \distanceHat(\ell)\geq 0,
     \distanceHatStar(\ell) \geq 0,
     \muHatPrimed(\ell) \geq 0,
     \distanceHatPrimed(\ell) \geq 0
     &
     \ell\in[\nHat]
     &
     \\
     &
     \qHat(\ell) \in \naturals
     &
     \ell\in[\nHat]
     \\
     &
     \sum_{\ell\in[\nHat]}
     1 + \qHat(\ell) = \mHat
     &
    \end{array}
\end{align*}

In Program~\ref{eq:factor revealing program 2}
we need to enumerate over all possible permutations,
which indicates the order of $\{\muHat(\ell)\}$.
In contrast, 
Program~\ref{eq:factor revealing program loss}
specifies the order over $\{\muHat(\ell),\muHat\primed(\ell)\}$,
i.e., $\muHat(\ell - 1) \leq \muHatPrimed(\ell) \leq \muHat(\ell)$,
but it still needs to search $\{\qHat(\ell)\}$
subject to constraint $ \sum_{\ell\in[\nHat]}
     1 + \qHat(\ell) = \mHat$.
     Based on the numerically evaluation, 
     for $\mHat = 20$, its objective value is than 3.55.
     
     
     
\newpage

     
\subsection{Counterexample for Induction Argument}

We want to use an induction argument to show 
the worst objective value of program below is achieved 
with monotone $\{\muHat(\ell)\}$,
i.e., $\muHat(1) \leq \muHat(2) \leq \dots \leq \muHat(\mHat)$.
\begin{align*}
\label{eq:factor revealing program 0}
\tag{$\mathbb{P}_{\texttt{FR-O}}$}
    \arraycolsep=5.4pt\def\arraystretch{1}
    &\begin{array}{clll}
    \max\limits_{\substack{\costHat\\
    \{\muHat(\ell),\distanceHat(\ell),
\distanceHatStar(\ell)\}_{\ell\in[\mHat]}}} &
     \displaystyle\sum\nolimits_{\ell\in[\mHat]}
     2\muHat(\ell) - \distanceHatStar(\ell)
    & \text{s.t.} & \\
    \langle\frcone\rangle
    & 
    \muHat(\ell') \leq \distanceHatStar(\ell) 
    + \distanceHat(\ell) + \distanceHat(\ell')
     & 
     \ell,\ell'\in[\mHat], \ell < \ell'
     &
     \\
    \langle\frctwo\rangle
     &
     \displaystyle\sum\nolimits_{\ell'\in[\ell:\mHat]}
     \plus{\min\{\muHat(\ell),\muHat(\ell')\} - 
     \distanceHat(\ell')}
     \leq 
     \costHat
     &
     \ell\in[\mHat]
     &
     \\
    \langle\frcthree\rangle
     &
     \costHat 
     +
     \displaystyle\sum\nolimits_{\ell\in[\mHat]}
     \distanceHat(\ell)
     \leq 1
     &
     \\
    \langle\frcfour\rangle
     &
     \distanceHatStar(\ell) \leq \muHat(\ell)
     &
     \ell\in[\mHat]
     &
     \\
    \langle\frcfive\rangle
     &
     \costHat\geq 0
     &&
     \\
    \langle\frcsix\rangle
     &
     \muHat(\ell) \geq 0, 
     \distanceHat(\ell)\geq 0,
     \distanceHatStar(\ell) \geq 0
     &
     \ell\in[\mHat]
     &
    \end{array}
\end{align*}

In the inductive step, we want to set all variables related to $\ell = 1$
(i.e., $\{\muHat(1), \distanceHat(1), \distanceHatStar(1)\}$)
as some constants, and argue that 
the new program with only variables ($\costHat$,
$\{\muHat(\ell),\distanceHat(\ell),
\distanceHatStar(\ell)\}_{\ell=2,\dots \mHat}$)
achieves its worst objective value with monotone 
$\{\muHat(\ell)\}_{\ell=2,\dots \mHat}$.

Here we give a counterexample with $\mHat = 4$.
% Suppose $\mHat = 4$. 
Let 
\begin{align*}
    \muHat(1) \gets \frac{3}{9}, 
    \qquad 
    \distanceHat(1) \gets \frac{2}{9},
    \qquad 
    \distanceHatStar(1) \gets 0
\end{align*}
The unique worst solution for the optimization program with 
remaining variables ($\costHat$, $\{\muHat(\ell),\distanceHat(\ell),
\distanceHatStar(\ell)\}_{\ell=2,3,4}$)~is 
\begin{align*}
    &\costHat =  \frac{2}{9} \\
    &\muHat(2) =  \frac{3.5}{9} \qquad \distanceHat(2) = \frac{2}{9}
    \qquad \distanceHatStar(2) = 0 \\
    &\muHat(3) =  \frac{5}{9} \qquad \distanceHat(3) = \frac{3}{9}
    \qquad \distanceHatStar(3) = 0 \\
    &\muHat(4) =  0 \qquad \distanceHat(4) = 0
    \qquad \distanceHatStar(4) = 0 \\
\end{align*}

\subsection{Optimal Solution under a Relaxed Objective Has 
Ordered $\muHat(\cdot)$ for $\mHat = 2$}

In this subsection, we consider a relaxed program of \ref{eq:factor revealing program 0}
where we replace its objective function
with $\sum_{\ell\in[\mHat]} 2\muHat(\ell)$.

Here we show that when $\mHat = 2$,
the optimal solution in
program~\ref{eq:factor revealing program 0}
has $\muHat(1) \leq \muHat(2)$.
We use the following two-step argument.

\begin{claim}
For any $\mHat$,
there exists an optimal solution of program~\ref{eq:factor revealing program 0}
satisfying that 
$\muHat(\ell) \geq \distanceHat(\ell)$
for every $\ell\in[\mHat]$.
\end{claim}
\begin{proof}
For any feasible solution of program~\ref{eq:factor revealing program 0}.
Suppose $\muHat(\ell) < \distanceHat(\ell)$
for some $\ell\in[\mHat]$.
We can construct a new solution,
where we set $\muHat'(\ell) \gets \distanceHat(\ell)$, while holding 
all other variable assignments fixed.
It is straightforward to verify that all constraints are satisfied and the objective value increases,
which concludes the proof.
\end{proof}

\begin{claim}
For $\mHat = 2$,
there exists an
optimal solution of program~\ref{eq:factor revealing program 0}
satisfying that 
$\muHat(1) \leq \muHat(2)$.
\end{claim}
\begin{proof}
Suppose 
there exists an
optimal solution of program~\ref{eq:factor revealing program 0}
satisfying that 
$\muHat(1) > \muHat(2)$.
Below we discuss how to construct an optimal solution with 
$\muHat(1) \leq \muHat(2)$.

By Claim A.1 and the assumption
that $\muHat(1) > \muHat(2)$,
constraint \frcfour\ 
with $\ell = 1$
can be written as $\muHat(1) - \distanceHat(1) + \muHat(2) - \distanceHat(2) \leq \costHat$.

Now we can construct a new solution for 
program~\ref{eq:factor revealing program 0}
with $\mHat' = 1$ as follows:
let $\costHat' \gets \costHat$,
$\muHat'(1) \gets \muHat(1) + \muHat(2)$,
$\distanceHat'(1) \gets \distanceHat(1) + \distanceHat(2)$,
$\distanceHatStar'(1) \gets \distanceHatStar(1) + \distanceHatStar(2)$.
It is straightforward to verify that 
the constructed solution is feasible and has 
the same objective value as the original solution.

Thus, the optimal objective value of 
program~\ref{eq:factor revealing program 0}
with $\mHat' = 1$ is weakly larger than 
the optimal objective value of 
program~\ref{eq:factor revealing program 0}
with $\mHat = 2$.

To finish the proof, note that 
for any optimal solution in program~\ref{eq:factor revealing program 0}
with $\mHat' = 1$,
we can duplicate and halve each variables $\muHat, \distanceHat,\distanceHatStar$.
As a consequence, we obtain a feasible solution
in program~\ref{eq:factor revealing program 0}
with $\mHat = 2$
such that $\muHat(1) = \muHat(2)$
and its objective value equals to the optimal objective value of program~\ref{eq:factor revealing program 0}
with $\mHat' = 1$.
\end{proof}

\subsection{An Additional Constraint Added to Factor Revealing Program}

Consider the assignment construction in 
Step 3.1 on page 7. We note that 
the constructed assignment also satisfies the following inequality:
\begin{align*}
    \sum_{\ell'\in[\mHat]: \muHat(\ell') \geq \muHat(\ell)}
    \plus{\muHat(\ell) - \distanceHat(\ell')}
    +
    \sum_{\ell'\in[\ell + 1:\mHat]:
    \muHat(\ell') < \muHat(\ell)}
    \plus{\muHat(\ell') - \distanceHat(\ell')}
    \leq c
\end{align*}
The argument is similar to the argument of verifying the feasibility of the constructed assignment for constraint \frctwo.


\newpage

\end{comment}
\input{Notes/factor-revealing-quad-program}

==> Notes/factor-revealing-quad-program.tex <==
\subsection{Strongly Factor Revealing Quadratic Program}

Consider the following program parameterized by 
$\nHat\in\naturals$
with variables 
    $\{\qHat(a, b), \muHat(a, b),\distanceHat(a, b),
\distanceHatStar(a, b)\}_{a\in[\nHat], b \in [a]}$
and $\costHat$:
\begin{align*}
% \label{eq:strongly factor-revealing quadratic program}
% \tag{$\mathcal{P}_{\texttt{FR-Quad}}(\nHat)$}
    \arraycolsep=5.4pt\def\arraystretch{1}
    &\begin{array}{clll}
    \max &
     \displaystyle\sum\nolimits_{a\in[\nHat]}
     \displaystyle\sum\nolimits_{b \in[a]}
     \qHat(a,b)\cdot 
    \left(2\muHat(a,b) - \distanceHatStar(a,b)\right)
    & \text{s.t.} & \\
    (i) &
    \muHat(a, b) \leq \muHat(a', b')
    &
    a, a'\in[\nHat],
    b\in[a], b'\in[a'], b < b'
    \\
    (ii) &
    \muHat(a', b') \leq 
    \distanceHatStar(a, b) + \distanceHat(a, b)
    +
    \distanceHat(a', b')
    &
    a,a'\in[\nHat],
    b\in[a], b'\in[a'],
    a < a'
    &
    \\
    (iii.1) &
    \distanceHat(a, b) \leq \muHat(a, b)
    &
    a\in[\nHat],
    b\in[a]
    \\
    (iii.2) &
    \distanceHatStar(a, b) \leq \muHat(a, b)
    &
    a\in[\nHat],
    b\in[a]
    \\
    (iv) &
    \displaystyle\sum\nolimits_{a' \in [a + 1:\nHat]}
    \displaystyle\sum\nolimits_{b' \in [a]}
    \qHat(a',b')\cdot \plus{\muHat(a', b') - \distanceHat(a',b')}
    &
    \\
    &
    +\displaystyle\sum\nolimits_{a' \in [a+1:\nHat]}
    \displaystyle\sum\nolimits_{b' \in [a + 1:a']}
    \qHat(a',b')\cdot \plus{\muHat(a, a) - \distanceHat(a',b')}
    \leq \costHat
    &
    a\in[\nHat - 1]
    \\
    % (iv.2) &
    % \displaystyle\sum\nolimits_{a' \in [a:\nHat]}
    % \displaystyle\sum\nolimits_{b' \in [a - 1]}
    % \qHat(a',b')\cdot \plus{\muHat(a', b') - \distanceHat(a',b')}
    % &
    % \\
    % &
    % +\displaystyle\sum\nolimits_{a' \in [a:\nHat]}
    % \displaystyle\sum\nolimits_{b' \in [a:a']}
    % \qHat(a',b')\cdot \plus{\muHat(a, a - 1) - \distanceHat(a',b')}
    % \leq \costHat
    % &
    % a\in[2:\nHat]
    %  \\
     (v) &
     \costHat 
     +
     \displaystyle\sum\nolimits_{a\in[\nHat]}
     \displaystyle\sum\nolimits_{b \in[a]}
     \qHat(a,b)\cdot \distanceHat(a,b)
     \leq 1
     &
     \\
     (vi) &
     \displaystyle\sum\nolimits_{a = [b:\nHat]}
     \qHat(a, b) = 1
     &
     b\in[\nHat]
     \\
     (vii)&
     \costHat\geq 0,
     \qHat(a, b) \geq 0,
     \muHat(a,b) \geq 0,
     \distanceHat(a, b) \geq 0,
     \distanceHatStar(a, b) \geq 0
     &
     a\in[\nHat],b\in[a]
    \end{array}
\end{align*}
% 
% 
% \begin{remark}
Here we provide some intuitions on the necessity of 
each constraint in program~\ref{eq:strongly factor-revealing quadratic program} by illustrating that 
its optimal objective value 
is constant (i.e., upperbounded by $12$) when $\nHat = 2$.
\begin{enumerate}
    \item[(a)] Constraint (iv) at $a = 1$ implies 
    $\qHat(2, 2) \cdot (\muHat(1, 1) - \distanceHat(2, 2)) \leq \costHat$.
    Combining with constraint (v) and constraint (vi) at $b = 2$,
    we have $\muHat(1, 1) \leq 1$.
    \item[(b)] Constraint (ii) at $a = 1, a' = 2, b = 1, b' = 2$,
    and constraints (iii.1) (iii.2) at $a = 1, b = 1$ imply
    that 
    $\muHat(2, 2) \leq \distanceHatStar(1, 1) + \distanceHat(1, 1) + \distanceHat(2, 2) \leq 2 + \distanceHat(2, 2)$.
    Combining with constraint (v) and constraint (vi) at $b = 2$,
    we have $\distanceHat(2, 2) \leq 1$ and thus $\muHat(2, 2) \leq 3$.
    \item[(c)] Constraint (i) at $a = 2, b = 1, a' = 2, b'= 2$
    implies that $\muHat(2, 1) \leq \muHat(2, 2) = 3$.
    \item [(d)] Combining step (a)-(c) and constraint (vi),
    the objective value is upperbounded by 12.\footnote{In fact, we numerically verify (using Gurobi) that $\rm{\texttt{OBJ}}\left[\text{\hyperref[eq:strongly factor-revealing quadratic program]{$\mathcal{P}_{\texttt{FR-Quad}}(2)$}}\right] = 6$.}
\end{enumerate}
% We start by showing that $\muHat(1, 1) \leq 1$ for any feasible solution.

% first show that for any feasible solution $\muHat(1, 1) \leq 1$,
% $\muHat(2, 1) \leq 3$, $\muHat(2, 2) \leq 3$.

% \end{remark}

\newcommand{\xHat}{\hat{x}}

Note that we can introduce non-negative variables 
$\{\xHat(a, a',b')\}$ 
% $\{\xHat(a, a',b),\yHat(a,a', b)\}$ 
to handle 
$\plus{\cdot}$ operator in constraint (iv).
% (iv.2). 
In this case, program \ref{eq:strongly factor-revealing quadratic program} is a non-convex optimization program with 
quadratic objective and quadratic constraints,
which we can numerically solved (using Gurobi).



\begin{theorem}
\label{thm:strongly factor-revealing quadratic program}
The approximation ratio of \Cref{alg:greedy modified}
is upperbounded by $\rm{\texttt{OBJ}}\left[\text{\ref{eq:strongly factor-revealing quadratic program}}\right]$
% \begin{align*}
%     \max_{\nHat\in\naturals:\theta(\nHat - 1) \leq 1 \leq \theta(2\nHat- 1)}~
%     \rm{\texttt{OBJ}}\left[\text{\ref{eq:strongly factor-revealing quadratic program}}\right]
% \end{align*}
for every $\nHat \in \naturals$.
\end{theorem}


\begin{lemma}
We numerically verify (using Gurobi) that
$\rm{\texttt{OBJ}}\left[\text{\hyperref[eq:strongly factor-revealing quadratic program]{$\mathcal{P}_{\texttt{FR-Quad}}(50)$}}\right] \leq 3.103$.
\end{lemma}

\begin{corollary}
The approximation of \Cref{alg:greedy modified} is at most 3.103.
\end{corollary}

Below, we discuss the proof of \Cref{thm:strongly factor-revealing quadratic program}. 



Following in discussion in the main text and Appendix A.1, the 
approximation of \Cref{alg:greedy modified}
is upperbouned by
\begin{align*}
    \sup_{\mHat\in\naturals}
    \rm{\texttt{OBJ}}\left[\text{\ref{eq:factor revealing program original}}\right]
\end{align*}
where program \ref{eq:factor revealing program original} parameterized by $\mHat \in\naturals$ 
is 
\begin{align*}
\label{eq:factor revealing program original}
\tag{$\mathcal{P}_{\texttt{FR-0}}(\mHat)$}
    \arraycolsep=5.4pt\def\arraystretch{1}
    &\begin{array}{clll}
    \max\limits_{\substack{\costHat,\\ \{\muHat(\ell),\distanceHat(\ell),
\distanceHatStar(\ell)\}_{\ell\in[\mHat]}}} &
    \displaystyle\sum\nolimits_{\ell\in[\mHat]}
     2\muHat(\ell) - \distanceHatStar(\ell)
    & \text{s.t.} & \\
    \langle\frcone\rangle
    & 
    \muHat(\ell') \leq \distanceHatStar(\ell) 
    + \distanceHat(\ell) + \distanceHat(\ell')
     & 
     \ell,\ell'\in[\mHat], \ell < \ell'
     &
     \\
    \langle\frctwo\rangle
     &
     \displaystyle\sum\nolimits_{\ell'\in[\ell:\mHat]}
     \plus{\min\{\muHat(\ell),\muHat(\ell')\} - 
     \distanceHat(\ell')}
     \leq 
     \costHat
     &
     \ell\in[\mHat]
     &
     \\
    \langle\frcthree\rangle
     &
     \costHat 
     +
     \displaystyle\sum\nolimits_{\ell\in[\mHat]}
     \distanceHat(\ell)
     \leq 1
     &
     \\
    \langle\frcfour\rangle
     &
     \distanceHatStar(\ell) \leq \muHat(\ell)
     &
     \ell\in[\mHat]
     &
     \\
    \langle\frcfive\rangle
     &
     \costHat\geq 0,
     \muHat(\ell) \geq 0, 
     \distanceHat(\ell)\geq 0,
     \distanceHatStar(\ell) \geq 0
     &
     \ell\in[\mHat]
     &
    \end{array}
\end{align*}

Fix an arbitrary $\mHat \in \naturals$.
Suppose $(\costHat, \{\muHat(\ell), \distanceHat(\ell),\distanceHatStar(\ell)\})$
is an arbitrary feasible solution of program~\ref{eq:factor revealing program original}.
Next we show that for all $\nHat\in\naturals$,
we can convert this feasible solution $(\costHat, \{\muHat(\ell), \distanceHat(\ell),\distanceHatStar(\ell)\})$
of program~\ref{eq:factor revealing program original}
into a feasible solution 
$(\costHat, \{\qHat(a, b), \muHat(a, b),\distanceHat(a, b),
\distanceHatStar(a, b)\})$
in program~\ref{eq:strongly factor-revealing quadratic program} with weakly higher objective value.
Thus, for every $\mHat\in\naturals$, $\nHat\in\naturals$,
$\rm{\texttt{OBJ}}\left[\text{\ref{eq:factor revealing program original}}\right] \leq \rm{\texttt{OBJ}}\left[\text{\ref{eq:strongly factor-revealing quadratic program}}\right]$,
which  proves \Cref{thm:strongly factor-revealing quadratic program}.\footnote{We numerically verify 
(using Gurobi) that $\rm{\texttt{OBJ}}\left[\text{\hyperref[eq:factor revealing program original]{$\mathcal{P}_{\texttt{FR-0}}(500)$}}\right] \geq 3.073$. 
We conjecture that $\sup_{\mHat\in\naturals}\rm{\texttt{OBJ}}\left[\text{\ref{eq:factor revealing program original}}\right] =
\inf_{\nHat\in\naturals}\rm{\texttt{OBJ}}\left[\text{\ref{eq:strongly factor-revealing quadratic program}}\right]$.}

First, we claim that it is without loss of generality to assume that the feasible solution $(\costHat, \{\muHat(\ell), \distanceHat(\ell),\distanceHatStar(\ell)\})$
satisfies $\distanceHat(\ell) \leq \muHat(\ell)$ for every $\ell\in[\mHat]$.

\begin{claim}
\label{claim:distance upperbound}
For any $\mHat\in\naturals$ and any feasible solution $(\costHat, \{\muHat(\ell), \distanceHat(\ell),\distanceHatStar(\ell)\})$
of program~\ref{eq:factor revealing program original},
there exists $\mHat\primed \in\naturals$ and 
a feasible solution $(\costHat\primed, \{\muHat\primed(\ell), \distanceHat\primed(\ell),\distanceHatStar\primed(\ell)\})$
of program~\hyperref[eq:factor revealing program original]{$\mathcal{P}_{\texttt{FR-0}}(\mHat\primed)$}
such that $\distanceHat\primed(\ell)\leq \muHat\primed(\ell)$
for every $\ell\in[\mHat\primed]$ and 
has weakly higher objective value.
\end{claim}
\begin{proof}
We explicitly construct $\mHat\primed$ and $(\costHat\primed, \{\muHat\primed(\ell), \distanceHat\primed(\ell),\distanceHatStar\primed(\ell)\})$
from $\mHat$ and $(\costHat, \{\muHat(\ell), \distanceHat(\ell),\distanceHatStar(\ell)\})$.

Let $\ell^*$ be the index with largest $\muHat(\ell)$,
i.e., $\ell^*= \argmax_{\ell\in[\mHat]} \muHat(\ell)$.
If $\distanceHat(\ell^*) > \muHat(\ell^*)$,
then we can re-set $\muHat(\ell^*) \gets \distanceHat(\ell^*)$, and ensures that (i) the solution is
still feasible in 
program~\ref{eq:factor revealing program original} 
(in particular, constraints \frcone, \frctwo\ 
are still satisfied), and has higher objective value.

Now, we partition index set $[\mHat]$ into two subsets:
$\Delta = \{\ell\in[\muHat]: \distanceHat(\ell) 
\leq \muHat(\ell)\}$ and 
$\bar \Delta = [\mHat]\backslash \Delta$.
As we discussed in the previous paragraph,
we can assume $\ell^* \in \Delta$.
Let $\mHat\primed \gets |\Delta|$, 
$\costHat\primed\gets \costHat$,
and assign $\{\muHat\primed(\ell), \distanceHat\primed(\ell),
\distanceHatStar\primed(\ell)\}_{\ell\in[\mHat\primed]} 
\gets 
\{\muHat(\ell), \distanceHat(\ell),\distanceHatStar(\ell)\}_{
\ell\in\Delta}$ (in the same index order).
Suppose index $\ell^{*\dagger}\in[\mHat\primed]$ 
receives assignment of index $\ell^*\in[\mHat]$.
We further increases 
$\muHat\primed(\ell^{*\dagger}) 
\gets 
\muHat\primed(\ell^{*\dagger}) + 
\sum_{\ell\in\bar\Delta}\distanceHat(\ell)$,
and
$\distanceHat\primed(\ell^{*\dagger}) 
\gets 
\distanceHat\primed(\ell^{*\dagger}) + 
\sum_{\ell\in\bar\Delta}\distanceHat(\ell)$.
It is straightforward to verify that 
the constructed solution is feasible in 
program~\hyperref[eq:factor revealing program original]{$\mathcal{P}_{\texttt{FR-0}}(\mHat\primed)$},
and its objective value is weakly higher.
\end{proof}

Due to \Cref{claim:distance upperbound},
in the remaining of the discussion, we assume $\distanceHat(\ell) \leq \muHat(\ell)$ for every $\ell\in[\mHat]$.

\newcommand{\ptr}{\texttt{ptr}}

Let $L\subseteq[\mHat]$ be a subset of index  
constructed as follows,
\begin{enumerate}
    \item Initialize $L \gets \emptyset$,
    $\ptr \gets \mHat$.
    \item While $\ptr > 0$ do
    \begin{enumerate}
        \item find $\ell\primed \gets \argmax_{\ell \in [1:\ptr]}
        \muHat(\ell)$ 
        <tie-breaking towards smaller index>
        \item update $L \gets L \cup\{\ell\primed\}$,
        $\ptr \gets \ell\primed - 1$
    \end{enumerate}
\end{enumerate}
Let $n\triangleq |L|$.
In the construction of set $L$,
we first add the 
index $\ell_{n}$ with the largest $\muHat(\ell)$, then add
the index $\ell_{n - 1}$ with the largest $\muHat(\ell)$ between 
from
$\ell\in[1,\ell_n - 1]$, add $\ell_{n - 2}$ with the largest $\muHat(\ell)$ between 
from
$\ell\in[1,\ell_{n - 1} - 1]$,
and keep repeating until index $1$ is added into $L$
as $\ell_{1}$.\footnote{For example, 
suppose $\mHat = 10$ and $\muHat(\ell)$
takes value 3, 5, 4, 2, 5, 6, 8, 9, 1, 6;
then $L = \{1, 2, 6, 7, 8\}$.}
% See a graphical example illustration in Figure XYZ.
Below, we add subscript $a$ to all indexes in set $L$,
i.e., $L=  \{\ell_a\}_{a\in[n]}$, where $\ell_a$ is increasing in $a$.\footnote{Here we add 
subscript $a$ to
index $\ell$ to indicate the construction (formally defined later) of
partial solution 
$\{\qHat(a, b), \muHat(a, b),\distanceHat(a, b),
\distanceHatStar(a, b)\}$ with index $(a, b)$
in 
program~\ref{eq:strongly factor-revealing quadratic program}.}
For ease of presentation, we further introduce dummy $\ell_0 = 0$ and $\ell_{n + 1} = \mHat + 1$.



We make the following claim about 
the feasible solution $(\costHat, \{\muHat(\ell), \distanceHat(\ell),\distanceHatStar(\ell)\})$
as well as set $L$ constructed above.

\begin{claim}
\label{claim:2d monotonicity}
For any adjacent $\ell_a, \ell_{a+1}\in L$,
we have 
and $\mu(\ell) < \muHat(\ell_a) < \muHat(\ell_{a+1})$ 
for every $\ell\in[\ell_a + 1:\ell_{a+1} - 1]$.
Similarly, $\muHat(\ell) < \muHat(\ell_n)$
for every $\ell\in[\ell_n + 1: \mHat]$.
\end{claim}
\begin{proof}
The claim holds due to the construction of set $L$.
Suppose $\muHat(\ell) \geq \muHat(\ell_{n})$
for some $\ell\in [\ell_n + 1: \mHat]$,
the construction of set $L$ implies that $\ell\in L$,
which leads to a contradiction.
The remaining guarantees in the claim statement can be verified similarly.
\end{proof}

In the remaining of the discussion, 
we proceed 
with the following two-step approach:
First, we construct 
a solution 
$(\costHat, \{\qHat(a, b), \muHat(a, b),\distanceHat(a, b),
\distanceHatStar(a, b)\})$
which satisfies constraints (i), (ii), (iii.1), (iii.2),
(v), (vii) 
of program~\hyperref[eq:strongly factor-revealing quadratic program]{$\mathcal{P}_{\texttt{FR-Quad}}(n)$},
as well as constraint (iv.0)
which is a stronger version of
% \footnote{Constraint (iv.0) is clearly stronger than constraint (iv),
% and is also stronger than constraint (iv.2) when 
% constraint (i.2) is satisfied.} 
% than (iv.1) (iv.2) 
constraint (iv) defined as follows,
\begin{align*}
    (iv.0) \qquad
    &\sum_{a' \in [a:\nHat]}
    \sum_{b' \in [a]}
    \qHat(a',b')\cdot \plus{\muHat(a', b') - \distanceHat(a',b')}
    \\
    &\qquad 
    +\sum_{a' \in [a:\nHat]}
    \sum_{b' \in [a + 1:a']}
    \qHat(a',b')\cdot \plus{\muHat(a, a) - \distanceHat(a',b')}
    \leq \costHat
    \qquad 
    a\in[n]
\end{align*}
Second, we use a ``stretch then compress'' argument
to further modify this solution into a feasible solution 
of program program~\ref{eq:strongly factor-revealing quadratic program}
with any targeted $\nHat\in\naturals$ as desired.

\paragraph{Step 1.}
In this step, we construct 
a solution 
$(\costHat, \{\qHat(a, b), \muHat(a, b),\distanceHat(a, b),
\distanceHatStar(a, b)\})$
which satisfies 
constraints (i), (ii), (iii.1), (iii.2),
(v), (vii) 
of program~\hyperref[eq:strongly factor-revealing quadratic program]{$\mathcal{P}_{\texttt{FR-Quad}}(n)$}
as well as constraint (iv.0).

For each $a\in[n]$, $b\in[a]$, define set 
$L(a, b)$
be the subset of $[\ell_a: \ell_{a + 1} - 1]$
whose $\muHat(\ell)$ is between $\muHat(\ell_{b-1})$ and 
$\muHat(\ell_b)$,
i.e., 
$L(a,b) = \{
\ell \in [\ell_a: \ell_{a + 1} - 1]:
\muHat(\ell_{b - 1}) < \muHat(\ell) \leq \muHat(\ell_b)
\}$.\footnote{For ease of presentation, we 
add dummy $\muHat(\ell_0) = 0$.}
By \Cref{claim:2d monotonicity}, 
$\{L(a, b)\}_{b\in[a]}$ is a partition of 
$[\ell_a: \ell_{a+1} - 1]$,
and $\{L(a, b)\}_{a\in[n],b\in[a]}$
is a partition of $[\mHat]$.

Briefly speaking, we set $\muHat(a, b)$
(resp.\ $\distanceHat(a, b)$, $\distanceHatStar(a, b)$) 
for each 
% cell\footnote{For distinction, 
% we call $\ell$ ``index'', and $(a, b)$ ``cell''.} 
$(a, b)$
as the average of $\muHat(\ell)$
(resp.\ $\distanceHat(\ell)$, $\distanceHatStar(\ell)$) 
over $\ell\in L(a, b)$.
The formal construction is as follows,
\begin{align*}
    a\in[n], b\in[a],
    |L(a,b)|\geq 1:
    \qquad 
    &\muHat(a, b) \gets 
    \sum_{\ell\in L(a, b)} 
    \frac{
    \muHat(\ell)
    }{
    |L(a,b)|
    },
    \quad
    \distanceHat(a, b) \gets 
    \sum_{\ell\in L(a, b)} 
    \frac{ \distanceHat(\ell)
    }{
    |L(a,b)|
    },
    \\
    &\distanceHatStar(a, b) \gets 
    \sum_{\ell\in L(a, b)} 
    \frac{\distanceHatStar(\ell)
    }{
    |L(a,b)|
    },
    \quad
    \qHat(a, b) \gets |L(a,b)|
    \\
    a\in[n], b\in[a],
    |L(a,b)| = 0:
    \qquad 
    &\muHat(a, b) \gets 
    \muHat(a - 1, b),
    \quad
    \distanceHat(a, b) \gets \distanceHat(a - 1, b),
    \\
    &\distanceHatStar(a, b) \gets \distanceHatStar(a - 1, b),
    \quad
    \qHat(a, b) \gets |L(a,b)|
    \\
    & 
    \costHat\gets \costHat
\end{align*}
Note that $|L(a, a)| \geq 1$ for each $a\in[n]$,\footnote{Note that $\ell_a\in L(a, a)$ by definition.}
and thus the construction (in particular, the part to handle $|L(a, b)| = 0$) is well-defined. 
It is straightforward to verify that 
the constructed solution satisfies 
constraints (i), (ii), (iii.1), (iii.2),
(v), (vii) 
of program~\hyperref[eq:strongly factor-revealing quadratic program]{$\mathcal{P}_{\texttt{FR-Quad}}(n)$}
as well as constraint (iv.0).
For completeness, we verify them one by one.
\begin{enumerate}
    \item[(i)] It is implied by the construction of solution, construction of $L(a, b)$, 
    and \Cref{claim:2d monotonicity}.
    \item[(ii)] It is implied by \frcone\ in
    program~\ref{eq:factor revealing program original}
    and the construction of solution.
    % the fact that taking average of 
    % $\muHat(\cdot),\distanceHat(\cdot),
    % \distanceHatStar(\cdot)$ of
    % indexes $\ell\primed,\ell\doubleprimed$
    % does not violate \frcone \ between
    % this average and $\muHat(\ell'),\distanceHat(\ell'),
    % \distanceHatStar(\ell')$ for every $\ell' < \min\{\ell\primed,\ell\doubleprimed\}$
    % and every $\ell' > \max\{\ell\primed,\ell\doubleprimed\}$.
    % More specifically,
    Specifically,
    for any $a, a'\in[n], b\in[a],b'\in[a']$, 
    $a < a'$, 
    suppose\footnote{The arguments for other cases
    (i.e., 
    $|L(a, b)| = 0$ or $|L(a', b')| = 0$)
    are similar 
    and thus omitted here.} 
    $|L(a, b)| \geq 1$, $|L(a', b')| \geq 1$, then
    we have
    \begin{align*}
        \muHat(a', b') 
        &\overset{(a)}{=} 
        \sum_{\ell'\in L(a', b')} \frac{\muHat(\ell')}{|L(a', b')|}
        \\
        &\overset{(b)}{\leq}
        \sum_{\ell'\in L(a', b')} \left(\frac{1}{|L(a', b')|}
        \sum_{\ell\in L(a, b)} \frac{1}{|L(a, b)|}
        \left(
        \distanceHatStar(\ell) + \distanceHat(\ell) +
        \distanceHat(\ell')
        \right)
        \right)
        \\
        &=
        \sum_{\ell\in L(a, b)} \frac{
        \distanceHatStar(\ell)}{|L(a, b)|}
        +
        \sum_{\ell\in L(a, b)} \frac{
        \distanceHat(\ell)}{|L(a, b)|}
        +
        \sum_{\ell'\in L(a', b')} \frac{\distanceHat(\ell')}{|L(a', b')|}
        \\
        &\overset{(c)}{=}
        \distanceHatStar(a, b) + \distanceHat(a, b) + \distanceHat(a', b')
    \end{align*}
    where equalities~(a) (c) holds due to the solution construction;
    and inequality~(b) holds due to constraint \frcone\ and 
    the construction of $L(a, b), L(a', b')$, which guarantees
    $\ell < \ell'$ for every $\ell\in L(a, b)$, $\ell'\in L(a', b')$.
    \item[(iii.1)] It is implied by \Cref{claim:distance upperbound} and the construction of solution.
    \item[(iii.2)] It is implied by \frcfour\  and the construction of solution.
    \item[(iv.0)]
    It is implied by \frctwo\  and the construction of solution.
    Specifically, 
    for any $a\in[n]$, we have 
    \begin{align*}
        \costHat 
        &\overset{(a)}{\geq} 
         \sum_{\ell'\in[\ell_a:\mHat]}
     \plus{\min\{\muHat(\ell_a),\muHat(\ell')\} - 
     \distanceHat(\ell')}
     \\
    &\overset{(b)}{=} 
     \sum_{a'\in[a:n]}\sum_{b'\in[a']}
     \sum_{\ell'\in L(a', b')}
     \plus{\min\{\muHat(\ell_a),\muHat(\ell')\} - 
     \distanceHat(\ell')}
     \\
    % &\geq
    %  \sum_{a'\in[a + 1:n]}\sum_{b'\in[a']}
    %  \sum_{\ell'\in L(a', b')}
    %  \plus{\min\{\muHat(\ell_a),\muHat(\ell')\} - 
    %  \distanceHat(\ell')}
    %  \\
     &\overset{(c)}{=}
     \sum_{a'\in[a:n]}
     \left(
     \sum_{b'\in[a]}
     \sum_{\ell'\in L(a', b')}
     \plus{\muHat(\ell') - 
     \distanceHat(\ell')}
     +
     \sum_{b'\in[a+1:a']}
     \sum_{\ell'\in L(a', b')}
     \plus{\muHat(\ell_a) - 
     \distanceHat(\ell')}
     \right)
     \\
    & \overset{(d)}{\geq}
    \sum_{a'\in[a:n]}
     \sum_{b'\in[a]}
     |L(a', b')|
     \cdot 
     \plus{
     \sum_{\ell'\in L(a', b')}
     \frac{\muHat(\ell') - \distanceHat(\ell')}
     {|L(a', b')|}
     }
     \\
     &\qquad\qquad 
    +\sum_{a'\in[a:n]}
     \sum_{b'\in[a+1:a']}
     |L(a', b')|
     \cdot 
     \plus{
     \sum_{\ell'\in L(a', b')}
     \frac{\muHat(\ell_a) - \distanceHat(\ell')}
     {|L(a', b')|}
     }
     \\
     &\overset{(e)}{=}
    \sum_{a'\in[a:n]}
     \sum_{b'\in[a]}
     \qHat(a', b')
     \cdot 
     \plus{
     \muHat(a', b') - \distanceHat(a', b')
     }
     \\
     &\qquad\qquad 
    +\sum_{a'\in[a:n]}
     \sum_{b'\in[a+1:a']}
     \qHat(a', b')
     \cdot 
     \plus{
     \muHat(\ell_a) - \distanceHat(a', b')
     }
     \\
     &\overset{(f)}{\geq}
    \sum_{a'\in[a:n]}
     \sum_{b'\in[a]}
     \qHat(a', b')
     \cdot 
     \plus{
     \muHat(a', b') - \distanceHat(a', b')
     }
     \\
     &\qquad\qquad 
    +\sum_{a'\in[a:n]}
     \sum_{b'\in[a+1:a']}
     \qHat(a', b')
     \cdot 
     \plus{
     \muHat(a, a) - \distanceHat(a', b')
     }
    \end{align*}
    where inequality~(a) holds due to \frctwo\ at $\ell = \ell_a$;
    equality~(b) holds due to the construction of sets
    $\{L(a', b')\}_{a'\in[a:n],b'\in[a']}$,
    which guarantees that $\{L(a', b')\}_{a'\in[a:n],b'\in[a']}$
    is a partition of $[\ell_a, \mHat]$;
    equality~(c) holds due to the construction of sets
    $\{L(a', b')\}$,
    which guarantees that 
    for every $a' \in [a:n]$
    and every $\ell'\in L(a', b')$,
    $\muHat(\ell') \leq \muHat(\ell_a)$ 
    if and only if $b' \in [a]$;
    inequality~(d) holds due to the convexity of $\plus{\cdot}$;
    equality~(e) holds due to the solution construction;
    and inequality~(f) holds since 
    the solution construction which guarantees 
    $\muHat(\ell_a) \geq \muHat(a, a)$.
    
    
    \item[(v)] 
    It is implied by \frcthree\  and the construction of solution.
    
    \item[(vii)] It is implied by \frcfive\  and the construction of solution.
\end{enumerate}

We complete this step by noting that the constructed solution
$(\costHat, \{\qHat(a, b), \muHat(a, b),\distanceHat(a, b),
\distanceHatStar(a, b)\})$
has the same objective value 
as $(\costHat, \{\muHat(\ell),\distanceHat(\ell),
\distanceHatStar(\ell)\})$ due to the construction.
\paragraph{Step 2.}
In this step,
we use a ``stretch then compress'' argument
to modify the solution 
% of program~\hyperref[eq:strongly factor-revealing quadratic program]{$\mathcal{P}_{\texttt{FR-Quad}}(n)$}
obtained in \textbf{step 1}
into a feasible solution 
of program program~\ref{eq:strongly factor-revealing quadratic program}
with any targeted $\nHat\in\naturals$.

Note that by simultaneously
scaling $\{\qHat(a, b)\}$ down,
and $\{\muHat(a, b), \distanceHat(a, b), 
\distanceHatStar(a, b)\}$ up
by a 
multiplicative factor $\frac{n}{\nHat}$,\footnote{Namely, 
$\qHat(a, b) \gets \qHat(a, b) \cdot \frac{\nHat}{n}$,
and 
$\muHat(a, b) \gets \muHat(a, b) \cdot \frac{n}{\nHat}$,
$\distanceHat(a, b) \gets 
\distanceHat(a, b) \cdot \frac{n}{\nHat}$,
$\distanceHatStar(a, b) \gets 
\distanceHatStar(a, b) \cdot \frac{n}{\nHat}$.}
the solution still satisfies constraints (i), (ii), (iii.1), (iii.2),
(v), (vii) 
of program~\hyperref[eq:strongly factor-revealing quadratic program]{$\mathcal{P}_{\texttt{FR-Quad}}(n)$}
as well as constraint (iv.0).
Furthermore,
$\sum_{a\in[n]}\sum_{b\in[a]}\qHat(a, b) = \nHat$,
and the objective value remains unchanged. 

Next, we first \emph{stretch} the current solution 
in program~\hyperref[eq:strongly factor-revealing quadratic program]{$\mathcal{P}_{\texttt{FR-Quad}}(n)$}
into a solution 
in program~\hyperref[eq:strongly factor-revealing quadratic program]{$\mathcal{P}_{\texttt{FR-Quad}}(n')$}
for some larger $n' \in\naturals, n'\geq  n$ 
such that $\sum_{a\in[b:n']} \qHat(a, b) \leq \epsilon$
for every $b\in[b']$ and arbitrary small $\epsilon$.
Then, we \emph{compress} this solution in program~\hyperref[eq:strongly factor-revealing quadratic program]{$\mathcal{P}_{\texttt{FR-Quad}}(n')$}
into a feasible solution in program~\ref{eq:strongly factor-revealing quadratic program} as desired. 

\paragraph{Step 2.a- stretch.}
Here we use the following iterative approach.
Let $b^*$ be the index which maximizes $\sum_{a\in[b:n]}
\qHat(a, b)$.
Suppose $\sum_{a\in[b^*:n]}
\qHat(a, b^*) \geq \epsilon$.
Now, consider the following stretch-modification which increases $n$ by one.\footnote{In step 2.a, we use superscript $\dagger$ to denote the solution after the stretch-modification.}
\begin{align*}
    \muHat\primed(a, b) &\gets \left\{
    \begin{array}{ll}
    \muHat(a - 1, b - 1)     
    &  \forall b\in[b^* + 1:n + 1], a\in[b:n + 1]\\
    \muHat(a - 1, b)     
    &  \forall  b\in[1:b^*], a\in [b^* + 1: n + 1] \\
    \muHat(a, b) 
    & \forall b \in[1:b^* - 1], a \in [b, b^* - 1] \\
    \muHat(b^* - 1, b)
    & \forall b \in[1:b^* - 1], a = b^*\\
    \muHat(b^*, b^*)
    &\;~ b = b^*, a = b^*
    \end{array}
    \right.
    \\
    \distanceHat\primed(a, b) &\gets \left\{
    \begin{array}{ll}
    \distanceHat(a - 1, b - 1)     
    &  \forall b\in[b^* + 1:n + 1], a\in[b:n + 1]\\
    \distanceHat(a - 1, b)     
    &  \forall  b\in[1:b^*], a\in [b^* + 1: n + 1] \\
    \distanceHat(a, b) 
    & \forall b \in[1:b^* - 1], a \in [b, b^* - 1] \\
    \muHat(b^* - 1, b)
    & \forall b \in[1:b^* - 1], a = b^*\\
    \muHat(b^*, b^*)
    &\;~ b = b^*, a = b^*
    \end{array}
    \right.
    \\
    \distanceHatStar\primed(a, b) &\gets \left\{
    \begin{array}{ll}
    \distanceHatStar(a - 1, b - 1)     
    &  \forall b\in[b^* + 1:n + 1], a\in[b:n + 1]\\
    \distanceHatStar(a - 1, b)     
    &  \forall  b\in[1:b^*], a\in [b^* + 1: n + 1] \\
    \distanceHatStar(a, b) 
    & \forall b \in[1:b^* - 1], a \in [b, b^* - 1] \\
    \muHat(b^* - 1, b)
    & \forall b \in[1:b^* - 1], a = b^*\\
    \muHat(b^*, b^*)
    &\;~ b = b^*, a = b^*
    \end{array}
    \right.
    \\
    \qHat\primed(a, b) &\gets \left\{
    \begin{array}{ll}
    \qHat(a - 1, b - 1)     
    &  \forall b\in[b^* + 2:n + 1], a\in[b:n + 1]\\
    \frac{1}{2} \cdot \qHat(a - 1, b^*)
    &
    \forall b \in [b^*: b^* + 1], a \in[b^* + 1: n + 1] 
    \\
    \qHat(a, b) 
    &
    \forall b \in [1: b^* - 1], a\in[b: b^* - 1]
    \\
    \qHat(a - 1, b)
    &
    \forall b \in [1: b^* - 1], a \in [b^* + 1, n + 1] 
    \\
    0
    & 
    \forall b \in [1:b^*], a = b^*
    \end{array}
    \right.
    \\
    \costHat\primed &\gets \costHat,
    \qquad 
    n\primed \gets n + 1
\end{align*}
See a graphical illustration of the stretch-modification in 
\Cref{fig:stretch}.

\begin{figure}
    \centering
    \subfloat[
    before stretch-modification]{\input{Paper/figs/fig-stretch-0}}
    ~~~~
    \subfloat[
    after stretch-modification]{\input{Paper/figs/fig-stretch-1}}
    \caption{Graphical example illustration of the stretch-modification in 
    \textbf{step 2.1- stretch}:
    given an initial solution with $n = 9$ obtained in \textbf{step 1},
    we construct a feasible solution of program~\ref{eq:strongly factor-revealing quadratic program} with $n\primed = 10$.
    Here each solid box corresponds to an index $(a, b)$.
    First, we identify index $b^* = 5$ which maximizes 
    $\sum_{a\in[b, n]}\qHat(a, b)$.
    Then, we let 
    $\muHat(\cdot, b^*), \distanceHat(\cdot,b^*), \distanceHatStar(\cdot, b^*)$ in 
    row $b^*$ be duplicated, and $\qHat(\cdot, b^*)$
    be halved (i.e., break the black boxes into 
    dark gray boxes in row $b^*$ and $b^* + 1$).
    All light gray boxes remain unchanged, but their indexes may be shifted (depending on their positions).
    Finally, we add dummy (i.e., white) boxes whose 
    $\qHat\primed(b^*, \cdot) = 0$ and 
    duplicate $\muHat(b^*, b), \distanceHat(b^*,b), \distanceHatStar(b^*,b)$ from 
    $\muHat(b^* - 1,b)$ if $b \in[b^* - 1]$,
    and $\muHat(b^*, b^*)$ if $b = b^*$.
    % $\muHat\primed(b^*, b) = \distanceHat\primed(b^*,b)=
    % \distanceHatStar\primed(b^*,\cdot) \gets \muHat(b^*, \cdot)$.
    }
    % \label{fig:stretch}
\end{figure}

It is straightforward to verify that the objective value 
remains unchanged after the stretch-modification,
and constraints (i), (ii), (iii.1), 
(iii.2), (v), (vii) of 
of program~\hyperref[eq:strongly factor-revealing quadratic program]{$\mathcal{P}_{\texttt{FR-Quad}}(n\primed)$},
as well as  constraint (iv.0), 
and
$\sum_{a\in[n\primed]}\sum_{b\in[a]}\qHat\primed(a, b) = \nHat$ 
are satisfied.
The only non-trivial constraint is (ii).
Here, we verify two cases and the remaining cases follows similar arguments\footnote{Basically, the the remaining cases use almost the same arguments with slight modification on indexes.} and are thus omitted.
\begin{itemize}
    \item[-] 
    For $a\in[1:b^* - 1]$, $a' = b^*$,
    $b\in[a], b'\in[a']$, note that 
    \begin{align*}
        \muHat\primed(a', b') 
        &\overset{(a)}{=}
        % \muHat(b^*, b')
        % \overset{(b)}{=}
        \distanceHat\primed(a', b')
        \leq 
        \distanceHatStar\primed(a, b)
        +
        \distanceHat\primed(a, b)
        +
        \distanceHat\primed(a', b')
    \end{align*}
    where equality~(a) holds by construction.
    
    % \item[-] For $a = b^*$, $a' = b^* + 1$,
    % $b\in[a - 1], b' \in [a' - 1]$, note that 
    % \begin{align*}
    %     \muHat\primed(a', b') 
    %     &
    %     \overset{(a)}{=}
    %     % \muHat(a' - 1, b') 
    %     % \left\{
    %     % \begin{array}{ll}
    %     %  \muHat(a' - 1, b' - 1)  
    %     %  &  
    %     %  \quad \text{if $b' = a'$}\\
    %     %  \muHat(a' - 1, b')    & 
    %     %  \quad \text{if $b' = a' - 1$}
    %     % \end{array}
    %     % \right.
    %     % \\
    %     % &= 
    %     \muHat(b^*, b')
    %     \\
    %     &\overset{(b)}{\leq}
    %     \distanceHatStar(b^* - 1, b) + 
    %     \distanceHat(b^* - 1, b) 
    %     +
    %     \distanceHat(b^*, b')
    %     \\
    %     \&\overset
    %     \\
    %     &\overset{(d)}{=}
    %     % \distanceHatStar\primed(a, b)
    %     % \\
    %     % &\leq 
    %     \distanceHatStar\primed(a, b)
    %     +
    %     \distanceHat\primed(a, b)
    %     +
    %     \distanceHat\primed(a', b')
    % \end{align*}
    % where equalities (a) (c) hold by construction;
    % and inequality~(b) holds due to (ii) in the original solution.
    
    \item[-] For $a = b^*$, $a'\in[b^* + 2:n\primed]$, $b\in[a - 1], 
    b'\in[a']$, note that 
    \begin{align*}
         \muHat\primed(a', b') 
        &
        \overset{(a)}{=}
        \left\{
        \begin{array}{ll}
         \muHat(a' - 1, b' - 1)  
         &  
         \quad \text{if $b' \in [b^* + 1:n\primed]$}\\
         \muHat(a' - 1, b')    & 
         \quad \text{if $b' \in [1:b^*]$}
        \end{array}
        \right.
        \\
        &\overset{(b)}{\leq}
        \left\{
        \begin{array}{ll}
         \distanceHatStar(b^* - 1, b) + 
         \distanceHat(b^* - 1, b) +
         \distanceHat(a' - 1, b' - 1)  
         &  
         \quad \text{if $b' \in [b^* + 1:n\primed]$}\\
         \distanceHatStar(b^* - 1, b) + 
         \distanceHat(b^* - 1, b) +
         \distanceHat(a' - 1, b')    & 
         \quad \text{if $b' \in [1:b^*]$}
        \end{array}
        \right.
        \\
        &\overset{(c)}{\leq}
        \left\{
        \begin{array}{ll}
         \muHat(b^* - 1, b) + 
         \muHat(b^* - 1, b) +
         \distanceHat(a' - 1, b' - 1)  
         &  
         \quad \text{if $b' \in [b^* + 1:n\primed]$}\\
         \muHat(b^* - 1, b) + 
         \muHat(b^* - 1, b) +
         \distanceHat(a' - 1, b')    & 
         \quad \text{if $b' \in [1:b^*]$}
        \end{array}
        \right.
    \\
    &\overset{(d)}{=}
    \distanceHatStar\primed(a, b) + \distanceHat\primed(a, b)
    +
    \distanceHat\primed(a', b')
    \end{align*}
    where equalities~(a) (d) hold by construction;
    inequality~(b) holds due to (ii) in the original
    solution;
    % at $a = b^* - 1$, $b = b$;
    and inequality~(c) holds due to (iii.1) (iii.2)
    in the original solution.
    
\end{itemize}

\paragraph{Step 2.b- compress.}
Suppose we repeat \textbf{step 2.a- stretch} 
on solution $(\costHat, \{\qHat(a, b), \muHat(a, b),\distanceHat(a, b)$,
$\distanceHatStar(a, b)\}_{a\in[n], b\in[a]})$
until the following event\footnote{By
repeating \textbf{step 2.a- stretch},
in the limit,
we obtain a continuous version of solution
 $(\costHat, \{\qHat(a, b), \muHat(a, b),\distanceHat(a, b),
\distanceHatStar(a, b)\})$, i.e., 
index $(a, b)$ is no longer discrete, and $\{\qHat(a, b)\}$
becomes density.
Thus, it is guaranteed that 
the event happens in the limit.
For ease of presentation, we assume the event 
happens when $n$ is still finite. Our analysis extends straightforward when the event happens in the limit.} happens:
there exists $0 = b_0 < b_1 < b_2 < \dots
% <b_{\tau} <\dots 
< b_{\nHat} = n$
such that
for every $t\in[\nHat]$,
$\sum_{b\in [b_{t - 1} + 1: b_t]}
\sum_{a\in[b:n]}\qHat(a, b) = 1$.

To simplify the notation, 
for each $t\in[\nHat], \tau \in[t]$
let $C(t, \tau) = \{(a, b):
a\in[b_{t - 1} + 1:b_t],
b\in[b_{\tau - 1} + 1:\min\{a, b_\tau\}\}$.
By definition, $\{C(t, \tau)\}_{t\in[\nHat], \tau\in[t]}$
is a partition of index set $\{(a, b):a\in[n], b\in[a]\}$.

Now we construct a feasible solution of program~\ref{eq:strongly factor-revealing quadratic program} through compression as follows.\footnote{In step 2.b, we use superscript $\dagger$ to denote the solution after the compression.}
\begin{align*}
    t \in [\nHat],
    \tau \in [t]:&
    \qquad 
    \muHat\primed(t, \tau) \gets
    \frac{
    \sum_{(a, b)\in C(t, \tau)}
    % \sum_{a\in[b_{t - 1} + 1: b_t]}
    % \sum_{b\in[b_{\tau - 1} + 1: \min\{a, b_{\tau}\}]}
    \qHat(a, b) \cdot \muHat(a, b)
    }{
    \sum_{(a, b)\in C(t, \tau)}
    % \sum_{a\in[b_{t - 1} + 1: b_t]}
    % \sum_{b\in[b_{\tau - 1} + 1: \min\{a, b_{\tau}\}]}
    \qHat(a, b) 
    }\\&
    \qquad 
    \distanceHat\primed(t, \tau) \gets
    \frac{
    \sum_{(a, b)\in C(t, \tau)}
    % \sum_{a\in[b_{t - 1} + 1: b_t]}
    % \sum_{b\in[b_{\tau - 1} + 1: \min\{a, b_{\tau}\}]}
    \qHat(a, b) \cdot \distanceHat(a, b)
    }{
    \sum_{(a, b)\in C(t, \tau)}
    % \sum_{a\in[b_{t - 1} + 1: b_t]}
    % \sum_{b\in[b_{\tau - 1} + 1: \min\{a, b_{\tau}\}]}
    \qHat(a, b) 
    }\\&
    \qquad 
    \distanceHatStar\primed(t, \tau) \gets
    \frac{
    \sum_{(a, b)\in C(t, \tau)}
    % \sum_{a\in[b_{t - 1} + 1: b_t]}
    % \sum_{b\in[b_{\tau - 1} + 1: \min\{a, b_{\tau}\}]}
    \qHat(a, b) \cdot \distanceHatStar(a, b)
    }{
    \sum_{(a, b)\in C(t, \tau)}
    % \sum_{a\in[b_{t - 1} + 1: b_t]}
    % \sum_{b\in[b_{\tau - 1} + 1: \min\{a, b_{\tau}\}]}
    \qHat(a, b) 
    }\\&
    \qquad 
    \qHat\primed(t, \tau) \gets
    {
    \sum_{(a, b)\in C(t, \tau)}
    % \sum_{a\in[b_{t - 1} + 1: b_t]}
    % \sum_{b\in[b_{\tau - 1} + 1: \min\{a, b_{\tau}\}]}
    \qHat(a, b) 
    }\\
    &\qquad \costHat\primed \gets \costHat
\end{align*}
When $
    \sum_{(a, b)\in C(t, \tau)} \qHat(a, b)= 0$ for some 
$t\in[\nHat], \tau\in[t]$,
we set $\muHat\primed(t,\tau),
\distanceHat\primed(t,\tau),
\distanceHatStar(t, \tau)$
to
be the unweighted average,
and $\qHat\primed(t, \tau) = 0$.
See a graphical illustration of the construction
in \Cref{fig:compression}.

\begin{figure}
    \centering
    \input{Paper/figs/fig-compression}
    \caption{Graphical example illustration of \textbf{step 2.b- compress}:
    given an initial solution with $n = 10$ obtained in \textbf{step 2.a}, 
    we construct a feasible solution of program~\ref{eq:strongly factor-revealing quadratic program} with $\nHat = 4$.
    Here each solid box corresponds to an index $(a, b)$ of the initial solution.
    First, we identify $b_1 = 2, b_2 = 5, b_3 = 6, b_4 = 10$
    such that 
    for every $t\in[\nHat]$,
    $\sum_{b\in [b_{t - 1} + 1: b_t]}
    \sum_{a\in[b:\nHat]}\qHat(a, b) = 1$.
    Then, we take the weighted average for each dashed box,
    which corresponds to an index $(t, \tau)$ in program~\ref{eq:strongly factor-revealing quadratic program}.
    }
    % \label{fig:compression}
\end{figure}

It is straightforward to verify that 
the constructed solution has the same objective value.
Next, we verify that the constructed solution 
satisfies all constraints in program~\ref{eq:strongly factor-revealing quadratic program}, which finishes our proof.
\begin{enumerate}
    \item[(i)] It is implied by the construction of solution and (i) in the original solution.
    \item[(ii)] It follows a similar argument as 
    \textbf{step 1}.
    \item[(iii.1) (iii.2)] It is implied by the construction of solution and (iii.1) (iii.2) in the original solution.
    \item[(iv)] It follows a similar argument as 
    \textbf{step 1}.
    Specifically, for any $t\in[\nHat]$, we have
    \begin{align*}
        \costHat\primed 
        &\overset{(a)}{=}
        \costHat
        \\
        &\overset{(b)}{\geq}
        \sum_{a'\in[b_t:n]}
     \sum_{b'\in[a]}
     \qHat(a', b')
     \cdot 
     \plus{
     \muHat(a', b') - \distanceHat(a', b')
     }
     \\
     &\qquad\qquad 
     +\sum_{a'\in[b_t:n]}
     \sum_{b'\in[a+1:a']}
     \qHat(a', b')
     \cdot 
     \plus{
     \muHat(b_t, b_t) - \distanceHat(a', b')
     }
        \\
        &\overset{}{\geq}
        \sum_{a'\in[b_t + 1:n]}
     \sum_{b'\in[a]}
     \qHat(a', b')
     \cdot 
     \plus{
     \muHat(a', b') - \distanceHat(a', b')
     }
     \\
     &\qquad
     +\sum_{a'\in[b_t + 1:n]}
     \sum_{b'\in[a+1:a']}
     \qHat(a', b')
     \cdot 
     \plus{
     \muHat(b_t, b_t) - \distanceHat(a', b')
     }
        \\
        &\overset{(c)}{\geq}
        \sum_{t' \in[t + 1:\nHat]}
        \sum_{\tau'\in[t]}
        \left(
        \sum_{(a', b')\in C(t', \tau')}\qHat(a', b')
        \right)
        \cdot 
        \plus
        { 
        \frac{
        \sum_{(a', b')\in C(t', \tau')}\qHat(a', b')\cdot 
        (\muHat(a',b') - \distanceHat(a', b'))
        }{
        \sum_{(a', b')\in C(t', \tau')}\qHat(a', b')
        }
        }
     \\
     &\qquad
        +\sum_{t' \in[t + 1:\nHat]}
        \sum_{\tau'\in[t + 1:t']}
        \left(
        \sum_{(a', b')\in C(t', \tau')}\qHat(a', b')
        \right)
        \cdot 
        \plus
        { 
        \frac{
        \sum_{(a', b')\in C(t', \tau')}\qHat(a', b')\cdot 
        (\muHat(b_t,b_t) - \distanceHat(a', b'))
        }{
        \sum_{(a', b')\in C(t', \tau')}\qHat(a', b')
        }
        }
        \\
        &\overset{(d)}{=}
        \sum_{t' \in[t + 1:\nHat]}
        \sum_{\tau'\in[t]}
        \qHat\primed(t',\tau')
        \cdot 
        \plus
        { 
        \muHat\primed(t',\tau') -
        \distanceHat\primed(t', \tau')
        }
     \\
     &\qquad
        +\sum_{t' \in[t + 1:\nHat]}
        \sum_{\tau'\in[t + 1:t']}
        \qHat\primed(t',\tau')
        \cdot 
        \plus
        {
        \muHat(b_t, b_t) - 
        \distanceHat\primed(t', \tau')
        }
        \\
        &\overset{(e)}{\geq}
        \sum_{t' \in[t + 1:\nHat]}
        \sum_{\tau'\in[t]}
        \qHat\primed(t',\tau')
        \cdot 
        \plus
        { 
        \muHat\primed(t',\tau') -
        \distanceHat\primed(t', \tau')
        }
     \\
     &\qquad
        +\sum_{t' \in[t + 1:\nHat]}
        \sum_{\tau'\in[t + 1:t']}
        \qHat\primed(t',\tau')
        \cdot 
        \plus
        {
        \muHat\primed(t, t) - 
        \distanceHat\primed(t', \tau')
        }
    \end{align*}
    where equalities~(a) (d) hold by construction;
    inequality~(b) holds due to (iv.0) at $a = b_t$
    in the original solution;
    inequality~(c) holds due to the convexity of $\plus{\cdot}$;
    and 
    inequality~(e) holds due to 
    the construction of 
    $\muHat\primed(t, t)$ and 
    (i) in the original solution,
    which guarantees $\muHat\primed(t, t) \leq 
    \muHat(b_t, b_t)$.
    % \item[(iv.2)] It follows a similar argument as 
    % \textbf{step 1}.
    % Specifically,
    % \begin{align*}
    %     ss
    % \end{align*}
    \item[(v)] It is implied by the construction of solution and (v) in the original solution.
    \item[(vi)] It is implied by the definition $(b_1, \dots, b_{\nHat})$.
    \item[(vii)] It is implied by  the construction of solution and (vii) in the original solution.
\end{enumerate}

==> Notes/lower-bound.tex <==
\section{Approximation Lower Bound}
When we restrict to instances 
where $\alpha_{ii} = 1$ for all node $i\in V$,
the problem reduce to standard 
facility location problem
\citep[cf.][]{GK-99}
where the distance cost between $i$ to $j$
is defined as $\frac{2\exp(-d_{ij})}{C + 2\exp(-d_{ij}}$
which satisfies triangle inequality, symmetry
but violates identity of indiscernibles.

==> Notes/notation.tex <==
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{ifthen}
\usepackage{fixmath}
\usepackage{xfrac}
\usepackage{sidecap}
\usepackage{subfig}
\usepackage{caption}

\newcommand{\rand}{\pi}

\newcommand{\revelationgap}{\gaplowerbound}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\newcommand{\agind}[1][i]{_{#1}}


%\newcommand{\ulz}[1]{{\def\ULdepth{0in}\uline{#1}}}

\newcommand{\jj}[2][j]{\{#2\}_{#1}}
\newcommand{\jopt}{j\opt}
\newcommand{\jjopt}{\jj[\jopt]}

%\newcommand{\jjul}[2][j]{#2_{\ulz{\smash{#1}}}}

% accents for using with newagentvar
% (must take a single argument)
\newcommand{\ironed}{\bar}
\newcommand{\constrained}{\hat}
\newcommand{\optconstrained}{\composed{\optimized}{\constrained}}
\newcommand{\optimized}[1]{#1\opt}
\newcommand{\differentiated}[1]{#1'}
\newcommand{\fortype}{\tilde}
\newcommand{\tagged}[2]{{#2}^{#1}}
 

\newcommand{\starred}[1]{#1^\star}
\newcommand{\primedarg}[1]{#1\primed}
\newcommand{\noaccents}[1]{#1}
% compose accents on the fly
\newcommand{\composed}[3]{#1{#2{#3}}}





\newcommand{\newagentvar}[3][\noaccents]{%
\expandafter\newcommand\expandafter{\csname #2\endcsname}{#1{#3}}%
\expandafter\newcommand\expandafter{\csname #2s\endcsname}{#1{\boldsymbol{#3}}}%
\expandafter\newcommand\expandafter{\csname #2smi\endcsname}[1][i]{#1{\boldsymbol{#3}}_{-##1}}%
\expandafter\newcommand\expandafter{\csname #2i\endcsname}[1][i]{#1{#3}\agind[##1]}%
\expandafter\newcommand\expandafter{\csname #2ith\endcsname}[1][i]{#1{#3}_{(##1)}}%
}

\newcommand{\newitemvar}[3][\noaccents]{%
\expandafter\newcommand\expandafter{\csname #2\endcsname}{#1{#3}}%
\expandafter\newcommand\expandafter{\csname #2s\endcsname}{#1{\boldsymbol{#3}}}%
\expandafter\newcommand\expandafter{\csname #2smj\endcsname}[1][j]{#1{\boldsymbol{#3}}_{-##1}}%
\expandafter\newcommand\expandafter{\csname #2j\endcsname}[1][j]{#1{#3}_{##1}}%
\expandafter\newcommand\expandafter{\csname #2jth\endcsname}[1][j]{#1{#3}_{(##1)}}%
}





%
% perhaps don't use this.
%
\newagentvar{alloc}{x}


%
% flattened.
%
\newagentvar{falloc}{z}

%
% in quantile space.
%
\newagentvar{quant}{q}
\newagentvar[\constrained]{exquant}{\quant}
\newagentvar[\constrained]{critquant}{\quant}  %remove?
\newcommand{\monoq}{\quant_m}
\newagentvar{Val}{\nu}
\newagentvar{toquant}{Q}

% remove these?
\newcommand{\quantp}{\exquant}
\newagentvar{qprice}{\price}
\newagentvar{qrev}{R}
\newagentvar[\ironed]{iqrev}{\qrev}


%\newagentvar{\calloc}{\starred \alloc}

\newagentvar{qalloc}{y}
\newagentvar{cumalloc}{Y}
%\newagentvar[\constrained]{calloc}{\qalloc}
\newagentvar[\constrained]{cumcalloc}{\cumalloc}
\newagentvar[\ironed]{ialloc}{\qalloc}
\newagentvar[\ironed]{icumalloc}{\cumalloc}

\newcommand{\exposted}[1]{#1^{\text{\it EP}}}
\newagentvar[\composed{\exposted}{\constrained}]{excalloc}{\qalloc}
\newagentvar[\exposted]{exalloc}{\qalloc}
\newagentvar[\exposted]{extalloc}{\talloc}
\newagentvar[\exposted]{exfalloc}{\falloc}



\newagentvar{rev}{R}
\newagentvar[\differentiated]{marg}{\rev}
\newagentvar{rawrev}{P}
\newagentvar[\differentiated]{rawmarg}{\rawrev}

\newagentvar[\primedarg]{inducedrev}{\rev}

\newagentvar[\tilde]{pseudorev}{\rev}
\newagentvar[\tilde]{pseudorawrev}{\rawrev}


%
% in value/type space
%

\newagentvar{typespace}{\mathcal{T}}
% \newagentvar{feasible}{\mathcal{F}}
\newagentvar{typesubspace}{S}
\newcommand{\extypes}[1][\exquant]{\typesubspace^{#1}\!}

\newagentvar{type}{t}
\newagentvar{othertype}{s}
\newagentvar{val}{v}
\newagentvar{hval}{\overline{\val}}
\newagentvar{lval}{\underline{\val}}
\newagentvar{hbudget}{\bar \wealth}
\newagentvar{budget}{w}
\newagentvar{wealth}{w}
\newagentvar{lbudget}{\underaccent{\bar}{ \wealth}}
\newagentvar{lowestval}{\lval}
\newagentvar{cumval}{V}
\newagentvar{cumprice}{\cumpayoff}
\newagentvar{revcurve}{\payoffcurve}
\newagentvar{cumwelfare}{\cumpayoff}
\newagentvar{welcurve}{\payoffcurve}

% \newagentvar{cumval}{V}
% \newagentvar{cumprice}{P}
% \newagentvar{revcurve}{R}
% \newagentvar{cumwelfare}{K}
% \newagentvar{welcurve}{W}

\newagentvar{outcome}{w}
\newagentvar{outcomespace}{\mathcal{W}}
\newcommand{\nulloutcome}{\emptyset}


\newcommand{\served}[1]{#1^1}
\newcommand{\nonserved}[1]{#1^0}
\newcommand{\alloced}[1]{#1^{\alloc}}
\newcommand{\allocedi}[1]{#1^{\alloci}}
\newagentvar[\alloced]{xoutcome}{\outcome}
\newagentvar[\allocedi]{xioutcome}{\outcome}
\newagentvar[\served]{soutcome}{\outcome}

\newagentvar[\nonserved]{nsoutcome}{\outcome}


\newagentvar{price}{p}
\newagentvar{randomprice}{\prices}
\newagentvar{randomquant}{\quants}
\newagentvar{talloc}{\alloc}
\newagentvar[\tilde]{balloc}{\alloc}
\newagentvar[\tilde]{bprice}{\price}

\newagentvar{act}{a}
\newagentvar{bidspace}{A}
\newagentvar{actspace}{A}



\newagentvar[\constrained]{critval}{\val}
\newagentvar[\constrained]{crittype}{\type}
\newagentvar[\constrained]{critvirt}{\virt}
\newagentvar[\constrained]{reserve}{\val} % should this be used???
\newagentvar[\constrained]{bidreserve}{\bid} % should this be used???
\newcommand{\monop}{\val_m}
\newagentvar[\constrained]{monot}{\type}
\newagentvar[\optimized]{monorev}{\rev}


%%
%% Bayes-Nash Approximation
%%
\newagentvar{rcalloc}{y}
\newagentvar[\optimized]{optrcalloc}{\rcalloc}
\newagentvar{biddist}{G}
\newcommand{\revcov}{\mu}
\newagentvar[\constrained]{critbid}{\bid}
\newagentvar[\constrained]{cbid}{B}
\newagentvar[\primedarg]{wbid}{\bid}
\newagentvar{gfunc}{\vartheta}
\newagentvar{block}{C}




\newagentvar{util}{u}

% why two?
\newagentvar{strat}{s}
\newagentvar{bid}{b}



\newagentvar{virt}{\phi}
\newagentvar{cumvirt}{\Phi}
\newagentvar{qvirt}{\phi}
\newagentvar[\ironed]{ivirt}{\virt}
\newagentvar[\ironed]{icumvirt}{\cumvirt}

\newagentvar[\tagged{\text{SD}}]{sdvirt}{\virt}
\newagentvar[\composed{\tagged{\text{SD}}}{\ironed}]{sdivirt}{\virt}
\newagentvar[\tagged{\text{MD}}]{mdvirt}{\virt}
\newagentvar[\composed{\tagged{\text{MD}}}{\ironed}]{mdivirt}{\virt}



\newagentvar{dist}{F}
\newagentvar{dens}{f}
\newagentvar{hazard}{h}
\newagentvar{cumhazard}{H}



\newagentvar[\ironed]{iprice}{\price}  %% what for?
\newagentvar[\ironed]{ival}{\val}  %% what for?

\newagentvar[\ironed]{icumval}{\cumval}
\newagentvar{ints}{\mathcal{I}}




\newcommand{\exfeasible}{\text{EAF}}
\newcommand{\feasibles}{\mathcal{X}}
\newcommand{\tfeasibles}{\feasibles}
\newcommand{\ffeasibles}{\mathcal{Z}}
\newcommand{\qfeasibles}{\mathcal{Y}}

% for position auctions.
% is this used!?!?
\newagentvar{wal}{w}



%
% for items
%




\newitemvar{pos}{j}
\newitemvar{weight}{w}
\newitemvar[\differentiated]{mweight}{\weight}
\newitemvar{udtype}{\type}
\newitemvar[\constrained]{udcrittype}{\type}
\newitemvar{udalloc}{\alloc}
\newitemvar{udprice}{\price}
\newitemvar[\constrained]{udcalloc}{\qalloc}
\newitemvar[\constrained]{udcumcalloc}{\cumalloc}





\newagentvar{mech}{\mathcal{M}}
\newagentvar[\skew{5}{\hat}]{cmech}{\mathcal{M}}
\newagentvar{alg}{\mathcal{A}}



\newcommand{\dquant}{r}
\newcommand{\dval}{z}

%\newcommand{\Rev}[1]{\mathbf{Rev}[#1]}

\newcommand{\Rev}[2][]{\text{\bf Rev}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}

\newcommand{\Revsb}[1]{\text{\bf Rev}_{#1}({\rm SB})}
% \newcommand{\Revsb}[2][]{\text{\bf Rev}_{\text{sb}}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}

% \newcommand{\Rev}[2][]{\text{\bf Rev}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}

\newcommand{\MargRev}[1]{\mathbf{MargRev}[#1]}
\newcommand{\Obj}[1]{\mathbf{Payoff}[#1]}

\newcommand{\Wel}[2][]{\text{\bf Payoff}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}

% \newcommand{\Wel}[2][]{\text{\bf Wel}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}

\newcommand{\indep}{\mathcal{I}}





\newcommand{\udmaxj}{\optimized{j}}
\newcommand{\udtypemax}{\udtypej[\optimized{j}]}


\newcommand{\udtypemin}{\type^{\min}}
\newcommand{\maxtype}{\type^{\max}}
\newcommand{\lagrange}{\lambda}
\newcommand{\optlagrange}{\optimized{\lagrange}}
% \newcommand{\budget}{B}
% \newcommand{\wealth}{w}




\newcommand{\iG}{\bar{G}}
\newcommand{\ig}{\bar{g}}
\newcommand{\iq}{\bar{q}}

\newcommand{\game}{G}





\newcommand{\rawprice}{\price^{\game}}
\newcommand{\rawprices}{\prices^{\game}}
\newcommand{\rawpricesmi}{\rawprices_{-i}}
\newcommand{\rawpricei}[1][i]{\rawprice\agind[#1]}




\newcommand{\rawalloc}{\alloc^{\game}}
\newcommand{\rawallocs}{\allocs^{\game}}
\newcommand{\rawallocsmi}{\rawallocs_{-i}}
\newcommand{\rawalloci}[1][i]{\rawalloc\agind[#1]}




\newcommand{\zeros}{{\mathbf 0}}
\newcommand{\ones}{{\mathbf 1}}



\newcommand{\cost}{c}

\DeclareMathOperator{\OPT}{OPT}
\DeclareMathOperator{\Vic}{Vic}
\DeclareMathOperator{\Mye}{Mye}
\DeclareMathOperator{\VCG}{VCG}
\DeclareMathOperator{\SM}{SM}
\DeclareMathOperator{\RM}{RM}
\DeclareMathOperator{\VSM}{VSM}
\DeclareMathOperator{\IVSM}{IVSM}
\DeclareMathOperator{\FP}{FP}
\DeclareMathOperator{\SP}{SP}


\DeclareMathOperator{\EF}{EF}
\DeclareMathOperator{\EFO}{EFO}
\DeclareMathOperator{\RSEM}{RSEM}
\DeclareMathOperator{\RSOP}{RSOP}
\DeclareMathOperator{\RSPE}{RSPE}

\DeclareMathOperator{\surplus}{Surplus}
\DeclareMathOperator{\IID}{IID}
\DeclareMathOperator{\profit}{Profit}

\DeclareMathOperator{\REF}{REF}
\DeclareMathOperator{\APX}{APX}
\DeclareMathOperator{\UB}{UB}
\DeclareMathOperator{\LB}{LB}

\def\BM{\REF}
\def\PERF{\APX}


\newcommand{\poly}{\mathcal{P}}
\newcommand{\Lot}{\mathcal{L}}
\newcommand{\np}{\mathcal{NP}}
\newcommand{\algo}{\mathcal{A}}
\newcommand{\auction}{\mathcal{A}}
\newcommand{\mecha}{\mathcal{M}}
\newcommand{\ialgo}{\bar\mathcal{A}}

\newcommand{\osp}{\mathcal{F}}
\newcommand{\osps}{\osp \super 2}

\newcommand{\EFOs}{\EFO \super 2}
 
\newcommand{\bm}{\mathcal{G}}
\newcommand{\bms}{\bm \super 2}

%\newcommand{\setsize}[1]{{\left|#1\right|}}

\newcommand{\reals}{{\mathbb R}}
\newcommand{\posreals}{\reals_+}






\newcommand{\thealloc}{\hat{\alloc}}
\newcommand{\analloc}{\alloc\primed}


\newagentvar{trans}{\sigma}

\newagentvar{demandset}{S}

\newcommand{\opt}{^{\star}}
\newcommand{\primed}{^\dagger}
\newcommand{\doubleprimed}{^{\ddagger}}
\newcommand{\tripleprimed}{^{\S}}
\newcommand{\pprimed}{\doubleprimed}

\newagentvar{distout}{w}
\newagentvar{idistout}{\bar{w}}

\newcommand{\rsmsize}{m}

\newcommand{\metric}{c}


\newcommand{\implements}{\preceq}
\newcommand{\isimplementedby}{\succeq}


%
% matroid definitions.
%
\DeclareMathOperator{\matrank}{rank}
\newcommand{\rank}{\matrank}            % xphase this out.
\newcommand{\matset}{S}
\newcommand{\matground}{N}
\newcommand{\matindeps}{\mathcal{I}}
\newcommand{\matweightedrank}[1][\wals]{\rank_{#1}}

%% correlation gap, set functions

\newcommand{\cset}{S}
\newcommand{\setfunc}{g}
\newcommand{\mwesetfunc}{\setfunc^{\text{MWE}}}
\newcommand{\oomsetfunc}{\setfunc^{\text{OOM}}}

\newcommand{\setdist}{\mathcal{D}}
\newcommand{\margsetdist}{\setdist^{I}}


%% prophet inequality
\newcommand{\gamblerpayoff}{\APX}
\newcommand{\prophetpayoff}{\REF}
\newcommand{\prnosale}{\chi}
\newcommand{\prnone}{\chi}
\newcommand{\Ei}{\mathcal{E}_i}

\newcommand{\numpieces}{\ell}
\newcommand{\numtypes}{\ell}

\newcommand{\rejectset}{\perp}


\newcommand{\threshutil}{\mu}

\newcommand{\convexcomb}{\alpha}


\newcommand{\concavefunc}{h}



\newcommand{\uniformzeroone}{U[0,1]}

\newcommand{\disteqr}{\dist^{\text{EQR}}}
\newcommand{\rawreveqr}{\rawrev^{\text{EQR}}}
\newcommand{\reveqr}{\rev^{\text{EQR}}}
\newcommand{\Valeqr}{\Val^{\text{EQR}}}
\newcommand{\denseqr}{\dens^{\text{EQR}}}


\newcommand{\virtexp}{\virt^{\text{EXP}}}
\newcommand{\distexp}{\dist^{\text{EXP}}}
\newcommand{\revexp}{\rev^{\text{EXP}}}
\newcommand{\densexp}{\dens^{\text{EXP}}}
\newcommand{\hazardexp}{\hazard^{\text{EXP}}}



\newcommand{\harmonick}[1][k]{\mathcal{H}_{#1}}



\newcommand{\positivepart}[1]{\smash{(#1)^+}} 



\newcommand{\apx}{\beta}
\newcommand{\optapx}{\apx\opt}


%%
%% PRIOR FREE
%%
\newcommand{\target}{\Pi}
\newcommand{\resolution}{\gamma}
\newcommand{\optresolution}{\resolution\opt}
\newcommand{\efalloc}{y}


\newcommand{\highval}{h}



\newcommand{\mincoini}[1][i]{w_{#1}}
\newcommand{\cummincoini}[1][i]{W_{#1}}

\newcommand{\sampind}{y}
\newcommand{\cumsampind}{Y}
\newcommand{\sampindi}[1][i]{\sampind_{#1}}
\newcommand{\cumsampindi}[1][i]{\cumsampind_{#1}}

\newcommand{\optind}{i\opt}
\newcommand{\optval}{\monop}
\newcommand{\sampleoptval}{\monop_S}
\newcommand{\marketoptval}{\monop_M}

\newcommand{\valssample}{\vals_{S}}
\newcommand{\sampleoptind}{\optind_S}
\newcommand{\marketoptind}{\optind_M}
\newcommand{\samplevals}{\vals_{S}}
\newcommand{\marketvals}{\vals_{M}}


%%
%% mutli-dimensional and non-linear.
%%
\newcommand{\pathdist}{\dist_{1}}
\newcommand{\pathdens}{\dens_{1}}
\newcommand{\pathmonop}{\monop_{1}}
\newcommand{\pathvirt}{\virt_{1}}
\newcommand{\pathfunc}{\tau}
\newcommand{\pathtype}[1][\quant]{\pathfunc({#1})}
\newcommand{\margpathtype}[1][\quant]{\pathfunc'({#1})}
\newcommand{\pathzero}{1}
\newcommand{\pathtypezero}{\pathtype[\pathzero]}
\newcommand{\pathq}{\theta}
\newcommand{\pathcritq}{\constrained{\pathq}}
\newcommand{\pathfuncq}[1][\pathq]{\pathfunc \super {#1}}
\newcommand{\pathtypespaceq}[1][\pathq]{\typespace \super {#1}}
\newcommand{\pathdistq}[1][\pathq]{\dist \super {#1}}
\newcommand{\pathtypesvq}[1][\critval\pathcritq]{\typesubspace \super {#1}\!}
\newcommand{\pathtypesv}[1][\critval]{\typesubspace \super {#1}\!}

%% \newcommand{\pathdist}{\dist_{\max}}
%% \newcommand{\pathdens}{\dens_{\max}}
%% \newcommand{\pathmonop}{\monop_{\max}}
%% \newcommand{\pathvirt}{\virt_{\max}}
%% \newcommand{\pathfunc}{C}
%% \newcommand{\pathtypezero}{\pathtype[0]}
%% \newcommand{\pathtype}[1][\val]{\type^{#1}}
%% \newcommand{\pathq}{\theta}
%% \newcommand{\pathcritq}{\constrained{\pathq}}
%% \newcommand{\pathfuncq}[1][\pathq]{\pathfunc_{#1}}
%% \newcommand{\pathtypespaceq}[1][\pathq]{\typespace_{#1}}
%% \newcommand{\pathdistq}[1][\pathq]{\dist_{#1}}
%% \newcommand{\pathtypesvq}[1][\critval\pathcritq]{\typesubspace^{#1}\!}
%% \newcommand{\pathtypesv}[1][\critval]{\typesubspace^{#1}\!}


\newcommand{\typespaceboundary}{\partial\typespace}
\newcommand{\normal}{\eta}


% multi-dimensional approx

\newcommand{\maxcore}{\critval}
\newcommand{\bundleprice}{\critval\primed}


\DeclareMathOperator{\CORE}{CORE}
\DeclareMathOperator{\TAIL}{TAIL}
\DeclareMathOperator{\BUNDLE}{BNDL}
\DeclareMathOperator{\ITEM}{ITEM}
\DeclareMathOperator{\SD}{SD}
\DeclareMathOperator{\UNIF}{UNIF}
\DeclareMathOperator{\FAV}{FAVE} 
\DeclareMathOperator{\NONFAV}{NONFAVE} 
%\DeclareMathOperator{\SP}{\text{SP}}
\DeclareMathOperator{\PP}{PP}

\newcommand{\exquantspace}{\constrained\mathcal{Q}}

\newagentvar{gap}{\delta}


%\DeclareMathOperator{\welfare}{welfare}
\newagentvar[\starred]{calloc}{\alloc}
\newcommand{\welfare}{\text{\textbf{welfare}}}

\newcommand{\PO}{\text{PP}}
\newcommand{\allocPO}{\alloc_\PO}
\newcommand{\VCGL}{\text{VCG}_k}
\newcommand{\allocVCGL}{\alloc_{\VCGL}}
\newcommand{\CL}{\text{Clinch}_k}
\newcommand{\allocCL}{\alloc_{\CL}}
\newcommand{\CC}{\text{Clinch}}
\newcommand{\allocCC}{\alloc_{\CC}}

\newcommand{\allocAP}{\alloc_\text{AP}}
\newcommand{\aalloc}{z}
\newcommand{\event}{\mathcal{E}}

\newcommand{\valp}{\val\primed}
\newcommand{\valdp}{\val\doubleprimed}
\newcommand{\dvp}{\lambda(\valdp - 1)}
\newcommand{\sdk}{\sum_{k=\valp+1}^\highestval\frac{\highestval - k + 1}{k - 1}}
\newcommand{\mt}{Z}
\newcommand{\allocspace}{\mathcal{X}}
\newcommand{\MECHS}{\text{MECHS}}
\newcommand{\DISTS}{\text{DISTS}}
\newcommand{\gaplowerbound}{1.013}
\newcommand{\clinchinglowerbound}{1.03}



\newcommand{\lambdas}{\mathbold \lambda}
\newcommand{\Lambdas}{\mathbf \Lambda}
\newcommand{\betas}{\mathbold \beta}
\newcommand{\mus}{\mathbold \mu}



\newcommand{\R}{\mathbb R}
\newcommand{\alphaPrivate}
{\left(1 + 3\budgetQuantile - \frac{1}{\budgetQuantile} \right)}
% \newcommand{\APprivate}
% {(\alphaprivate)(\betaprivate)\rho}
% % {
% % \tfrac{(\budgetQuantile^2+2\budgetQuantile-1)
% % (\budgetQuantile^2+\budgetQuantile-1
% % )}
% % {\budgetQuantile^2-1}
% % \rho}
% \newcommand{\alphaprivate}
% {\budgetQuantile+2}
% % {\tfrac{\budgetQuantile^2+2\budgetQuantile-1}
% % %{\tfrac{(\budgetQuantile^2+2\budgetQuantile-1)}
% % {\budgetQuantile}}
% \newcommand{\betaprivate}
% {\budgetQuantile+1}
% % {\tfrac{\budgetQuantile
% % (\budgetQuantile^2+\budgetQuantile-1)}
% % {\budgetQuantile^2-1}}
% %{(\budgetQuantile^2-1)}}
% \newcommand{\alphaPrivateMHR}{(2e-1)}
% \newcommand{\betaPrivateMHR}{1}

\newcommand{\seq}{{\bf o}}

\newcommand{\seqprices}{{\{\pricei\}_{i=1}^n}}
\newcommand{\seqquants}{{\{\quanti\}_{i=1}^n}}
\newcommand{\randomseqprices}{{\{\randompricei\}_{i=1}^n}}
\newcommand{\randomseqquants}{{\{\randomquanti\}_{i=1}^n}}
\newcommand{\quantTorandomprice}{{RP}}

\newcommand{\randomseqpricesprimed}{{\{\randomprice\primed_i\}_{i=1}^n}}

\newcommand{\seqpricesprimed}{{\{\price\primed_i\}_{i=1}^n}}

\newcommand{\linearapproxratio}{\gamma}

\newcommand{\exanteprobability}{\hat{q}}
\newcommand{\quasilinearquantile}{q^L}
\newcommand{\exantelinearrev}{R^L}
\newcommand{\postlinearcurve}{P^L}
\newcommand{\pricerev}{{\rm AP}}
\newcommand{\seqpricerev}{{\rm SPR}}
\newcommand{\seqpricewel}{{\rm SPW}}
\newcommand{\seqquantpayoff}{{\rm SPP}}
\newcommand{\obquantpayoff}{{\rm OPP}}
\newcommand{\obpricerev}{{\rm OPR}}
\newcommand{\obpricewel}{{\rm OPW}}
\newcommand{\obquantrev}{{\rm OPR}}
\newcommand{\obquantwel}{{\rm OPW}}
% \newcommand{\WEL}{{\rm WEL}}
\newcommand{\pricelinearrev}{AP^L}
\newcommand{\exanteprice}{\hat{p}}
\newcommand{\cumpricelinear}{\cumprice^L}
\newcommand{\correspondingprice}{\price\primed}
\newcommand{\correspondingquant}{\quant\primed}
\newcommand{\EX}{{\rm EX}}
\newcommand{\EXS}{{\rm EX\primed}}
\newcommand{\EXL}{{\rm EX\doubleprimed}}
\newcommand{\EXM}{{\rm EX\tripleprimed}}
\newcommand{\APF}{\tau}
\newcommand{\APFS}{\tau\primed}
\newcommand{\APFL}{\tau\doubleprimed}
\newcommand{\APFM}{\tau\tripleprimed}
\newcommand{\RevAPFMww}{\Rev[\wealth]{\APFM_\wealth}}
\newcommand{\RevAPFMwEw}{\Rev[\wealth^*]{\APFM_\wealth}}
\newcommand{\RevAPFww}{\Rev[\wealth]{\APFL_\wealth}}
\newcommand{\RevAPFwEw}{\Rev[\wealth^*]{\APFL_\wealth}}
\newcommand{\RevPPw}{\Rev[\wealth]{\price}}
\newcommand{\RevPPEw}{\Rev[\wealth^*]{\price}}


\newcommand{\revcurveT}{\revcurve_{\scaleto{T}{4pt}}}
\newcommand{\cumpriceT}{\cumprice_{\scaleto{T}{4pt}}}
\newcommand{\valT}{\val_{\scaleto{T}{4pt}}\primed}
\newcommand{\quantT}{\quant_{\scaleto{T}{4pt}}}

\newagentvar{distribution}{F}
\newcommand{\instance}{\mathcal{I}}
\newcommand{\agent}{i}
\newcommand{\agents}{V}
% \newcommand{\distribution}{\mathcal{D}}
\newcommand{\agentsnum}{n}
\newcommand{\linearinstance}{\mathcal{I}^L}
\newcommand{\lineardistributions}{\mathcal{D}^L}
\newcommand{\lineartypespace}{\mathcal{T}^L}
\newcommand{\linearutil}{u^L}

\newcommand{\exanterelax}{{\rm EAR}}
\newcommand{\exantewel}{{\rm EAR}}


\newcommand{\priceToQuantile}{Q}
\newcommand{\budgetQuantile}{\kappa}

\newcommand{\capacity}{C}
\newcommand{\mincapacity}{\underaccent{\bar}{C}}
\newcommand{\maxval}{\hval}

\newcommand{\myersonReserve}{m^*}
\newcommand{\optimalReserve}{m^*_\cumprice}

\newcommand{\valfunc}{V}
\newcommand{\optquant}{\hat{\quant}}

% \newcommand{\remainingprob}{\tau}
% \newcommand{\remainpricingprob}{\tau\primed}

% \newcommand{\distributions}{\boldsymbol\mathcal{D}}
%\newcommand{\typespaceset}{{\boldsymbol\mathcal{T}}}
%\newcommand{\utils}{{\bf u}}

\newagentvar{cumpayoff}{Y}
\newagentvar{payoffcurve}{Z}

\newcommand{\virtualcurve}{\Phi(\cumpayoff)}
\newcommand{\virtualcurvei}{\Phi_i(\cumpayoffi)}

\newcommand{\payoffHull}{\bar{\cumpayoff}}
% \newcommand{\concaveHull}{\bar{\cumprice}}
% \newcommand{\welfareHull}{\bar{\cumwelfare}}
\newcommand{\concaveHull}{\payoffHull}
\newcommand{\welfareHull}{\payoffHull}
\newcommand{\availableprob}{\varsigma}
\newcommand{\feasibleprob}{\varsigma\primed}
\newcommand{\randomavailableprob}{\varsigma\doubleprimed}


\newcommand{\normalization}{\varpi}
\newcommand{\budgetnum}{m}


\newcommand{\marginP}{\alloc^*_\wealth}
\newcommand{\marginW}{\alloc^\sharp_\wealth}

\newcommand{\AP}{{\rm AP}}
\newcommand{\SPP}{{\rm SPP}}


\newcommand{\mhrbound}{3}

\newcommand{\improvedAP}
{\max\{\alpha, \sqrt{\alpha\beta \eta}\}}


\newcommand{\threshold}{\varrho}
%\newcommand{\threshold}{\sqrt{\sfrac{\alpha \beta}{ \eta}}}


\newcommand{\group}{G}
\newcommand{\improvedAPln}{4\max\{\alpha, \eta \} 
\linearapproxratio \cdot \ln \beta }


\newcommand{\truncateCumprice}{\bar{\cumprice}}
\newcommand{\truncateExante}{\bar{\revcurve}}
\newcommand{\truncateHull}{\bar{\concaveHull}}

\newcommand{\marketclearing}{\price^\quant}

\newcommand{\prophetPrice}{\tau}

\newagentvar{budgetdist}{G}

\newcommand{\correlationgap}{\sfrac{e}{(e-1)}}
\newcommand{\kunit}{\sfrac{1}{(1-\sfrac{1}{\sqrt{2\pi k}})}}


\newcommand{\alloclow}{\alloc_L}
\newcommand{\allochigh}{\alloc_H}
\newcommand{\allocq}{\alloc_\quant}


\newcommand{\randprice}{\Tilde{\price}}
\newcommand{\virtual}{\phi}

\newcommand{\payfrac}{\alpha}
\newcommand{\allocfrac}{\beta}
\newcommand{\newbid}{\tilde{\bid}}
\newagentvar{givenalloc}{\tilde{\alloc}}



\newcommand{\sample}{s}
\newcommand{\scale}{\alpha}

\newcommand{\piratio}{\beta}

\newcommand{\bidmech}{sample-bid mechanism}
\newcommand{\monopq}{\monoq}
\newcommand{\monopr}{\monop}
\newcommand{\aq}{a}
\newcommand{\density}{f}
\newcommand{\qb}{\frac{\aq - \scale\monopq}{\val(1-\monopq)}}

\newcommand{\wel}{w}
% \newcommand{\mq}{\bar{\quant}}
\newcommand{\qhat}{\hat{\quant}}
\newcommand{\vhat}{\hat{\val}}
\newcommand{\bhat}{\hat{\bid}}

\newcommand{\criticalval}{\val^*}
\newcommand{\criticalquant}{\quant^*}
\newcommand{\vl}{\underline{\val}}
\newcommand{\ql}{\underline{\quant}}
\newcommand{\pscale}{0.7}

\newcommand{\priceval}{\price}
\newcommand{\pricequantlowerbound}{\underbar{$\priceval$}}

\newcommand{\midwelfare}{w}
\newcommand{\monoalphaq}{\quant\doubleprimed}
\newcommand{\qtilde}{\tilde\quant}
\newcommand{\vtilde}{\tilde\val}
\newcommand{\revM}{\mathbb{M}_r}
\newcommand{\nonrevM}{\mathbb{M}}
% \newcommand{\MECHS}{\mathbb{M}}
% \newcommand{\inalloc}{\tilde{\alloc}}
% \newcommand{\inprice}{\tilde{\price}}
\newcommand{\allocbid}{\tilde{\alloc}}
\newcommand{\pricebid}{\tilde{\price}}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
\newcommand{\payoff}{v}
\newcommand{\payoffi}{\payoff_{\agent}}

==> Notes/old-model.tex <==
\newpage

\section{Old Model}
Here we consider the following 
version of the facility location problem.

\begin{itemize}
\item A city consists of neighborhoods $V=[n]$. Neighborhood $i$ has population $N_i$.
\item $\alpha_{ij}$ fraction of population $N_i$ visits neighborhood $j$ on a given day.
\item The distance between adjacent neighborhoods $i$ and $j$ is $c(i,j)$.
\item A brand has stores in locations $S\subset V$.
\item Individuals visit one of the stores of the brand in the vicinity of where they live or visit. Specifically, 
\begin{itemize}
	\item Consider an individual of type $(i,j)$ who lives at $i$ and visits $j$. 
	\item Let $d_i(S)$ denote the distance of the closest store to $i$ (defined wrt the above distances).
	\item Type $(i,j)$ individual visits a store at a rate $$r_{ij}(S)= \frac{\exp(-d_i(S))+\exp(-d_j(S)) }{C+\exp(-d_i(S))+\exp(-d_j(S))}$$ 
	for some $C>0$.
	\item Here other decreasing functions of distance could be plausible. The above is consistent with a choice model (where the disutility of visiting a store scales linearly with distance).
\end{itemize}
\end{itemize}

A firm decides where to place its $K$ stores with the objective of maximizing total sales. Formally, we want to solve the firm's problem :
	$$ \max_{S: \abs{S}= K} \sum_i \sum_j N_i \alpha_{ij} r_{ij}(S).
$$



==> Notes/scaled-greedy.tex <==
\section{An Improved 2.5-approximation Algorithm}

% \newcommand{\costscalarinverse}{\alpha}


In this section, we present a modified version of the 2-Chance Greedy Algorithm with an improved approximation guarantee. 
We start with the following observation.
{\color{red}
\begin{lemma}
\label{lem:scaled opening cost}
    If there exists a polynomial-time algorithm $\ALG$
    such that every FLP instance $\instance$ and any solution $\SOL\subseteq[n]$,
    \begin{align}
    \label{eq:scaled approximation guarantee}
        \frac{1}{\costscalar} \CostF[\instance]{\ALG}
        +
        \CostC[\instance]{\ALG}
        \geq 
        \approxratio \cdot 
        \left(
        \frac{1}{\costscalar} \CostF[\instance]{\SOL}
        +
        \CostC[\instance]{\SOL}
        \right)
    \end{align}
    then there exists an polynomial-time algorithm $\ALG\primed$
    with approximation ratio $\approxratio$. 
    Here $\CostF[\instance]{\ALG}$, $\CostC[\instance]{\ALG}$,
    $\CostF[\instance]{\SOL}$, $\CostC[\instance]{\SOL}$
    are the facility opening cost and individual connection cost for algorithm $\ALG$ and solution $\SOL$
    under instance $\instance$, respectively.
\end{lemma}
\begin{proof}
    Consider the following algorithm $\widetilde{\ALG}$:
    For every instance $\instance = (n, \distance, 
\{\flowe\}_{\edge\in\Edge}, \opencosts_{i\in[n]})$, construct a modified instance $\instance\primed = (n, \distance, 
\{\flowe\}_{\edge\in\Edge}, \opencosts\primed_{i\in[n]})$ with modified facility opening cost $\opencosti\primed = \costscalar\cdot \opencosti$. 
    Namely, the modified instance $\instance\primed$ is the same as the original instance $\instance$, except that its facility opening costs are scaled up by a multiplicative factor of $\costscalar$ from the original instance.
    Invoke algorithm $\ALG$ on the modified instance $\instance\primed$ and return its solution.

    \paragraph{Running time.} It is straightforward to verify that the algorithm described above is polynomial-time, since its subroutine $\ALG$ is polynomial-time.

    \paragraph{Approximation guarantee.}
    Let $\SOL = \ALG(\instance\primed)$ be the solution returned by algorithm $\ALG$ for the modified instance $\instance\primed$,
    and $\OPT$ be the optimal solution for instance $\instance$.
    Note that 
    \begin{align*}
        \Cost[\instance]{\widetilde{\ALG}}
        &=
        \CostF[\instance]{\SOL}
        +
        \CostC[\instance]{\SOL}
        \\
        &\overset{(a)}{=} 
        \frac{1}{\costscalar}\CostF[\instance\primed]{{\SOL}}
        +
        \CostC[\instance\primed]{{\SOL}}
        \\
        &\overset{(b)}{\geq} 
        \approxratio\cdot 
        \left(
        \frac{1}{\costscalar}\CostF[\instance\primed]{{\OPT}}
        +
        \CostC[\instance\primed]{{\OPT}}
        \right)
        \\
        &\overset{(c)}{=}  
        \approxratio\cdot 
        \left(
        \CostF[\instance]{\OPT}
        +
        \CostC[\instance]{\OPT}
        \right)
        % \\
        % &
        = 
        \approxratio\cdot 
        \Cost[\instance]{\OPT}
    \end{align*}
    where equalities~(a) (c) holds due to the construction of 
    the modified instance $\instance\primed$,
    and inequality holds due to the assumption of algorithm $\ALG$ in the lemma statement.
\end{proof}}

Inspired by \Cref{lem:scaled opening cost}, we consider the following modified version of 
the 2-Chance Greedy Algorithm, which scales the facility opening costs up by a factor of $\costscalar$. See \Cref{alg:greedy modified v2}.

\input{Paper/alg-2-choice-greedy-v2}


\begin{lemma} 
\label{lem:weakly factor-revealing program scaled}
For any $\discountfactor \in[0, 1]$ and
$\costscalar \in [1, 1 + \discountfactor]$,
the (original) 2-Chance Greedy Algorithm (i.e., \Cref{alg:greedy modified}) with discount factor $\discountfactor$
satisfies inequality~\eqref{eq:scaled approximation guarantee} 
in \Cref{lem:scaled opening cost} with $$\approxratio =  \sup\limits_{\mHat\in\naturals, 
\permu
% \in[\mHat]^{\positivereals}
:[\mHat]\rightarrow\positivereals}
\Obj{\text{\ref{eq:weakly factor-revealing program scaled}}}$$
Here \ref{eq:weakly factor-revealing program scaled}
is the maximization program parameterized by 
$\mHat\in\naturals$ 
and $\permu:[\mHat]\rightarrow\positivereals$
defined as follows:
\begin{align}
\tag{$\WFRP{\mHat,\permu,\discountfactor, \costscalar}$}
\label{eq:weakly factor-revealing program scaled}
&\arraycolsep=1.4pt\def\arraystretch{2.2}
    \begin{array}{llll}
    \max\limits_{
    \substack{\costHat\geq 0,
    \\
    \muHatBf,
    \distanceHatBf,
    \distanceHatStarBf \geq 
    \zerobf
    }} &
    {\color{red}
    \displaystyle\sum\nolimits_{\ell\in[\mHat]}
    \frac{1 + \discountfactor}{\costscalar}
    \cdot
    \muHat(\ell) - 
    \left(
    \frac{1 + \discountfactor}{\costscalar} - 1
    \right)\cdot\distanceHatStar(\ell)}
    & \text{s.t.} & \\
    \WFRCtriangleineq &
    \discountfactor\cdot \muHat(\ell') \leq 
    \distanceHatStar(\ell) + \distanceHat(\ell)
    +
    \distanceHat(\ell')
    &
    \ell,\ell'\in[\mHat],
    \permu(\ell) < \permu(\ell')
    &
    \\
    \WFRCcontribution &
    \displaystyle\sum\nolimits_{\ell'\in[\mHat]:
    \permu(\ell') \geq \permu(\ell)}
    \plus{\discountfactor\cdot 
    \min\left\{\muHat(\ell), \muHat(\ell')\right\} - \distanceHat(\ell')}
    \leq \costHat\quad
    &
    \ell \in[\mHat]
    \\
    \WFRCconnectcost &
    \distanceHatStar(\ell) \leq \muHat(\ell)
    &
    \ell\in[\mHat]
    \\
     \WFRCtotalcost &
     {\color{red}\frac{1}{\costscalar}\cdot}\costHat 
     +
     \displaystyle\sum\nolimits_{\ell\in[\mHat]}
     \distanceHat(\ell)
     \leq 1
     &
    \end{array}
\end{align}
\end{lemma}

\begin{remark}
    The objective function in program~\ref{eq:weakly factor-revealing program scaled}
    can be simplified as $\sum_{\ell\in[m]}\muHat(\ell)$
    when $1 + \discountfactor = \costscalar$,
    and, in particular,
    $\discountfactor = 1$, $\costscalar = 2$.
\end{remark}


Combining \Cref{lem:scaled opening cost} and \Cref{lem:weakly factor-revealing program scaled}, we know that 
\Cref{alg:greedy modified v2} with discount factor $\discountfactor$ 
and opening cost scalar $\costscalar$ achieves an approximation ratio of 
$$\sup\limits_{\mHat\in\naturals, 
\permu
% \in[\mHat]^{\positivereals}
:[\mHat]\rightarrow\positivereals}
\Obj{\text{\ref{eq:weakly factor-revealing program scaled}}}$$
Note that following the same batching argument, we obtain a modified version of strongly factor-revealing program \ref{eq:strongly factor-revealing quadratic program} and thus the approximation ratio can be numerically computed.

\begin{proposition}
    Modified program~
    % d$\mathcal{P}_{\texttt{SFR}}(n = 20, \gamma = 1, \eta = 2) \leq 2.502$, and 
    $\mathcal{P}_{\texttt{SFR}}(n = 25, \gamma = 1, \eta = 2) \leq 2.497$.
\end{proposition}

Below we sketch the proof of \Cref{lem:weakly factor-revealing program scaled}.
The analysis follows the same structure as the one for \Cref{lem:weakly factor-revealing program}. We highlight the main changes in {\color{red}red}.

{\color{red}
\paragraph{Step 0- structural properties of the 2-Chance Greedy.} 
Note that \Cref{lem:scaled opening cost} considers the original 2-Chance Greedy Algorithm (\Cref{alg:greedy modified}),
instead of the modified 2-Chance Greedy Algorithm (\Cref{alg:greedy modified v2}). 
Thus, all three structural properties in \Cref{lem:structural lemma} hold exactly.
}

\begin{comment}
\paragraph{Step 1- lower bound of the optimal cost via configuration LP.} 
Given an \TWOLFLP\ instance,
the optimal solution can be formulated as an integer program as 
follows.
We define a \emph{service region}
$\starinstance = (i,\EdgeTilde)$
is a tuple that 
consists a facility at location $i$ 
and a subset edges $\EdgeTilde\subseteq\Edge$
that are served by facility $i$.
Let $\starspace \triangleq [n]\times 2^{\Edge}$
be the set of all possible service regions.
With a slight abuse of notation, for every service region
$\starinstance = (i, \EdgeTilde)\in\starspace$,
{\color{red}
we define its cost as
$\cost(\starinstance)
\triangleq \frac{1}{\costscalar}{\opencost_i}
    +
    {
    \sum_{\edge\in\EdgeTilde}
    \flowe\cdot \distance(\edge, i)}$
    where the first term is the scaled facility opening cost in location $i$,}
    and the second term is the total 
    connection cost between edge $\edge$ and facility $i$
    over all edge~$\edge\in\EdgeTilde$.
To capture the optimal solution, consider an integer program
where each service region $\starinstance=(i,\EdgeTilde)$ 
is associated with 
a binary variable $\allocstar$
indicating whether the optimal solution 
opens facility $i$ and serves every edge $\edge\in\EdgeTilde$
through facility $i$.
Below we present its linear program relaxation~\ref{eq:lp relaxtion}
as well as its dual program.
\begin{align}
\tag{$\mathcal{P}_{\texttt{OPT}}$}
\label{eq:lp relaxtion scaled}
    \arraycolsep=5.4pt\def\arraystretch{1}
    &\begin{array}{llllll}
    \min\limits_{\mathbf\alloc\geq \zerobf} &
    \displaystyle\sum\nolimits_{\starinstance\in\starspace} 
    \coststar \cdot \allocstar 
    & \text{s.t.} &
    \quad
    \max\limits_{\boldsymbol{\dual}\geq \zerobf} &
    \displaystyle\sum\nolimits_{\edge\in\Edge} 
    \duale
    & \text{s.t.} \\
    & \displaystyle\sum\nolimits_{\starinstance=(i, \EdgeTilde):
     \edge \in \EdgeTilde} 
     \allocstar \geq 1
     \quad
     & 
     \edge \in \Edge
     &
    &\displaystyle\sum\nolimits_{
     \edge \in \EdgeTilde} 
     \duale \leq \coststar
     \quad
     & 
     \starinstance = (i, \EdgeTilde)\in\starspace
    \end{array}
\end{align}
We formalize the connection between the optimal solution 
and program~\ref{eq:lp relaxtion scaled}
in \Cref{lem:lp relaxation scaled}.
\begin{lemma}
% {lemma}{lprelaxationscaled}
\label{lem:lp relaxation scaled}
Given any \TWOLFLP\ instance and any solution $\SOL$
the optimal {\color{red}scaled cost $\frac{1}{\costscalar}\CostF{\SOL} + \CostC{\SOL}$} is at least $\Obj{\text{\ref{eq:lp relaxtion}}}$.
\end{lemma}
\end{comment}


\paragraph{Step 2-
dual assignment construction.}
In this step, we construct the dual assignment~\eqref{eq:dual assignment}
of program~\ref{eq:lp relaxtion}
based on the execution path of the 2-Chance Greedy Algorithm.
Then we argue that the total cost of the algorithm
is at most the objective value of the constructed dual assignment (\Cref{lem:dual assignment objective value scaled}).
Combining with an argument that the constructed dual assignment is also 
approximately feasible presented in the step~3 (\Cref{lem:dual assignment approx feasible scaled}), 
the weak duality of linear program 
completes the proof of \Cref{lem:weakly factor-revealing program scaled}.

Let $\stores$ be the solution computed by \Cref{alg:greedy modified}.
Let $\{\greedycounter(\edge)\}$
and $\{\connectmapping(\edge,\edgeindex)\}_{
\edge\in\Edge,\edgeindex\in\hwset}$
be the values of these variables at the termination of \Cref{alg:greedy modified}.
We partition all edges $\edge\in\Edge$ into two disjoint subsets  
$\singlecountedgeset$
and $\doublecountedgeset$ 
% and 
 as follows: 
\begin{align*}
    \doublecountedgeset &\triangleq
    \{\edge\in\Edge: \connectmapping(\edge,h) \not= \nullsymbol
    \land 
    \connectmapping(\edge,w)  \not= \nullsymbol
    \land 
    \connectmapping(\edge,h) \not = \connectmapping(\edge,w)\}
    \qquad
    \singlecountedgeset \triangleq
    \Edge\backslash\doublecountedgeset
\end{align*}
Namely, $\singlecountedgeset$
contains every edge $\edge\in\Edge$ 
that is either partially connected or fully connected to 
a single facility;
while $\doublecountedgeset$
contains every edges$\edge\in\Edge$ 
that is fully connected to 
two facilities.

{\color{red}To simplify the presentation, without loss of generality,
we assume $\connectmapping(\edge,h)\in\stores$ for every individual on edge $\edge \in \singlecountedgeset$,
and $\distance(\edgehome, \connectmapping(\edge,h)) \leq 
 \distance(\edgework, \connectmapping(\edge,w))$
 for every individual on edge $\edge \in \doublecountedgeset$.}
Now,
consider the dual assignment (which is not feasible in the dual problem in general)
constructed
as follows,{\color{red}
\begin{align}
\label{eq:dual assignment scaled}
\begin{split}
    \edge\in\singlecountedgeset:&\qquad
    \duale \gets 
    \flowe\cdot 
    \left(\frac{1+\discountfactor}{\costscalar}
    \cdot \greedycounter(\edge)
    -
    \left(
    \frac{1 + \discountfactor}{\costscalar} - 1
    \right)
    \cdot 
    \distance(\edgehome, \connectmapping(\edge,h))
    \right)
    \\
    % \edge\in\doublecountedgeset:&\qquad
    % \duale \gets \flowe\cdot 
    % \left(
    % \frac{1 + \discountfactor}{\costscalar} \cdot \greedycounter(\edge) - 
    %  \left(
    % \frac{1 + \discountfactor}{\costscalar} - 1
    % \right) 
    % \cdot \max\{
    % \distance(\edgehome, \connectmapping(\edge,h)),
    % \distance(\edgework, \connectmapping(\edge,w))
    % \}
    % \right)
    \edge\in\doublecountedgeset:&\qquad
    \duale \gets \flowe\cdot 
    \left(
    \frac{1 + \discountfactor}{\costscalar} \cdot \greedycounter(\edge) 
    - 
    \frac{1}{\costscalar}
    \left(
    \distance(\edgehome, \connectmapping(\edge,h))
    +
    \distance(\edgework, \connectmapping(\edge,w))
    \right)
    +
    \distance(\edgehome, \connectmapping(\edge,h))
    \right)
\end{split}
\end{align}} 
The construction of \Cref{alg:greedy modified}
ensures that the {\color{red}scaled} cost of solution $\stores$
is upperbounded by the objective value of the constructed dual assignment.
We formalize this in \Cref{lem:dual assignment objective value scaled}.
\begin{lemma}
% {lemma}{dualassignmentobjectivevaluescaled}
\label{lem:dual assignment objective value scaled}
Given any \TWOLFLP\ instance,
the {\color{red}scaled cost $\frac{1}{\costscalar}\CostF{\stores} + \CostC{\stores}$}
of solution $\stores$ computed by \Cref{alg:greedy modified}
with discount factor $\discountfactor\in[0, 1]$
is at most the objective value of program~\ref{eq:lp relaxtion scaled}
with
the dual assignment \eqref{eq:dual assignment scaled},
i.e., {\color{red}$\frac{1}{\costscalar}\CostF{\stores} + \CostC{\stores} \leq \sum_{\edge\in\Edge}\duale$}.
\end{lemma}

\begin{proof}
{\color{red}
By the dual assignment~\eqref{eq:dual assignment scaled}, we have
\begin{align*}
    \sum_{\edge\in\Edge}\duale
    % \\
    =&
    \sum_{\edge \in \singlecountedgeset}
    \flowe\cdot 
    \left(
    \frac{1+\discountfactor}{\costscalar}
    \cdot \greedycounter(\edge)
    -
    \left(
    \frac{1 + \discountfactor}{\costscalar} - 1
    \right)
    \cdot 
    \distance(\edgehome, \connectmapping(\edge,h))
    \right)
    \\
    &\quad +
    \sum_{\edge \in \doublecountedgeset}
    \flowe\cdot 
    \left(
    \frac{1 + \discountfactor}{\costscalar} \cdot \greedycounter(\edge) 
    - 
    \frac{1}{\costscalar}
    \left(
    \distance(\edgehome, \connectmapping(\edge,h))
    +
    \distance(\edgework, \connectmapping(\edge,w))
    \right)
    +
    \distance(\edgehome, \connectmapping(\edge,h))
    \right)
\end{align*}
We analyze the term of each individual on each edge $\edge$ on the right-hand side separately. 
For each individual on edge $\edge \in \singlecountedgeset$,
we have
\begin{align*}
    &~\frac{1+\discountfactor}{\costscalar}
    \cdot \greedycounter(\edge)
    -
    \left(
    \frac{1 + \discountfactor}{\costscalar} - 1
    \right)
    \cdot 
    \distance(\edgehome, \connectmapping(\edge,h))
    \\
    =&~
    \frac{1+\discountfactor}{\costscalar}
    \cdot 
    \left(
    \greedycounter(\edge)
    -
    \distance(\edgehome, \connectmapping(\edge,h))
    \right)
    +
    \distance(\edgehome, \connectmapping(\edge,h))
    \\
    \geq&~
    \frac{1}{\costscalar}
    \cdot 
    \left(
    \greedycounter(\edge)
    -
    \distance(\edgehome, \connectmapping(\edge,h))
    \right)
    +
    \distance(\edgehome, \connectmapping(\edge,h))
\end{align*}
where the last inequality holds since $\greedycounter(\edge)
    \geq 
    \distance(\edgehome, \connectmapping(\edge,h))$,
    which is implied by the construction of the 2-Chance Greedy Algorithm.

For each individual on edge $\edge \in \doublecountedgeset$, we have
\begin{align*}
    &~\frac{1 + \discountfactor}{\costscalar} \cdot \greedycounter(\edge) 
    - 
    \frac{1}{\costscalar}
    \left(
    \distance(\edgehome, \connectmapping(\edge,h))
    +
    \distance(\edgework, \connectmapping(\edge,w))
    \right)
    +
    \distance(\edgehome, \connectmapping(\edge,h))
    \\
    =&~
    \frac{1}{\costscalar}
    \cdot 
    \left(
    (1+\discountfactor)
    \greedycounter(\edge)
    -
    \distance(\edgehome, \connectmapping(\edge,h))
    -
    \distance(\edgework, \connectmapping(\edge,w))
    \right)
    +
    \distance(\edgehome, \connectmapping(\edge,h))
\end{align*}
Combining two pieces together,
we obtain
\begin{align*}
    \sum_{\edge\in\Edge}\duale &\geq 
    \frac{1}{\costscalar}
    \cdot 
    \left(
    \sum_{\edge\in\singlecountedgeset} 
    \flowe \cdot 
    \left(
    \greedycounter(\edge)
    -
    \distance(\edgehome, \connectmapping(\edge,h))
    \right)
    +
    \sum_{\edge\in\doublecountedgeset}
    \flowe \cdot  \left(
    (1+\discountfactor)
    \greedycounter(\edge)
    -
    \distance(\edgehome, \connectmapping(\edge,h))
    -
    \distance(\edgework, \connectmapping(\edge,w))
    \right)
    \right)
    \\
    &\qquad +
    \sum_{\edge\in\Edge} \flowe\cdot \distance(\edgehome, \connectmapping(\edge,h))
\end{align*}
To finish the proof, note that the construction of the 2-Chance Greedy Algorithm implies that 
the first term on the right-hand side is equal to the facility opening cost of solution $\SOL$, and the second term on the right-hand side is at most the connection cost of solution $\SOL$.
}
\end{proof}

\paragraph{Step 3- approximate feasibility of dual assignment.}
It is straightforward to verify that the constructed dual assignment is non-negative, i.e., 
$\duale \geq 0$
for every edge $\edge\in\Edge$.
It remains to show that for each service region $\starinstance
=(i, \EdgeTilde)\in\starspace$,
the dual constraint associated with primal variable 
$\allocstar$
is approximately satisfied (with an approximation factor of $\Obj{\WFRP{\mHat,\permu,\discountfactor, \costscalar}}$
for some parameters $\mHat,\permu$ depending on $\starinstance$.
We formalize this
 in \Cref{lem:dual assignment approx feasible scaled}.

\begin{lemma}
% {lemma}{dualassignmentapproxfeasiblescaled}
\label{lem:dual assignment approx feasible scaled}
Given any \TWOLFLP\ instance,
for each service region $\starinstance
=(i, \EdgeTilde)\in\starspace$,
the dual assignment \eqref{eq:dual assignment scaled}
in program~\ref{eq:lp relaxtion scaled}
is approximately feasible up to 
multiplicative factor $\WFRapproxratio$ where
$$\WFRapproxratio = \sup\nolimits_{\mHat\in\naturals,
\permu:[\mHat]\rightarrow\positivereals}
\Obj{\WFRP{\mHat,\permu,\discountfactor, \costscalar}}$$
In particular,  
fix an arbitrary
service region $\starinstance
=(i, \EdgeTilde)\in\starspace$,
let
$\edgetoellmapping:\EdgeTilde\rightarrow[\mHat]$ 
be an arbitrary bijection 
from $\EdgeTilde$ to $[\mHat]$.
Consider $\mHat = |\EdgeTilde|$,
and $\permu(\edgetoellmapping(\edge)) = 
\permuTGD(\edge,\config_i(\edge))$
for every edge $\edge\in\EdgeTilde$.\footnote{Recall
that $\permuTGD$, $\config_i$
are defined in \Cref{lem:structural lemma}.
For ease of presentation, in step 3 we make the assumption
that $\flowe \equiv 1$ for every edge $\edge\in\EdgeTilde$. 
This assumption is without loss of generality, since our argument
can be directly extended by resetting $\mHat$
equal to the total populations over all edges in $\EdgeTilde$,
i.e., $\mHat= \sum_{\edge\in\EdgeTilde}\flowe$, and treat each
of those individuals separately.}
\begin{align*}
% \label{eq:dual feasibility approx}
    \sum\nolimits_{\edge\in\EdgeTilde}\duale \leq \Obj{\WFRP{\mHat,\permu,\discountfactor, \costscalar}}
    \cdot \coststar
\end{align*}
\end{lemma}
At a high level, 
for every \TWOLFLP\ instance,
and every service region $\starinstance
=(i,\EdgeTilde)$,
we construct a solution of program~\ref{eq:weakly factor-revealing program scaled}
based on the \TWOLFLP\ instance
as well as the execution path of the 
2-Chance Greedy Algorithm as follows,
\begin{align*}
    &\qquad\costHat\primed \gets \normalizefactor \cdot {\opencost_i},
    \\
    \edge\in\EdgeTilde:&
    \qquad
    \muHat\primed(\edgetoellmapping(\edge)) \gets 
    \normalizefactor \cdot {\greedycounter(\edge)},
    \quad 
    \distanceHat\primed(\edgetoellmapping(\edge)) \gets 
    \normalizefactor \cdot 
    {\distance(\edge, i)},
    \\
    \edge\in\EdgeTilde\cap \singlecountedgeset:
    &\qquad
    \distanceHatStar\primed(\edgetoellmapping(\edge)) \gets 
    \normalizefactor\cdot {\distance(\edgehome, \connectmapping(\edge,h)) },
    \\
    \edge\in\EdgeTilde\cap \doublecountedgeset:
    &\qquad
    \distanceHatStar\primed(\edgetoellmapping(\edge)) \gets 
    \normalizefactor\cdot \distance(
    \edge_{\config_i(\edge)}, \connectmapping(\edge, \config_i(\edge)))
\end{align*}
where {\color{red}$\normalizefactor = \frac{1}{\frac{1}{\costscalar}\opencost_i+\sum_{\edge\in\EdgeTilde}
\distance(\edge, i)}$
is the normalization factor}.
This constructed solution 
of program~\ref{eq:weakly factor-revealing program scaled}
is feasible:
constraints~\WFRCtriangleineq--\WFRCconnectcost\ is satisfied due to \Cref{lem:structural lemma},
and constraint~\WFRCtotalcost\ 
is satisfied due to the normalization factor $\normalizefactor$.
Furthermore, its objective value equals to 
the ratio between $\sum_i\duale$ over
$\coststar$.


\begin{proof}[Proof of \Cref{lem:dual assignment approx feasible scaled}]
Fix an arbitrary 
\TWOLFLP\ instance, and 
an arbitrary service region $\starinstance = (i, \EdgeTilde)\in\starspace$
such that {\color{red}$\frac{1}{\costscalar}
\opencost_i+\sum_{\edge\in\EdgeTilde}\distance(\edge, i) 
> 0$.}\footnote{Otherwise, 
$\greedycounter(\edge) = 0$
for every edge $\edge\in\EdgeTilde$ and thus the dual constraint is satisfied 
with equality trivially.}
We construct a solution
$\{\costHat\primed,\muHat\primed(\ell),\distanceHat\primed(\ell),
\distanceHatStar\primed(\ell)\}$ for program~\ref{eq:weakly factor-revealing program} as follows:\footnote{Here we use superscript $\dagger$
to denote the solution in program~\ref{eq:weakly factor-revealing program}.}
\begin{align*}
    &\qquad\costHat\primed \gets \normalizefactor \cdot {\opencost_i},
    \\
    \edge\in\EdgeTilde:&
    \qquad
    \muHat\primed(\edgetoellmapping(\edge)) \gets 
    \normalizefactor \cdot {\greedycounter(\edge)},
    \quad 
    \distanceHat\primed(\edgetoellmapping(\edge)) \gets 
    \normalizefactor \cdot 
    {\distance(\edge, i)},
    \\
    \edge\in\EdgeTilde\cap \singlecountedgeset:
    &\qquad
    \distanceHatStar\primed(\edgetoellmapping(\edge)) \gets 
    \normalizefactor\cdot 
    \distance(\edgehome, \connectmapping(\edge,h)),
    % {\greedycounter(\edge) },
    \\
    \edge\in\EdgeTilde\cap \doublecountedgeset:
    &\qquad
    \distanceHatStar\primed(\edgetoellmapping(\edge)) \gets 
    \normalizefactor\cdot \distance(\edge_{\config_i(\edge)}, \connectmapping(\edge, \config_i(\edge)))
\end{align*}
where {\color{red}$\normalizefactor = \frac{1}{\frac{1}{\costscalar}\opencost_i+\sum_{\edge\in\EdgeTilde}
\distance(\edge, i)}$
is the normalization factor} which guarantees the feasibility of 
constraint~\WFRCtotalcost.
Moreover, \Cref{lem:structural lemma} and the solution construction
implies the feasibility of constraints~\WFRCtriangleineq, \WFRCcontribution, and
\WFRCconnectcost.

{\color{red}
To prove $\frac{\sum_{\edge\in\EdgeTilde} \duale}{\coststar}$ is upperbounded by the objective value of the constructed solution in program~\ref{eq:weakly factor-revealing program scaled}, it is sufficient to argue that for every $\edge\in \EdgeTilde$, 
\begin{align*}
    \frac{\duale}{\coststar} \leq 
     \frac{1 + \discountfactor}{\costscalar}
     \cdot \muHat\primed(\edgetoellmapping(\edge)) - 
    \left(
    \frac{1 + \discountfactor}{\costscalar} - 1
    \right)
    \cdot \distanceHatStar\primed(\edgetoellmapping(\edge))
\end{align*}
We show this inequality for two different cases separately. 

\smallskip
For each edge $\edge \in \EdgeTilde\cap \singlecountedgeset$, we have
\begin{align*}
     \frac{\duale}{\coststar}
     &\overset{(a)}{=}
     \frac{\frac{1+\discountfactor}{\costscalar}
    \cdot \greedycounter(\edge)
    -
    \left(
    \frac{1 + \discountfactor}{\costscalar} - 1
    \right)
    \cdot 
    \distance(\edgehome, \connectmapping(\edge,h))
    }{\frac{1}{\costscalar}\opencost_i+\sum_{\edge'\in\EdgeTilde}
\distance(\edge', i)}
    \\
     &\overset{(b)}{=}
     \frac{\frac{1+\discountfactor}{\costscalar}
    \cdot \muHat\primed(\edgetoellmapping(\edge))
    -
    \left(
    \frac{1 + \discountfactor}{\costscalar} - 1
    \right)
    \cdot 
    \distanceHatStar\primed(\edgetoellmapping(\edge))
    }{\frac{1}{\costscalar}\opencost\primed+\sum_{\ell\in[m]}
\distance\primed(\ell)}
    \\
    &\overset{(c)}{\leq}
     \frac{1 + \discountfactor}{\costscalar}
     \cdot \muHat\primed(\edgetoellmapping(\edge)) - 
    \left(
    \frac{1 + \discountfactor}{\costscalar} - 1
    \right)
    \cdot \distanceHatStar\primed(\edgetoellmapping(\edge))
\end{align*}
where equality~(a) holds due to $\flowe = 1$ and the dual assignment \eqref{eq:dual assignment scaled};
equality~(b) holds due to the solution construction in program~\ref{eq:weakly factor-revealing program scaled};
and inequality~(c) holds due to constraint~\WFRCtotalcost\ in program~\ref{eq:weakly factor-revealing program scaled}.

\smallskip
For each edge $\edge \in \EdgeTilde\cap \doublecountedgeset$, we have
\begin{align*}
     \frac{\duale}{\coststar}
     &\overset{(a)}{=}
     \frac{    
     \frac{1 + \discountfactor}{\costscalar} \cdot \greedycounter(\edge) 
    - 
    \frac{1}{\costscalar}
    \left(
    \distance(\edgehome, \connectmapping(\edge,h))
    +
    \distance(\edgework, \connectmapping(\edge,w))
    \right)
    +
    \distance(\edgehome, \connectmapping(\edge,h))
    }{\frac{1}{\costscalar}\opencost_i+\sum_{\edge'\in\EdgeTilde}
\distance(\edge', i)}
    \\
     &\overset{}{=}
     \frac{
     \frac{1 + \discountfactor}{\costscalar} \cdot \greedycounter(\edge) 
    - 
    \frac{1}{\costscalar}
    \distance(\edgework, \connectmapping(\edge,w))
    +
    \left(1 - \frac{1}{\costscalar}\right)
    \distance(\edgehome, \connectmapping(\edge,h))
     }{\frac{1}{\costscalar}\opencost_i+\sum_{\edge'\in\EdgeTilde}
\distance(\edge', i)}
    \\
     &\overset{(b)}{\leq}
     \frac{
     \frac{1 + \discountfactor}{\costscalar} \cdot \greedycounter(\edge) 
    - 
    \frac{1}{\costscalar}
    \distance(\edgework, \connectmapping(\edge,w))
    +
    \left(1 - \frac{1}{\costscalar}\right)
    \distance(\edgework, \connectmapping(\edge,w))
     }{\frac{1}{\costscalar}\opencost_i+\sum_{\edge'\in\EdgeTilde}
\distance(\edge', i)}
    \\
     &\overset{(c)}{\leq}
     \frac{\left(\frac{1+\discountfactor}{\costscalar}
    \cdot \muHat\primed(\edgetoellmapping(\edge))
    -
    \left(
    \frac{1 + \discountfactor}{\costscalar} - 1
    \right)
    \cdot 
    \distanceHatStar\primed(\edgetoellmapping(\edge))
    \right)}{\frac{1}{\costscalar}\opencost\primed+\sum_{\ell\in[m]}
\distance\primed(\ell)}
    \\
    &\overset{(d)}{\leq}
     \frac{1 + \discountfactor}{\costscalar}
     \cdot \muHat\primed(\edgetoellmapping(\edge)) - 
    \left(
    \frac{1 + \discountfactor}{\costscalar} - 1
    \right)
    \cdot \distanceHatStar\primed(\edgetoellmapping(\edge))
\end{align*}
where equality~(a) holds due to $\flowe = 1$ and the dual assignment \eqref{eq:dual assignment scaled};
inequality~(b) holds due to the assumption that $\distance(\edgehome, \connectmapping(\edge,h)) \leq 
 \distance(\edgework, \connectmapping(\edge,w))$ introduced in step 2 and $(1 - \sfrac{1}{\costscalar}) \geq 0$;
equality~(c) holds due to the solution construction in program~\ref{eq:weakly factor-revealing program scaled}, the assumption that $\distance(\edgehome, \connectmapping(\edge,h)) \leq 
 \distance(\edgework, \connectmapping(\edge,w))$ introduced in step 2 and $\sfrac{2}{\costscalar} - 1 
 \geq \sfrac{(1 + \discountfactor)}{\costscalar} - 1 \geq 0$;
and inequality~(d) holds due to constraint~\WFRCtotalcost\ in program~\ref{eq:weakly factor-revealing program scaled}.
}
\end{proof}

% Putting all pieces together, we are ready to prove \Cref{lem:weakly factor-revealing program}.
\begin{proof}[Proof of \Cref{lem:weakly factor-revealing program scaled}]
% Consider linear program~\ref{eq:lp relaxtion}.
Invoking 
% \Cref{lem:lp relaxation}, \Cref{lem:dual assignment objective value},
% and
% \Cref{lem:dual assignment approx feasible},
\Cref{lem:lp relaxation scaled,lem:dual assignment objective value scaled,lem:dual assignment approx feasible scaled}
and weak duality of LP finishes the proof.
\end{proof}




==> Notes/todo.tex <==
\section*{Todo}

==> Notes/two-circle-0-0.tex <==
\subsection{Extreme Case: $a = 0$ and $A = 0$}

In this subsection,
we consider an extreme case where 
$a = 0$ and $A = 0$,
i.e., 
all individuals who reside in 
the inner (outer) circle
work in the outer (inner) circle.

In this case, 
\begin{align*}
    \frac{\partial c}{\partial K}
    = 
    - \mu 
 \frac{\pi r^2}{6k^2R}+F
\end{align*}
where the right-hand side does not depend on $K$.
Thus, if the right-hand side is not zero, 
$K^* = 0$ (the other boundary case $K^* =\infty$
is clearly not cost minimizer).
Assuming $K^* = 0$, we can solve $k^*$
by its FOC
\begin{align*}
    \frac{\partial c}{\partial k}=
  - \mu\frac{\pi  r}{2k^2}+f=0
\end{align*}
which implies 
$k^* = \sqrt{\frac{\pi (m + M) r}{2f}}$.
The cost for $(k^*, K^*)$
is
\begin{align*}
    c(k^*,K^*) =
\sqrt{2(m+M)r f}
\end{align*}
Note that this cost 
$c(k^*,K^*)$ 
does not depend on parameter $F, R$
since we implicitly assume 
$\gamma \leq 1$.

We note that the multiplicative gap between
$c(k^*,K^*)$ and 
$c(k_W,K_W)$
can be arbitrary large. 
To see this, 
let $f = F = 1$, 
$m = M = 100$,
and $r = 1$.
Then 
$c(k_W,K_W) = \Theta(R)$
and 
$c(k^*,K^*) = \Theta(\sqrt{R})$.
See \Cref{fig:two-cricle-0-0-ratio}
for a graphical illustration.

\begin{figure}
    \centering
    \includegraphics[scale = 0.7]{figs/two-circle-0-0-ratio.png}
    \caption{Plot 
    of $\frac{c(k_W, K_W)}{c(k^*, K^*)}$
    for $f = F = 1$, 
$m = M = 100$, $r = 1$
and $R \in [1, 10]$.
}
    \label{fig:two-cricle-0-0-ratio}
\end{figure}

==> Notes/two-circle-1-0.tex <==
\subsection{Extreme Case: $a = 1$ and $A = 0$}

In this subsection,
we consider an extreme case where 
$a = 1$ and $A = 0$,
i.e., 
all individuals 
work in the inner circle.

In this case, 
\begin{align*}
    \frac{\partial c}{\partial K}
    = 
    - \mu 
 \frac{\pi r^2}{6k^2R}+F
\end{align*}
where the right-hand side does not depend on $K$.
Thus, if the right-hand side is not zero, 
$K^* = 0$ (the other boundary case $K^* =\infty$
is clearly not cost minimizer).
Therefore, the optimization problem of 
$k^*$ becomes the identical as 
the one which assumes
that individuals shop only near their work places,
which implies
$k^* = k_W$ and $K^* = K_W = 0$.

==> Notes/two-circle-A-0.tex <==
\subsection{Extreme Case: $A = 0$}

In this subsection,
we consider an extreme case where 
$A = 0$,
i.e., 
all individuals who reside in 
the outer circle
work in the inner circle.

In this case, 
\begin{align*}
    \frac{\partial c}{\partial K}
    = 
    - \mu 
 \frac{\pi r^2}{6k^2R}+F
\end{align*}
where the right-hand side does not depend on $K$.
Thus, if the right-hand side is not zero, 
$K^* = 0$ (the other boundary case $K^* =\infty$
is clearly not cost minimizer).
Assuming $K^* = 0$, we can solve $k^*$
by its FOC
\begin{align*}
    \frac{\partial c}{\partial k}=
  -am \frac{\pi r}{2k^2}
 - \mu\frac{\pi r}{2k^2} + f=0
\end{align*}
which implies\footnote{Note that $k^*$
as well as $c(k^*,K^*)$
does not depend on $a$.} 
$k^* = \sqrt{\frac{ (m + M)\pi r}{2f}}$.
The cost for $(k^*, K^*)$
is
\begin{align*}
    c(k^*,K^*) =
\sqrt{2(m+M)\pi r f}
\end{align*}
Note that this cost 
$c(k^*,K^*)$ 
does not depend on parameter $F, R$
since we implicitly assume 
$\gamma \leq 1$.

Now we compare $c(k^*, K^*)$ 
with $c(k_W, K_W)$
where
$k_W=\sqrt{\frac{(a m + M)\pi r}{2f}}$ and
$K_W=\sqrt{\frac{(1-a) m\pi R}{2F}}$.
Note that their ratio 
$\frac{c(k_W, K_W)}{c(k^*, K^*)}\geq 1$
is monotone decreasing in $a\in[0, 1]$,
where 
$\frac{c(k_W, K_W)}{c(k^*, K^*)} = 1$
for $a = 1$.
See \Cref{fig:two-cricle-A-0-ratio-a}
and
\Cref{fig:two-cricle-A-0-ratio-b}
for graphical illustrations.



\begin{figure}
    \centering
    \includegraphics[scale = 0.7]{Notes/figs/two-circle-A-0-a.png}
    \caption{Plot 
    of $\frac{c(k_W, K_W)}{c(k^*, K^*)}$,
    with $f = F = 1$, 
$m = M = 100$, $r = 1$, $R = 10$,
$A = 0$ and $a\in[0, 1]$.
}
    \label{fig:two-cricle-A-0-ratio-a}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale = 0.7]{Notes/figs/two-circle-A-0-b.png}
    \caption{Plot 
    of 
    $\frac{c(k_W, K_W)}{c(k^*, K^*)}$,
    with $f = 2$, $F = 1$, 
$m = 20$, $M = 100$, $r = 1$, $R = 10$,
$A = 0$ and $a\in[0, 1]$.
}
    \label{fig:two-cricle-A-0-ratio-b}
\end{figure}

==> Notes/two-circle.tex <==
\section{Two Circle Model}
\begin{itemize}
    \item The city consists of two co-centric circles. The smaller one has radius $r$, the bigger one has radius $R$.
    \item The smaller one has $m$ individuals, and the larger one has $M$ individuals, distributed uniformly on the circle.
    \item $a$ fraction of individuals at each point on the inner circle works at her home location. The remaining $1-a$ fraction works on the outer circle, with workplace distributed uniformly at random. 
    \item  $A$ fraction of individuals at each point on the inner circle works at her home location. The remaining $1-A$ fraction works on the inner circle, with workplace distributed uniformly at random. 
    \item Note that the total number of work places on the inner circle is given by $w=m a + M (1-A)$. Similarly there are
    $W=M A + m(1-a)$ individuals
    on the outer circle.

    \item Cost of opening a facility in the inner circle is $f$, and the outer circle is $F$.
\end{itemize}

In this case,  optimal policies (using mobility data or only the work place data) share a simple structure: it places $k$ equally spaced stores in the inner circle, and $K$ in the outer circle. The cost of this policy is given as follows:
\[
c(k,K)=
am \frac{\pi r}{2k}+
AM \frac{\pi R}{2K}+
((1-a)m 
+(1-A)M )
(\gamma \frac{\pi r}{3k} + (1- \gamma) \frac{\pi r}{2k} )
+ fk+FK,
\]
where $\gamma=\frac{r/k}{R/K}$.
Here, the first (second) term is the cost for the individuals whose work and home places coincide, and who are in the inner (outer) circle.
The third term concerns the population whose work place is in one circle and the home is in another. Note that the closest facility in the outer circle is within $\pi r/k$ distance with probability $\gamma$ (we'll focus on parameters that ensure that $\gamma \leq 1$ at optimal solution). With complementary probability the closest facility is in the inner circle, and the expected distance is $\pi r/2k$.
With probability $\gamma$, the closest distance in expectation is given by computing the  
expectation of 
the minimum of 
two uniform random variables distributed in $[0, \pi r /k]$, which is given by\footnote{The expectation of
the $\ell$-th order 
statistics of $n$ uniform distributed 
samples in $[0, 1]$ is $\frac{\ell}{n + 1}$.}
\[\frac{1}{({\pi r}/{k})^2 /2} \int_0^{\frac{\pi r}{k}} \int_0^x y dy dx = 
\frac{1}{({\pi r}/{k})^2/2} \int_0^{\frac{\pi r}{k}}  x^2/2 dx
=\frac{\pi r}{3k}.
\]
Combining these observations yields the third term. The last two terms capture the cost of opening.

Note that in this derivation, we implicitly assumed that a person shops on the circle containing work/home location, in the vicinity of these locations.
They do not go from home location to the other circle (radially), unless this is to reach their workplaces. A sufficient condition for this is given as follows:
\begin{equation} \label{eq:RCond}
R-r>\max\{\pi R/K  , \pi r/k\} =    \pi R/K,
\end{equation}
where the last equality follows since $\gamma \leq 1$.
In what follows we will choose the parameters such that this is always satisfied in the optimal solution.

Next we consider the design that assumes that individuals shop only near their work places. In this case, the problem is decoupled over the inner and outer circles. The designer puts $k$ equally spaced facilities on the inner circle, and $K$ on the outer circle. The total cost (under the aforementioned misspecification) is given by:
\[
C_W= (am + (1 - A)M)\frac{\pi r}{2k} 
+ 
((1-a)m + A M)\frac{\pi R}{2K} + fk+FK.
\] 
Here $\frac{\pi r}{2k}$ is the expected distance from a workplace in the inner circle, and $\frac{\pi r}{2K}$ is the expected distance from a workplace in the outer circle.
Once again, we'll consider the regime where \eqref{eq:RCond} holds.
%so that individuals do not have incentive to walk from the outer circle to inner one (or vice versa).

Using first order conditions to minimize $C_W$, we get
$k_W=\sqrt{\frac{(a m + (1-A)M)\pi r}{2f}}$ and
$K_W=\sqrt{\frac{((1-a) m + AM)\pi R}{2F}}$.
% Note that \eqref{eq:RCond} is equivalent to
% $R-r> \max\{
% \sqrt{\frac{2\pi RF}{M}}, \sqrt{\frac{2\pi rf}{m}}\}$.
Note that we can evaluate the actual cost for this $(k_W,K_W)$.
% , and get:
% \begin{align*}
% c(k_W,K_W) =
% a\sqrt{\frac{m\pi rf}{2}}
% &+
% A\sqrt{\frac{M\pi RF}{2}}
% \\
% &+
% ((1-a)m 
% +(1-A)M )
% \left(\gamma
% \sqrt{\frac{2\pi rf}{9m}}
% + (1- \gamma) \sqrt{\frac{\pi rf}{2m}}
% \right)
% + \sqrt{\frac{m\pi rf}{2}}+ \sqrt{\frac{M\pi RF}{2}}.
% \end{align*}

Next we consider the optimal policy that takes into account the OD information. To that end, we rewrite $c(k,K)$ more explicitly as follows:
\[
c(k,K)=
am \frac{\pi r}{2k}+
AM \frac{\pi R}{2K}+
((1-a)m 
+(1-A)M )
(- \frac{\pi r^2K}{6k^2R} +  \frac{\pi r}{2k} )
+ fk+FK,
\]

Using FOC we conclude that at the optimal solution
\[
\frac{\partial c}{\partial k}=
-am \frac{\pi r}{2k^2}+
\mu ( \frac{\pi r^2K}{3k^3R}- \frac{\pi r}{2k^2})+f=0
\]
\[
\frac{\partial c}{\partial K}=
-AM \frac{\pi R}{2K^2}- \mu 
 \frac{\pi r^2}{6k^2R}+F=0
\]
where $\mu=((1-a)m 
+(1-A)M )$.

The solution to systems like this do not seem possible analytically in general\footnote{See \url{https://tinyurl.com/tjr94ck}.} but maybe cancellations of coefficients could yield a tractable solution.
If not, numerical solution for some primitives could be obtained.

\input{Notes/two-circle-A-0}

% \input{two-circle-1-0}

==> Notes/value-of-information.tex <==
\section{Value of Information}
Suppose we observe $\alpha_{ij}+\epsilon_{ij}$ where $\sum_j\epsilon_{ij}=0$ denote noise terms with variance $\sigma$. 
	In other words, the mobility data is noisy.
	If $\sigma$ is large we effectively only know where people live (but no mobility information is available).
	What is the dependence of the platform's payoffs on $\sigma$? 
	For what type of networks, the mobility information is important vs.\ safe to ignore?

==> Paper-MS/macros-MS.tex <==
\usepackage[parfill]{parskip}
\usepackage[letterpaper, left=1in, right=1in, top=1in, bottom=1in]{geometry}


% \usepackage[boxed]{algorithm2e}

\usepackage{pgfplots}
\pgfplotsset{compat=1.18}
\usepackage{tikz}

\usetikzlibrary{patterns}

\usepackage{amsmath,amssymb}
% \PassOptionsToPackage{numbers, compress}{natbib}
% \usepackage{tcolorbox}
\usepackage{xcolor}
\usepackage{bbm}
\usepackage{multicol}



\usepackage{natbib}
\bibliographystyle{plainnat}
\bibpunct{(}{)}{;}{a}{,}{,}
 
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage[usenames,dvipsnames]{xcolor}
\usepackage[colorlinks=true, linkcolor=blue!70!black, citecolor=blue!70!black,urlcolor=black,breaklinks=true]{hyperref}

\usepackage{hyperref}

\usepackage{comment}
\usepackage{csquotes}

\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\usepackage{mathtools, bm}

\usepackage[frak=mma]{mathalfa}


\allowdisplaybreaks


% \usepackage{algorithm} 
% \usepackage{algorithmic}  
% \usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e} 

% \usepackage[lined,boxed,ruled,norelsize,algo2e,linesnumbered,noend]{algorithm2e}
\newcommand{\algcomment}[1]{\textcolor{blue!70!black}{{\texttt{\textbf{#1}}}}}
\newcommand\mycommfont[1]{\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}

\usepackage{subcaption}
\usepackage{multirow}
\usepackage{float}
\usepackage{xspace}

\usepackage{enumitem}

\usepackage{xfrac}

\usepackage{cleveref}


\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]

\usepackage{thm-restate}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}% reset theorem numbering for each chapter

% \newenvironment{numberedtheorem}[1]{%
% \renewcommand{\thetheorem}{#1}%
% \begin{theorem}}{\end{theorem}\addtocounter{theorem}{-1}}

% \newenvironment{numberedlemma}[1]{%
% \renewcommand{\thetheorem}{#1}%
% \begin{lemma}}{\end{lemma}\addtocounter{theorem}{-1}}


\newtheorem{informal}{Informal Theorem}


\theoremstyle{plain}
\newtheorem{definition}{Definition}[section] % definition numbers are dependent on theorem numbers
\newtheorem{example}[definition]{Example}
% \newtheorem{assumption}[definition]{Assumption} 
\newtheorem{remark}[definition]{Remark} 
\newtheorem{conjecture}[definition]{Conjecture} 
\newtheorem{task}[definition]{Task} 
\newtheorem{observation}[definition]{Observation}

\theoremstyle{plain}

\newenvironment{numbereddefinition}[1]{%
\renewcommand{\thedefinition}{#1}%
\begin{definition}}{\end{definition}\addtocounter{definition}{-1}}


\newtheorem{assumption}{Assumption}
% \newtheorem{assumption}[definition]{Assumption} 


\newenvironment{numberedassumption}[1]{%
\renewcommand{\thedefinition}{#1}%
\begin{assumption}}{\end{assumption}\addtocounter{definition}{-1}}



	\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
	\newcommand{\reals}{\mathbb{R}}
	\newcommand{\positivereals}{\tiny \reals_{+}}
	\newcommand*{\R}{\mathbb{R}}



\makeatletter
\newcommand{\subalign}[1]{%
  \vcenter{%
    \Let@ \restore@math@cr \default@tag
    \baselineskip\fontdimen10 \scriptfont\tw@
    \advance\baselineskip\fontdimen12 \scriptfont\tw@
    \lineskip\thr@@\fontdimen8 \scriptfont\thr@@
    \lineskiplimit\lineskip
    \ialign{\hfil$\m@th\scriptstyle##$&$\m@th\scriptstyle{}##$\hfil\crcr
      #1\crcr
    }%
  }%
}
\makeatother




\usepackage{mathptmx}
\usepackage[T1]{fontenc}



% 	\DeclareMathOperator{\argmax}{argmax}
% 	\DeclareMathOperator{\argmin}{argmin}
	\DeclareMathOperator{\OPT}{\texttt{OPT}}
	\DeclareMathOperator{\MC}{\textrm{MaxCut}}
	\newcommand{\SDP}{\texttt{OPT-SDP}}
	\newcommand{\Ws}{\sum_{(i,j)\in E}w_{ij}}
	\newcommand{\OBJ}{\texttt{OBJ}}
	\newcommand{\Ycal}{\mathcal{Y}}
	\newcommand{\Ecal}{\mathcal{E}}
	\newcommand{\Zcal}{\mathcal{Z}}

	\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
	\DeclarePairedDelimiter{\card}{\lvert}{\rvert}
	\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
	\providecommand{\given}{}
	\DeclarePairedDelimiterX{\set}[1]\{\}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
	\let\Pr\relax
	\DeclarePairedDelimiterXPP{\Pr}[1]{\mathbb{P}}[]{}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
	\DeclarePairedDelimiterXPP{\Ex}[1]{\mathbb{E}}[]{}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
	\DeclarePairedDelimiter{\dotp}{\langle}{\rangle}
	\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
	\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}


	

	%%%-----------------Macros for this paper ------------------

	\newcommand{\YF}[1]{\textcolor{blue}{ (\em Yiding: \bf#1)}}



\newcommand{\durationpdf}{g}
\newcommand{\durationcdfi}{\bar{\durationdistribution}}
\newcommand{\inventorydistribution}{\mathcal H}
\newcommand{\inventorycdf}{\inventorydistribution}
\newcommand{\inventorycdfi}{{\bar{\inventorycdf}}}
\newcommand{\magicprob}{\eta}

\newcommand{\bench}[1]{\textbf{OPT}\left[#1\right]}
\newcommand{\tpre}{t'}
	\newcommand{\opt}{^{\star}}
	\newcommand{\primed}{^\dagger}
	\newcommand{\doubleprimed}{^{\ddagger}}
	\newcommand{\pprimed}{\doubleprimed}


	\newcommand{\Z}{\mathbb{Z}}
	\newcommand{\inventory}{c}
	\newcommand{\mininventory}{{\inventory_{\min}}}%{\underaccent{\bar}{\inventory}}

	\newcommand{\xit}{x_i(t)}
	\newcommand{\yit}{y_i(t)}
	\newcommand{\rit}{r_i(t)}
	\newcommand{\xitp}{x_i(t')}
	\newcommand{\fit}{f_i(t)}
	\newcommand{\fitp}{f_i(t')}
	\newcommand{\fitm}{f_i(t^-)}
	\newcommand{\yitm}{y_i(t^-)}
	\newcommand{\fitpm}{f_i((t')^-)}
	\newcommand{\yitp}{y_i(t')}
	\newcommand{\yitpm}{y_i((t')^-)}
	\newcommand{\ritp}{r_i(t')}
	\newcommand{\yst}{y_S(t)}
	\newcommand{\ystp}{y_S(t')}
	\newcommand{\feasibleset}{\mathcal F}
	\newcommand{\lit}{\lambda_i(t)}
	\newcommand{\litp}{\lambda_i(t')}
	\newcommand{\tht}{\theta(t)}
% 	\newcommand{\thit}{\theta_i(t)}
	\newcommand{\thitp}{\theta_i(t')}
	\newcommand{\lt}{\lambda(t)}
	\newcommand{\totaltime}{T}
	\newcommand{\reward}{r}
	\newcommand{\rewards}{\mathbf \reward}
	\newcommand{\choice}{\phi}
	\newcommand{\pen}{\Psi}
	%\newcommand{\choices}{\boldsymbol{\choice}}
	\newcommand{\durationdistribution}{G}
	\newcommand{\durationdistributions}{{\mathbf{\durationdistribution}}}
	\newcommand{\assortment}{S}
	\newcommand{\assortmentspace}{\mathcal{S}}
	\newcommand{\duration}{d}
	\newcommand{\typedistribution}{F}

	\newcommand{\inventorydual}{\theta}
	\newcommand{\inventoryduali}{\inventorydual_{i, k,t}}
	\newcommand{\probdual}{\lambda}
	\newcommand{\probduali}{\probdual_{t}}
\newcommand{\probdualtype}{\lambda_{t,\type_t}}
	\newcommand{\typesequence}{\{\type_t\}_{t = 1}^\totaltime}
	\newcommand{\inversetypesequence}{\{\type_t\}_{t = 1}^\totaltime}
	\newcommand{\typedistributionsequence}{\{\typedistribution_t\}_{t = 1}^\totaltime}

\newcommand{\EAR}{\text{EAR}}
\newcommand{\EARPrime}{\text{EAR}\primed}
% 	\newcommand{\EAR}[2][]{\text{\bf Expected-LP}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
% 	\newcommand{\EARPrime}[2][]{\text{\bf Expected-LP}^{\dagger}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
	\newcommand{\algo}{\mathcal{A}}

    \newcommand{\Profit}[2][]{\text{\bf Profit}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
    \newcommand{\Cost}[2][]{\text{\bf COST}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
    \newcommand{\CostF}[2][]{\text{\bf COST}^{\bf{F}}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
    \newcommand{\CostC}[2][]{\text{\bf COST}^{\bf{C}}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}

	\newcommand{\Rev}[2][]{\text{\bf Rev}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
	\newcommand{\MargRev}[1]{\mathbf{MargRev}[#1]}

	
    \newcommand{\Obj}[2][]{\text{\bf OBJ}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
    
    \newcommand{\SFRP}[1]{\text{\hyperref[eq:strongly factor-revealing quadratic program]{$\mathcal{P}_{\texttt{SFR}}(#1)$}}}
    \newcommand{\WFRP}[1]{\text{\hyperref[eq:weakly factor-revealing program]{$\mathcal{P}_{\texttt{FR}}(#1)$}}}

    \newcommand{\SFRPMFLP}[1]{\text{\hyperref[eq:strongly factor-revealing program MFLP]{$\mathcal{P}_{\texttt{SFR-MFLP}}(#1)$}}}
    \newcommand{\WFRPMFLP}[1]{\text{\hyperref[eq:weakly factor-revealing program MFLP]{$\mathcal{P}_{\texttt{FR-MFLP}}(#1)$}}}

\newcommand{\LBLP}[1]{\text{\hyperref[eq:lower bound LP]{$\mathcal{P}_{\texttt{LB}}(#1)$}}}




	\newcommand{\alloc}{x}
	\newcommand{\curalloc}{\alloc_{\indexnew, t}}
	\newcommand{\curalloctype}{\alloc_{\assortment, t, \type_t}}
	\newcommand{\curalloctypeopt}{\alloc^*_{\assortment, t, \type_t}}
	\newcommand{\curexantetype}{X_{\assortment, t, \type_t}}
	\newcommand{\curchoice}{\choice_{t}(\assortment, i)}
	\newcommand{\curreward}{\reward_i^{\type_t}}
	\newcommand{\price}{P}
	\newcommand{\curprice}{\price_{i, t}^{\type_t}}
	\newcommand{\curdurationdistribution}{\durationdistribution_i^{\type_t}}
	\newcommand{\curinventorya}{I_{i, t}}
	\newcommand{\curinventoryb}{I_{i, t}}
	\newcommand{\curpseudoinventory}{{\tilde{I}_{i, t}}}
	\newcommand{\curpenA}{\pen\left(\curinventorya/\inventory_i\right)}
	\newcommand{\curpenB}{\pen\left(\curinventoryb/\inventory_i\right)}
	\newcommand{\curpena}{\pen_i(t^-)}
	\newcommand{\curpenb}{\pen_i(t)}
	\newcommand{\previous}{^\prime}
	\newcommand{\prealloc}{\alloc_{\indexnew, \tpre}}
	\newcommand{\prechoice}{\choice_{\tpre}(\assortment, i)}
	%\newcommand{\curchoicetype}{\choice^{\type_t}(\assortment, i)}


	% accents for using with newagentvar
	% (must take a single argument)
	\newcommand{\ironed}{\bar}
	\newcommand{\constrained}{\hat}
	\newcommand{\optconstrained}{\composed{\optimized}{\constrained}}
	\newcommand{\optimized}[1]{#1\opt}
	\newcommand{\differentiated}[1]{#1'}
	\newcommand{\fortype}{\tilde}
	\newcommand{\tagged}[2]{{#2}^{#1}}


	\newcommand{\starred}[1]{#1^\star}
	\newcommand{\primedarg}[1]{#1\primed}
	\newcommand{\noaccents}[1]{#1}
	% compose accents on the fly
	\newcommand{\composed}[3]{#1{#2{#3}}}
	\newcommand{\newagentvar}[3][\noaccents]{%
		\expandafter\newcommand\expandafter{\csname #2\endcsname}{#1{#3}}%
		\expandafter\newcommand\expandafter{\csname #2s\endcsname}{#1{\boldsymbol{#3}}}%
		\expandafter\newcommand\expandafter{\csname #2smi\endcsname}[1][i]{#1{\boldsymbol{#3}}_{-##1}}%
		\expandafter\newcommand\expandafter{\csname #2i\endcsname}[1][i]{#1{#3}\agind[##1]}%
		\expandafter\newcommand\expandafter{\csname #2ith\endcsname}[1][i]{#1{#3}_{(##1)}}%
	}
	\newagentvar{typespace}{{\cal Z}}
	\newagentvar{typesubspace}{S}
	\newcommand{\extypes}[1][\exquant]{\typesubspace^{#1}\!}
	\newagentvar{type}{z}
	\newagentvar{othertype}{s}
	\newagentvar{val}{v}
	\newagentvar{hval}{\bar \val}
	\newagentvar{hbudget}{\bar \wealth}
	\newagentvar{budget}{B}
	\newagentvar{lbudget}{\underaccent{\bar}{ \wealth}}
	\newagentvar{lowestval}{0}
	\newagentvar{cumval}{V}
	\newagentvar{cumprice}{P}
	\newagentvar{welcurve}{W}
	\newagentvar{revcurve}{R}
	\newagentvar{outcome}{w}
	\newagentvar{outcomespace}{{\cal W}}
	\newcommand{\nulloutcome}{\emptyset}
	


	
	\newcommand{\distance}{d}
\newcommand{\flow}{\tau}
\newcommand{\flowi}{\flow_{ij}}
\newcommand{\flows}{\{\flowi\}}
\newcommand{\pop}{N}
\newcommand{\popi}{\pop_i}
\newcommand{\popj}{\pop_j}
\newcommand{\pops}{\{\popi\}}
\newcommand{\emp}{E}
\newcommand{\empi}{\emp_i}
\newcommand{\empj}{\emp_j}
\newcommand{\emps}{\{\empi\}}
\newcommand{\stores}{\SOL}
\newcommand{\home}{h}
\newcommand{\workplace}{w}
% \newcommand{\distance}{d}
\newcommand{\opencost}{f}
\newcommand{\opencosti}{\opencost_i}
\newcommand{\opencosts}{\{\opencosti\}}
\newcommand{\serveradius}{R}

\newcommand{\servingpopulation}{\texttt{Service}}
\newcommand{\servingpopulationand}{\servingpopulation_\land}
\newcommand{\servingpopulationor}{\servingpopulation_\lor}

\newcommand{\data}{D}
\newcommand{\mobilitydata}{\data_{M}}
\newcommand{\partialdata}{\data_{L}}
\newcommand{\datas}{\mathcal{\data}}
\newcommand{\mobilitydatas}{\datas_{M}}
\newcommand{\allmobilitydatas}{\bar\datas_{M}}


\newcommand{\population}{\emp}
\newcommand{\employee}{\pop}
% \newcommand{\flow}{\tau}
\newcommand{\flowbf}{\boldsymbol{\flow}}
% \newcommand{\flowi}{\flow_{ij}}

\newcommand{\instance}{I}
\newcommand{\instances}{\mathcal{\instance}}
\newcommand{\observeinstance}{D}
\newcommand{\SOL}{\texttt{SOL}}
\renewcommand{\OPT}{\texttt{OPT}}
\newcommand{\voi}{\Gamma}
\newcommand{\voior}{\voi_\lor}
\newcommand{\voiand}{\voi_\land}



% \newcommand{\OPT}{\texttt{OPT}}
\newcommand{\approxratio}{\Gamma}
\newcommand{\SFRapproxratio}{\approxratio_{\texttt{SFR}}(\discountfactor,\costscalar)}
\newcommand{\WFRapproxratio}{\approxratio_{\texttt{FR}}(\discountfactor, \costscalar)}

\newcommand{\SFRMFLPapproxratio}{\approxratio_{\texttt{SFR-MFLP}}}
\newcommand{\WFRMFLPapproxratio}{\approxratio_{\texttt{FR-MFLP}}}


\newcommand{\connectioncost}{c}
\newcommand{\sol}{\Psi}


\newcommand{\distanceHat}{{\distance}}
\newcommand{\costHat}{{\opencost}}
\newcommand{\distanceHatStar}{{\connectioncost}}
\newcommand{\muHat}{{\alpha}}
\newcommand{\dualapproxHat}{\hat{\dualapprox}}
\newcommand{\permuspace}{\mathbb{\chi}}
\newcommand{\permu}{\chi}

\newcommand{\greedyapprox}{\text{2.497}}
\newcommand{\greedyapproxMFLP}{\text{1.819}}
\newcommand{\greedyapproxLB}{2.428}


\newcommand{\Home}{\texttt{H}}
\newcommand{\Work}{\texttt{W}}

\newcommand{\TWOLFLP}{2-LFLP}
\newcommand{\edge}{e}
\newcommand{\edgehome}{\edge_\Home}
\newcommand{\edgework}{\edge_\Work}
\newcommand{\flowe}{\flow_\edge}
\newcommand{\ALG}{\texttt{ALG}}

\newcommand{\plus}[1]{{\left( #1 \right)^+}}

\newcommand{\dual}{\mu}
\newcommand{\currentset}{U}
\newcommand{\starinstance}{S}
\newcommand{\pendingset}{W}
\newcommand{\N}{\mathbb{N}}
\newcommand{\edgeindex}{\texttt{L}}

\newcommand{\frcone}{\texttt{FRC-1}}
\newcommand{\frctwo}{\texttt{FRC-2}}
\newcommand{\frcthree}{\texttt{FRC-3}}
\newcommand{\frcfour}{\texttt{FRC-4}}
\newcommand{\frcfive}{\texttt{FRC-5}}
\newcommand{\frcsix}{\texttt{FRC-6}}

\newcommand{\greedycounter}{\alpha}
\newcommand{\firstchanceset}{U}
\newcommand{\secondchanceset}{U^{(2)}}
\newcommand{\secondchancesetwork}{\secondchanceset_w}
\newcommand{\secondchancesethome}{\secondchanceset_h}
\newcommand{\connectmapping}{\psi}
\newcommand{\Edge}{E}
\newcommand{\config}{\sigma}
% \newcommand{\config}{\mathfrak{H}}
\newcommand{\confige}{{\config(\edge)}}
\newcommand{\configi}{\confige}
\newcommand{\timeindex}{t}
\newcommand{\cost}{c}
\newcommand{\coststar}{\cost(\starinstance)}
\newcommand{\allocstar}{\alloc(\starinstance)}
\newcommand{\duale}{\dual(\edge)}
\newcommand{\starspace}{\mathcal{S}}
\newcommand{\singlecountedgeset}{\Edge^{(1)}}
\newcommand{\kcountedgeset}{\Edge^{(k)}}
\newcommand{\doublecountedgeset}{\Edge^{(2)}}
\newcommand{\singlecountedgesetHat}{\hat{\singlecountedgeset}}
\newcommand{\doublecountedgesetHat}{\hat{\doublecountedgeset}}
\newcommand{\mHat}{{m}}
\newcommand{\nHat}{{n}}
\newcommand{\qHat}{{q}}
\newcommand{\dualapprox}{\Gamma}



\newcommand{\qHatBf}{\mathbf{q}}
\newcommand{\muHatBf}{\boldsymbol{\muHat}}
\newcommand{\distanceHatBf}{{\mathbf{\distance}}}
\newcommand{\distanceHatStarBf}{{\mathbf{\connectioncost}}}
\newcommand{\zerobf}{\mathbf{0}}

\newcommand{\naturals}{\mathbb{N}}


\newcommand{\yHat}{\hat{y}}



\newcommand{\discountfactor}{\gamma}
\newcommand{\nullsymbol}{\bot}
\newcommand{\hwset}{\{\Home,\Work\}}

\newcommand{\normalizefactor}{N}
\newcommand{\SFRCmonotonicity}{\texttt{(SFR.i)}}
\newcommand{\SFRCtriangleineq}{\texttt{(SFR.ii)}}
\newcommand{\SFRCcontribution}{\texttt{(SFR.iii)}}
\newcommand{\SFRCcontributionstronger}{\texttt{(SFR.iii.0)}}
\newcommand{\SFRCdistance}{\texttt{(SFR.iv)}}
\newcommand{\SFRCconnectcost}{\texttt{(SFR.v)}}
\newcommand{\SFRCtotalcost}{\texttt{(SFR.vi)}}
\newcommand{\SFRCdensity}{\texttt{(SFR.vii)}}

\newcommand{\WFRCtriangleineq}{\texttt{(FR.i)}}
\newcommand{\WFRCcontribution}{\texttt{(FR.ii)}}
\newcommand{\WFRCconnectcost}{\texttt{(FR.iii)}}
\newcommand{\WFRCtotalcost}{\texttt{(FR.iv)}}

\newcommand{\EdgeTilde}{\tilde{\Edge}}
\newcommand{\edgetoellmapping}{\kappa}
\newcommand{\edgetoellmappingconfig}{\edgetoellmapping_{\config}}

\newcommand{\empattract}{\rho}
\newcommand{\flowconstructionfactor}{\iota}
\newcommand{\costconstructionfactor}{\bar{\opencost}}
\newcommand{\zhvi}{z}
\newcommand{\CFAlg}{\texttt{2-GR}}
\newcommand{\CFAlgP}{\texttt{2-GRP}}
\newcommand{\GDH}{\texttt{GR-H}}
\newcommand{\GDW}{\texttt{GR-W}}

\newcommand{\candidatecosttext}{candidate cost}

\newcommand{\KLFLP}{$K$-LFLP}
\newcommand{\RelaxSFRapproxratio}{\approxratio_{\texttt{SFR-K}}}
\newcommand{\RelaxSFRP}[1]{\text{\hyperref[eq:relax strongly factor-revealing quadratic program]{$\mathcal{P}_{\texttt{SFR-K}}(#1)$}}}



\newcommand{\permuTGD}{\mathcal{Y}}


\newcommand{\costscalar}{\eta}

==> Paper-MS/math-MS.tex <==
\newcommand{\setsize}[1]{{\left|#1\right|}}





\newcommand{\super}[1]{^{(#1)}}

% \newcommand{\inteval}[1]{\Big[#1\Big]}
\newcommand{\tinteval}[1]{\left[#1\right]}
\newcommand{\distcond}[2]{\left.#1\vphantom{\big|}\right|_{#2}}
\newcommand{\evalat}[2]{\left.#1\vphantom{\big|}\right|_{#2}}


%
% probability stuff.
%
\newcommand{\condition}{\,\mid\,}

% resizing brackets 
\newcommand{\prob}[2][]{\text{Pr}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}
\newcommand{\expect}[2][]{\mathbb{E}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[{\def\givenn{\middle|}#2}\right]}


% brackets configured with \tparen
\newcommand{\tparen}{\big}
\newcommand{\tprob}[2][]{\text{Pr}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\tparen[{\def\given{\tparen|}#2}\tparen]}
\newcommand{\texpect}[2][]{\mathbb{E}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\tparen[{\def\given{\tparen|}#2}\tparen]}


% brackets do not resize.
\newcommand{\sprob}[2][]{\text{Pr}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}[#2]}
\newcommand{\sexpect}[2][]{\mathbb{E}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}[#2]}






\newcommand{\suchthat}{\,:\,}


\newcommand{\partialx}[2][]{{\tfrac{\partial #1}{\partial #2}}}
\newcommand{\nicepartialx}[2][]{{\nicefrac{\partial #1}{\partial #2}}}
\newcommand{\dd}{{\mathrm d}}
\newcommand{\ddx}[2][]{{\tfrac{\dd #1}{\dd #2}}}
\newcommand{\niceddx}[2][]{{\nicefrac{\dd #1}{\dd #2}}}
\newcommand{\grad}{\nabla}

\newcommand{\symdiff}{\triangle}



\newcommand{\indicator}[1]{{\mathbbm{1}\left\{ #1 \right\}}}





==> Paper/alg-2-choice-greedy-v2.tex <==
\begin{algorithm}
    \SetKwInOut{Input}{input}
    \SetKwInOut{Output}{output}

    \Input{discount factor $\discountfactor\in[0, 1]$,
    {\color{red}opening cost scalar $\costscalar \in \reals_+$,} and
    \TWOLFLP\ instance $\instance = 
    (n, \distance, 
\{\flowe\}_{\edge\in\Edge}, \opencosts_{i\in[n]})$}
%  	\vspace{1mm}
    \Output{subset $\stores \subseteq[n]$
    as the locations of opened facilities.}
 	\caption{2-Chance Greedy Algorithm V2}
 	\label{alg:greedy modified v2}
%  	\vspace{2mm}
 	
 	initialize $\stores \gets \emptyset$
 	
 	initialize $\greedycounter(\edge) \gets 0$ for each edge $\edge\in\Edge$
 	
%  	\vspace{1mm}
 	
 	initialize $\firstchanceset \gets \Edge$,
%  	\vspace{2mm}

    initialize $\connectmapping(\edge,\edgeindex) \gets \nullsymbol$
    for each edge $\edge \in\Edge$,
    each $\edgeindex\in\hwset$
 	
 	\While{$\firstchanceset \not= \emptyset$}{ 
 	  %  \vspace{1mm}
 	    increase $\greedycounter(\edge)$ by 
 	    $d\greedycounter$
 	    for every edge $\edge \in \firstchanceset$
 	    
 	    
 	    \tcc{Event (a)}
 	    
 	    \While{there exists edge $\edge \in \firstchanceset$
 	    and location $i\in\stores$ 
 	    s.t.\ $\greedycounter(\edge) = \distance(\edge, i)$ 
 	    }
 	    {
 	    
 	  %  \vspace{1mm}
 	  
 	    remove edge $\edge$ from $\firstchanceset$,
 	    i.e., $\firstchanceset\gets \firstchanceset\backslash\{\edge\}$
 	    
 	     \For{each $\edgeindex \in \hwset$}{
 	    \If{$\greedycounter(\edge) = \distance(\edge_\edgeindex,i)$}{
 	    
 	    connect edge $\edge$ and facility $i$ through 
      home/work location $\edge_\edgeindex$, i.e., 
 	    $\connectmapping(\edge,\edgeindex) \gets i$
 	    }
 	    }

 	    }
 	    
 	    
 	    \tcc{Event (b)}
 	    
 	    \While{there exists location $i\not\in\stores$ s.t.\
 	    $\sum_{\edge\in \firstchanceset} 
 	    \flowe\cdot 
 	    \plus{\greedycounter(\edge) - \distance(\edge, i)}
 	    +
 	    \sum_{
 	    \subalign{
 	    &\edge\not\in \firstchanceset,\\
 	    &\edgeindex\in\hwset:
 	    \connectmapping(\edge,\edgeindex) = \nullsymbol
 	    }}
 	    \flowe\cdot 
 	    \plus{\discountfactor\cdot \greedycounter(\edge) - \distance(\edge_\edgeindex,i)}
 	    = {\color{red}\costscalar\cdot }\opencost_i$
 	    }{
 	    
 	    \vspace{1mm}
 	    
 	    add location $i$ into $\stores$, i.e.,
 	    $\stores \gets \stores \cup \{i\}$
 	    
 	    
 	    
 	    \For{each edge $\edge\not\in \firstchanceset$}{
 	    \For {each $\edgeindex \in \hwset$}{
 	  %  \vspace{1mm}
 	  
 	    \If{$\connectmapping(\edge,\edgeindex) = \nullsymbol$ 
 	    and $\discountfactor\cdot \greedycounter(\edge) \geq \distance(\edge_\edgeindex, i) $}{
 	  
 	    connect edge $\edge$ and facility $i$ through 
      home/work location 
      $\edge_\edgeindex$, i.e., 
 	    $\connectmapping(\edge,\edgeindex) \gets i$
 	  %  \vspace{1mm}
 	   
 	    }
 	    }
 	    }
 	    
 	    \For{each edge $\edge\in \firstchanceset$}{
 	    
 	    \If{$\greedycounter(\edge) - \distance(\edge, i)\geq 0$}{
 	    
 	    remove edge $\edge$ from $\firstchanceset$,
 	    i.e., $\firstchanceset\gets \firstchanceset\backslash\{\edge\}$
 	    
 	    \For{each $\edgeindex \in \hwset$}{
 	    \If{$\greedycounter(\edge) \geq \distance(\edge_\edgeindex,i) $}{
 	    
 	    connect edge $\edge$ and facility $i$ through 
      home/work location 
      $\edge_\edgeindex$, i.e., 
 	    $\connectmapping(\edge,\edgeindex) \gets i$
 	    }
 	    }
 	    }
 	    }
 	    }
 	   
 	}
 	\textbf{return} $\stores$
\end{algorithm}







==> Paper/apx-numerical-additional-results.tex <==
\section{Additional Results 
for Numerical Experiments}
\label{apx:numerical additional results}

Here we present 
additional numerical results 
of the experiments over synthetic 
data. 
The experimental setup is the same 
as \Cref{sec:numerical synthetic},
except that the cost distribution 
$\texttt{Exponential}(\sfrac{1}{100})$
is replaced with 
$\texttt{Exponential}(\sfrac{1}{50})$
and 
$\texttt{Exponential}(\sfrac{1}{200})$.
In all setups, our observations in \Cref{sec:numerical synthetic} 
preserve. 
Specifically, $\CFAlgP(1)$ outperforms all other policies,
and the performance gap between $\CFAlgP(1)$ and $\GDH$, $\GDW$
is significant.
See the normalized performance for different policies
in \Cref{fig:numerical synthetic ratio ExpDist(1/50)},
\Cref{fig:numerical synthetic ratio ExpDist(1/200)},
\Cref{table:numerical synthetic ratio ExpDist(1/50)}
and \Cref{table:numerical synthetic ratio ExpDist(1/200)}.


\begin{figure}[ht]
  \centering
       \subfloat[uniform $\{\flowi\}$]
      {\includegraphics[width=0.45\textwidth]{Paper/figs/numerical/synthetic-uniform-ratio-50.png}}
      ~~~~
      ~~~~
      \subfloat[distance-discounted $\{\flowi\}$]
      {\includegraphics[width=0.45\textwidth]{Paper/figs/numerical/synthetic-disdiscount-ratio-50.png}}
  \caption{Comparison of different policies in terms of the normalized performance. Facility opening costs $\{\opencost_i\}$
  are drawn i.i.d.\ from $\texttt{Exponential}(\sfrac{1}{50})$.
  Results are based on 100 i.i.d.\ random instance.
  }
   \label{fig:numerical synthetic ratio ExpDist(1/50)}
\end{figure}

\begin{figure}[ht]
  \centering
       \subfloat[uniform $\{\flowi\}$]
      {\includegraphics[width=0.45\textwidth]{Paper/figs/numerical/synthetic-uniform-ratio-200.png}}
      ~~~~
      ~~~~
      \subfloat[distance-discounted $\{\flowi\}$]
      {\includegraphics[width=0.45\textwidth]{Paper/figs/numerical/synthetic-disdiscount-ratio-200.png}}
  \caption{Comparison of different policies in terms of the normalized performance. Facility opening costs $\{\opencost_i\}$
  are drawn i.i.d.\ from $\texttt{Exponential}(\sfrac{1}{200})$.
  Results are based on 100 i.i.d.\ random instance.
  }
   \label{fig:numerical synthetic ratio ExpDist(1/200)}
\end{figure}




\begin{table}[ht]
    \centering
    \caption{The average normalized performance for 
    different policies. Facility opening costs $\{\opencost_i\}$
  are drawn i.i.d.\ from $\texttt{Exponential}(\sfrac{1}{50})$.}
    \label{table:numerical synthetic ratio ExpDist(1/50)}
    \begin{tabular}[t]{cccccc}
    \toprule
    & 
    \CFAlg(1) & \CFAlg(0.7) & \CFAlg(0.5) &
    \CFAlg(0.3) & \CFAlg(0) 
     \\
     \midrule
     uniform $\{\flowi\}$ 
     & 1.022 & 1.008 & 1.011 & 1.024 & 1.049 \\
     dist.-discounted $\{\flowi\}$
     & 1.029 & 1.008 & 1.011 & 1.022 & 1.044 \\
    \bottomrule
    \\
    \toprule
    & 
    \CFAlgP(1) & \CFAlgP(0.7) & \CFAlgP(0.5) &
    \CFAlgP(0.3) & \CFAlgP(0) 
     \\
     \midrule
     uniform $\{\flowi\}$ 
     & 1.001 & 1.002 & 1.009 & 1.023 & 1.049 \\
     dist.-discounted $\{\flowi\}$
     & 1.001 & 1.002 & 1.009 & 1.021 & 1.044 \\
    \bottomrule\\
     \addlinespace[-\aboverulesep] 
    \cmidrule[\heavyrulewidth]{1-3}
    & 
    \GDH & \GDW
     \\
     \cmidrule{1-3}
     uniform $\{\flowi\}$ 
     & 1.191 & 1.186 \\
     dist.-discounted $\{\flowi\}$
     & 1.193 & 1.192 \\
 \cmidrule[\heavyrulewidth]{1-3}
     \addlinespace[-\belowrulesep] 
    \end{tabular}
\end{table}



\begin{table}[ht]
    \centering
    \caption{The average normalized performance for 
    different policies. Facility opening costs $\{\opencost_i\}$
  are drawn i.i.d.\ from $\texttt{Exponential}(\sfrac{1}{200})$.}
    \label{table:numerical synthetic ratio ExpDist(1/200)}
    \begin{tabular}[t]{cccccc}
    \toprule
    & 
    \CFAlg(1) & \CFAlg(0.7) & \CFAlg(0.5) &
    \CFAlg(0.3) & \CFAlg(0) 
     \\
     \midrule
     uniform $\{\flowi\}$ 
     & 1.009 & 1.006 & 1.013 & 1.024 & 1.046 \\
     dist.-discounted $\{\flowi\}$
     & 1.011 & 1.005 & 1.015 & 1.025 & 1.048 \\
    \bottomrule
    \\
    \toprule
    & 
    \CFAlgP(1) & \CFAlgP(0.7) & \CFAlgP(0.5) &
    \CFAlgP(0.3) & \CFAlgP(0) 
     \\
     \midrule
     uniform $\{\flowi\}$ 
     & 1.0 & 1.004 & 1.012 & 1.024 & 1.046 \\
     dist.-discounted $\{\flowi\}$
     & 1.0 & 1.003 & 1.014 & 1.024 & 1.048 \\
    \bottomrule\\
     \addlinespace[-\aboverulesep] 
    \cmidrule[\heavyrulewidth]{1-3}
    & 
    \GDH & \GDW
     \\
     \cmidrule{1-3}
     uniform $\{\flowi\}$ 
     & 1.107 & 1.11 \\
     dist.-discounted $\{\flowi\}$
     & 1.105 & 1.102 \\
 \cmidrule[\heavyrulewidth]{1-3}
     \addlinespace[-\belowrulesep] 
    \end{tabular}
\end{table}

==> Paper/experiments-old.tex <==
\section{Numerical Experiments}
\label{sec:numerical}

To 
provide numerical justifications
for the performance of our proposed algorithm,
we
run numerical experiments over
both synthetic data (\Cref{sec:numerical synthetic}) and
US census data (\Cref{sec:numerical us cities}).

\subsection{Experiments over synthetic data}
\label{sec:numerical synthetic}
We first discuss the numerical experiment
over randomly-generated synthetic data.

\paragraph{Experimental setup.}
In our test problem, there are $n = 30$ locations. 
Each location $i\in[n]$ is 
associated with a two-dimensional coordinate 
$(x_i, y_i)$, 
population $\pop_i$,
and 
facility opening cost $\opencost_i$.
Here coordinates $x_i, y_i$ are drawn i.i.d.\ 
from the normal distribution $\texttt{Normal}(0, 1)$,
population $\pop_i$
is drawn i.i.d.\ from the exponential distribution 
$\texttt{Exponential}(\sfrac{1}{100})$,
and facility opening cost $\opencost_i$ is drawn 
i.i.d.\ from the exponential distribution 
$\texttt{Exponential}(\sfrac{1}{\costconstructionfactor})$ with $\costconstructionfactor\in\{20, 100\}$.
\footnote{We also
ran our experiments by varying all parameters in our synthetic instances. We obtained similar results 
and verified the robustness of our numerical findings. 
In 
\Cref{apx:numerical additional results},
we include additional results by varying the distributions 
for the facility opening costs $\{\opencost_i\}$.}
We consider the Euclidean distance based on 
coordinates $\{(x_i, y_i)\}$
as the
distance function $\distance:[n]\times[n]\rightarrow
\reals_+$.


The number of individuals $\flowi$
for each edge $(i, j)\in\Edge$ is generated as follows.
Each location~$i\in[n]$ is associated with an 
employee attractiveness $\empattract_i$
drawn i.i.d.\ from the exponential distribution 
$\texttt{Exponential}(1)$.
For each edge $(i, j) \in \Edge$,
we set
\begin{align*}
    \flowi \triangleq 
    \displaystyle
    \popi \cdot \frac{
    \empattract_j\cdot 
    \exp\left(-\flowconstructionfactor
    \cdot \distance(i, j)\right)
    }{\sum_{k\in[n]}
    \empattract_k\cdot 
    \exp\left(-\flowconstructionfactor
    \cdot \distance(i, k)\right)
     }
\end{align*}
In this construction, $\flowi$
is inline with the standard MNL model 
by interpreting $\log(\flowconstructionfactor_j)$
as the value of location $j$.
Consequently, $\flowi$
increases as the employee attractiveness $\empattract_j$
of location $j$
increases.
Parameter~$\flowconstructionfactor$ 
controls the impact of distance between 
locations $i$ and $j$ on $\flowi$.
We conduct experiments  
for $\flowconstructionfactor \in \{0, \sfrac{1}{5}\}$ and 
refer them as 
\emph{uniform $\{\flowi\}$} and \emph{distance-discounted 
$\{\flowi\}$}, respectively.

\newcommand{\CFAlgStar}{\CFAlg^*}
\newcommand{\CFAlgPStar}{\CFAlgP^*}
\newcommand{\Param}{\texttt{Param}}

\paragraph{Policies.}
In this numerical experiment, 
we compare three different classes of policies:
\begin{enumerate}
    \item \textsl{The 2-Chance Greedy Algorithm}:
    this policy is \Cref{alg:greedy modified}
    parameterized by 
    discount factor~$\discountfactor$ and opening cost scalar $\costscalar$.
    Its approximation ratio is upperbounded by 
    $\SFRapproxratio$.
    We implement this policy with discount factor 
    $\discountfactor\in\{0, 0.2, 0.4, 0.6, 0.8, 1\}$ and opening cost scalar $\costscalar\in\{1, 1 + 0.5 \discountfactor, 1 + \discountfactor\}$,
    and refer it as $\CFAlg(\discountfactor,\costscalar)$.
    Hereafter, we use $\Param\triangleq \{(\discountfactor,\costscalar):\discountfactor\in\{0, 0.2, 0.4, 0.6, 0.8, 1\}, \costscalar\in\{1, 1 + 0.5 \discountfactor, 1 + \discountfactor\}\}$ to denote the space of discretized $\discountfactor$ and $\costscalar$ in our experiments.
    
    Moreover, for each randomly generated instance, we compute the total cost of $\CFAlg(\discountfactor,\costscalar)$ for all discretized $(\discountfactor,\costscalar)\in\Param$ described above, and then refer the best one as $\CFAlgStar$.
    Namely, for each randomly generated instance $\instance$, 
    $\CFAlgStar \triangleq \CFAlg(\discountfactor^*,\costscalar^*)$ with
    \begin{align*}
        (\discountfactor^*,\costscalar^*) = \argmin_{(\discountfactor,\costscalar)\in\Param} \Cost[\instance]{\CFAlg(\discountfactor,\costscalar)}
    \end{align*}
    where $\Cost[\instance]{\CFAlg(\discountfactor,\costscalar)}$ is the total cost of algorithm $\CFAlg(\discountfactor,\costscalar)$ on instance $\instance$.
    \item \textsl{The 2-Chance Greedy Algorithm
    with Myopic Pruning}:
    this policy combines \Cref{alg:greedy modified} 
    with an additional post-processing step 
    (i.e., myopic pruning) as follows.
    Given $\SOL$ returned by \Cref{alg:greedy modified},
    this policy iteratively checks whether 
    the total cost can be reduced by removing 
    (a.k.a., pruning) 
    a facility 
    from current solution $\SOL$. 
    If such a facility exists, 
    it \emph{greedily prunes} the one with the highest cost reduction, and repeats.
    By construction, the performance
    of this policy 
    is weakly better than \Cref{alg:greedy modified},
    and its approximation ratio 
    is upperbouned by $\SFRapproxratio$ as well.
    We implement this policy with discretized discount factor 
    $\discountfactor$ and opening cost scalar $\costscalar$ for all $(\discountfactor,\costscalar)\in\Param$,
    and refer it as $\CFAlgP(\discountfactor,\costscalar)$.
    Similar to $\CFAlgStar$, we introduce $\CFAlgPStar$ to denote algorithm $\CFAlgP(\discountfactor,\costscalar)$ with the best discretized $\discountfactor, \costscalar$ for each randomly generated instance.
    \item \textsl{The Greedy Algorithm 
    with Home (resp.\ Work) Location}:
    this policy is the JMMSV algorithm 
    (\citealp{JMMSV-02}, \Cref{alg:JMMSV})
    assuming that each individual can only be connected 
    through her home (resp.\ work) location.
    This policy requires the knowledge of 
    population $\{\popi\}$
    (resp.\ employment) for each location,
    and the knowledge of $\{\flowi\}$
    is unnecessary.
    Its approximation ratio in the \TWOLFLP\ 
    is unbounded.
    We refer this policy as $\GDH$ (resp.\ $\GDW$).
\end{enumerate}

\paragraph{Results.}
In order to compare different policies,
we sample 100 randomly generated synthetic instances.
For each instance and each policy, 
we normalize its performance by 
computing the ratio between
the cost of this policy on
this instance 
and 
the cost of policy $\CFAlgPStar$.
We use ``box and whisker'' plots 
to demonstrate the median normalized performance and  
the resulting confidence intervals 
(\Cref{fig:numerical synthetic ratio}).
Moreover, we report the average normalized performance in \Cref{table:numerical synthetic ratio}.
Below we discuss our numerical results in detail.

\begin{figure}[ht]
  \centering
       \subfloat[uniform $\{\flowi\}$]
      {\includegraphics[width=0.45\textwidth]{Paper/figs/numerical/synthetic-uniform-ratio.png}}
      ~~~~
      ~~~~
      \subfloat[distance-discounted $\{\flowi\}$]
      {\includegraphics[width=0.45\textwidth]{Paper/figs/numerical/synthetic-disdiscount-ratio.png}}
  \caption{Comparison of different policies in terms of the normalized performance in \Cref{sec:numerical synthetic}. Results are based on 100 i.i.d.\ random instance.
  }
   \label{fig:numerical synthetic ratio}
\end{figure}


% \begin{table}[t]
%     \centering
%     \caption{The average normalized performance for 
%     different policies in \Cref{sec:numerical synthetic}.}
%     \label{table:numerical synthetic ratio}
%     \begin{tabular}[t]{ccccccc}
%     \toprule
%     & 
%     \CFAlg(1) & \CFAlgP(1) &
%     \CFAlg(0.7) & \CFAlgP(0.7) &
%     \CFAlg(0.5) & \CFAlgP(0.5) 
%      \\
%      \midrule
%      uniform $\{\flowi\}$ 
%      & 1.016 & 1.0 & 1.007 & 1.004 & 1.011 & 1.011\\
%      dist.-discounted $\{\flowi\}$
%      & 1.02 & 1.0 & 1.007 & 1.004 & 1.014 & 1.013 \\
%     \bottomrule
%     \\
%     \\
%     \toprule
%     & 
%     \CFAlg(0.3) & \CFAlgP(0.3) &
%     \CFAlg(0) & \CFAlgP(0) &
%     \GDH & \GDH
%      \\
%      \midrule
%      uniform $\{\flowi\}$ 
%      & 1.025 &  1.025 & 1.05 & 1.05 & 1.144& 1.134 \\
%      dist.-discounted $\{\flowi\}$
%      & 1.024 & 1.024 & 1.051 & 1.051 & 1.137 & 1.141 \\
%     \bottomrule
%     \end{tabular}
% \end{table}

\begin{table}[t]
    \centering
    \caption{The average normalized performance for 
    different policies in \Cref{sec:numerical synthetic}.}
    \label{table:numerical synthetic ratio}
    \begin{tabular}[t]{cccccc}
    \toprule
    & 
    \CFAlg(1) & \CFAlg(0.7) & \CFAlg(0.5) &
    \CFAlg(0.3) & \CFAlg(0) 
     \\
     \midrule
     uniform $\{\flowi\}$ 
     & 1.016 & 1.007 & 1.011 & 1.025 & 1.05\\
     dist.-discounted $\{\flowi\}$
     & 1.02 & 1.007 & 1.014 & 1.024 & 1.051 \\
    \bottomrule
    \\
    \toprule
    & 
    \CFAlgP(1) & \CFAlgP(0.7) & \CFAlgP(0.5) &
    \CFAlgP(0.3) & \CFAlgP(0) 
     \\
     \midrule
     uniform $\{\flowi\}$ 
     & 1.0 &  1.004 & 1.011 & 1.025 & 1.05 \\
     dist.-discounted $\{\flowi\}$
     & 1.0 & 1.004 & 1.013 & 1.024 & 1.051 \\
    \bottomrule\\
     \addlinespace[-\aboverulesep] 
    \cmidrule[\heavyrulewidth]{1-3}
    & 
    \GDH & \GDW
     \\
     \cmidrule{1-3}
     uniform $\{\flowi\}$ 
     & 1.144& 1.134 \\
     dist.-discounted $\{\flowi\}$
     & 1.137 & 1.141 \\
 \cmidrule[\heavyrulewidth]{1-3}
     \addlinespace[-\belowrulesep] 
    \end{tabular}
\end{table}


\begin{figure}[ht]
  \centering
       \subfloat[uniform $\{\flowi\}$]
      {\includegraphics[width=0.45\textwidth]{Paper/figs/numerical/synthetic-uniform-size.png}}
      ~~~~
      ~~~~
      \subfloat[distance-discounted $\{\flowi\}$]
      {\includegraphics[width=0.45\textwidth]{Paper/figs/numerical/synthetic-disdiscount-size.png}}
  \caption{Comparison of different policies in terms of the size of solutions in \Cref{sec:numerical synthetic}. Results are based on 100 i.i.d.\ random instance.
  }
   \label{fig:numerical synthetic size}
\end{figure}

\noindent\textsl{\underline{The impact of discount factor $\discountfactor$
in the 2-Chance Greedy Algorithm.}}
Recall that
the approximation ratio of the 2-Chance Greedy Algorithm
becomes $\Omega(\log n)$
when discount factor $\discountfactor$ approaches zero
(\Cref{example:JMMSV failure}),
while the approximation is constant 
with positive constant discount factor $\discountfactor$,
e.g., a $\greedyapprox$-approximation for $\discountfactor = 1$
(\Cref{prop:approx ratio general gamma}).
From both \Cref{fig:numerical synthetic ratio} and 
\Cref{table:numerical synthetic ratio},
it can be observed that 
$\CFAlg(0.7)$ achieves the best average 
performance over all discount 
factors $\discountfactor\in\{0, 0.3, 0.5, 0.7, 1\}$.
Moreover, the average normalized performance of $\CFAlg(\discountfactor)$ 
improves 
for $\discountfactor\in\{0, 0.3, 0.5, 0.7\}$.

To understand why the average normalized performance of 
$\CFAlg(1)$ is worse than 
the average normalized performance of 
$\CFAlg(0.7)$,
note that the discount factor $\discountfactor$
controls the impacts 
of partially connected edges 
for opening a new facility.
Loosely speaking, 
$\CFAlg(\discountfactor)$ 
with larger discount factor $\discountfactor$
opens facilities more aggressively
(see \Cref{fig:numerical synthetic size}),
and some of those facilities are unnecessary
(i.e., removing some facilities from the final 
solution
reduces the total cost).
This observation in fact is what motivated the  2-Chance Greedy Algorithm 
with Myopic Pruning ($\CFAlgP(\discountfactor)$)
described above.
From both \Cref{fig:numerical synthetic ratio} and 
\Cref{table:numerical synthetic ratio},
we observe that 
the average normalized performance of $\CFAlgP(\discountfactor)$
is increasing in
$\discountfactor\in\{0, 0.3, 0.5, 0.7, 1\}$.
Moreover, $\CFAlgP(1)$ not only 
outperforms all other policies
on average, but also beats them in 96 out of 100
(resp.\ 97 out of 100) instances under 
uniform $\{\flowi\}$ (resp.\ distance-discounted $\{\flowi\}$).

\noindent\textsl{\underline{The value of mobility data.}}
When the mobility data $\{\flowi\}$
is not available and the 
social planner only has the 
population (resp.\ employment) 
information
in each location, 
one natural heuristic policy 
is pretending that
each individual can only be connected 
through her home (resp.\ work) location
and then implement $\GDH$ (resp.\ $\GDW$).
It is clear from both \Cref{fig:numerical synthetic ratio} and 
\Cref{table:numerical synthetic ratio}
that both $\CFAlg(\discountfactor)$
and $\CFAlgP(\discountfactor)$
perform noticeably better than $\GDH$ and $\GDW$.
Specifically, the average performance gap between
$\CFAlgP(1)$ and $\GDH$ (resp.\ $\GDW$)
is 14.4\%, 13.7\% (resp.\ 13.4\%, 14.1\%)
under uniform $\{\flowi\}$ and distance-discounted $\{\flowi\}$,
respectively.\footnote{In the 
single-location facility problem,
the solution outputted from JMMSV algorithm 
does not allow local improvement, i.e., 
it is impossible to reduce the total cost 
by removing a facility from this solution.
Therefore, the comparison between 
$\CFAlgP(\discountfactor)$
and $\GDH$, $\GDW$ is fair.}
Such
performance gap highlights the value of mobility 
data $\{\flowi\}$
in this numerical experiment over 
synthetic data.

\subsection{Experiments over US census data}
\label{sec:numerical us cities}
Our second numerical experiment is constructed 
through US census data.

\paragraph{Experimental setup.}
We construct four sets of
\TWOLFLP\ 
instances for 
four cities
in the US, including  
New York City (NYC), Los Angeles metropolitan area (greater LA),
Washington metropolitan area (greater DC),
and Raleigh-Durham-Cary CSA (Research Triangle).

In each instance, 
a location corresponds to a 
Zip Code Tabulation Area (ZCTA).\footnote{ZCTAs are closely 
related to zip codes. The ZCTA code of a block is the most common zip code contained in it; see \citet{ZCTA}.}
For each pair of locations, 
we define their distance as 
the Euclidean distance 
between the centroids of their corresponding 
ZCTAs. 
We set the facility opening cost $\opencost_i$
for each location $i$ as 
\begin{align*}
    \opencost_i \triangleq 
    \costconstructionfactor \cdot 
    \zhvi_i
\end{align*}
where $\zhvi_i$ is the Zillow Home Value Index\footnote{In each instance, 
there are less than 5\% of locations whose 
Zillow Home Value Index (ZHVI) is missing. We set their 
$\zhvi_i$'s as the average ZHVI of other locations.
We also explore other specifications and verify the robustness of our findings.}
recorded in 
\citet{ZHVI},
and $\costconstructionfactor$ is a cost normalization parameter 
which controls the tradeoff between facility opening costs and 
individual connection cost
in our experiments.
Our results are presented for 
different values of $\costconstructionfactor$.

Finally, \citet{LODES} records the total number of individuals 
who reside in one census block (CB) and work in another.
Aggregating it at the ZCTA level, we complete the construction of 
$\{\flowi\}$.
We summarize the number of locations and 
individuals in \Cref{table:instance construction}.

\begin{table}[t]
    \centering
    \caption{The number of locations and individuals
    in \Cref{sec:numerical us cities}.}
    \label{table:instance construction}
    \begin{tabular}[t]{ccccc}
    \toprule
    & 
    NYC & greater LA & greater DC & Research Tri.
     \\
     \midrule
     total locations & 177 & 386 & 313 & 102\\
     total population & 3166075 & 5338918 & 1934411 & 771249\\
    \bottomrule
    \end{tabular}
\end{table}

\paragraph{Policies.}
In this numerical experiment, we consider the same 
set of policies as in \Cref{sec:numerical synthetic}:
$\CFAlg(\discountfactor)$,
$\CFAlgP(\discountfactor)$
for $\discountfactor\in\{0, 0.3, 0.5, 0.7, 1\}$
and 
$\GDH$, $\GDW$.

\paragraph{Results.}
For each city, we 
construct the \TWOLFLP\ instances
under different values of 
cost normalization parameter $\costconstructionfactor$.
Loosely speaking, 
as parameter $\costconstructionfactor$ increases, 
the magnitude of facility opening cost increases and
consequently the sizes of solutions
in all policies decreases.
We consider two regimes:
\emph{low $\costconstructionfactor$ regime} 
(resp.\ 
\emph{high $\costconstructionfactor$ regime})
such that the facilities are opened 
in 40\% to 80\%
(resp.\ 5\% to 20\%) 
of total locations 
in policy $\CFAlgP(1)$.
For each city and each regime, our results
are qualitatively similar.
\Cref{table:numerical us cities ratio low}
and 
\Cref{table:numerical us cities ratio high}
illustrate the normalized performance
of different policies for a problem instance
for each city in the low $\costconstructionfactor$ regime
and the high $\costconstructionfactor$ regime, respectively.
Similar to the experiments over synthetic data in 
\Cref{sec:numerical synthetic},
the normalized performance 
of a policy is defined as 
the ratio between the cost of this policy
over and the minimum cost over policies
$\CFAlgP(\discountfactor)$,
$\discountfactor \in \{0, 0.3, 0.5, 0.7, 1\}$.
 Below we discuss our numerical results in detail.


\begin{table}[t]
    \centering
    \caption{The normalized performance 
    % of 
    % different policies 
    for a problem instance 
    in the low $\costconstructionfactor$ regime.}
    \label{table:numerical us cities ratio low}
    \begin{tabular}[t]{cccccc}
    \toprule
    & 
    \CFAlg(1) & \CFAlg(0.7) & \CFAlg(0.5) &
    \CFAlg(0.3) & \CFAlg(0) 
     \\
     \midrule
     NYC 
     & 1.093 & 1.029 & 1.01 & 1.009 & 1.042 \\
     greater LA
     & 1.067 & 1.024 & 1.012 & 1.008 & 1.018 \\
     greater DC
     & 1.018 & 1.017 & 1.012 & 1.005 & 1.003 \\
     Research Tri.
     & 1.063 & 1.042 & 1.027 & 1.001 & 1.008 \\
    \bottomrule
    \\
    \toprule
    & 
    \CFAlgP(1) & \CFAlgP(0.7) & \CFAlgP(0.5) &
    \CFAlgP(0.3) & \CFAlgP(0) 
     \\
     \midrule
     NYC 
     & 1.0 & 1.001 & 1.001 & 1.008 & 1.042 \\
     greater LA
     & 1.0 & 1.0 & 1.0 & 1.004 & 1.018 \\
     greater DC
     & 1.0 & 1.0 & 1.0 & 1.001 & 1.003 \\
     Research Tri.
     & 1.0 & 1.0 & 1.0 & 1.0 & 1.008 \\
    \bottomrule\\
     \addlinespace[-\aboverulesep] 
    \cmidrule[\heavyrulewidth]{1-3}
    & 
    \GDH & \GDW
     \\
     \cmidrule{1-3}
     NYC
     & 1.223 & 1.115 \\
     greater LA
     & 1.243 & 1.096 \\
     greater DC
     & 1.37 & 1.094 \\
     Research Tri.
     & 1.29 & 1.129 \\
 \cmidrule[\heavyrulewidth]{1-3}
     \addlinespace[-\belowrulesep] 
    \end{tabular}
\end{table}

\begin{table}[t]
    \centering
    \caption{The normalized performance 
    % of 
    % different policies 
    for a problem instance 
    in the high $\costconstructionfactor$ regime.}
    \label{table:numerical us cities ratio high}
    \begin{tabular}[t]{cccccc}
    \toprule
    & 
    \CFAlg(1) & \CFAlg(0.7) & \CFAlg(0.5) &
    \CFAlg(0.3) & \CFAlg(0) 
     \\
     \midrule
     NYC 
     & 1.036 & 1.009 & 1.005 & 1.013 & 1.071 \\
     greater LA
     & 1.021 & 1.01 & 1.014 & 1.024 & 1.054 \\
     greater DC
     & 1.065 & 1.012 & 1.008 & 1.01 & 1.034 \\
     Research Tri.
     & 1.04 & 1.02 & 1.007 & 1.026 & 1.056 \\
    \bottomrule
    \\
    \toprule
    & 
    \CFAlgP(1) & \CFAlgP(0.7) & \CFAlgP(0.5) &
    \CFAlgP(0.3) & \CFAlgP(0) 
     \\
     \midrule
     NYC 
     & 1.0 & 1.002 & 1.002 & 1.012 & 1.071 \\
     greater LA
     & 1.0 & 1.007 & 1.012 & 1.022 & 1.054 \\
     greater DC
     & 1.0 & 1.0 & 1.006 & 1.01 & 1.034 \\
     Research Tri.
     & 1.0 & 1.0 & 1.007 & 1.026 & 1.056 \\
    \bottomrule\\
     \addlinespace[-\aboverulesep] 
    \cmidrule[\heavyrulewidth]{1-3}
    & 
    \GDH & \GDW
     \\
     \cmidrule{1-3}
     NYC
     & 1.147 & 1.031 \\
     greater LA
     & 1.132 & 1.041 \\
     greater DC
     & 1.32 & 1.038 \\
     Research Tri.
     & 1.127 & 1.014 \\
 \cmidrule[\heavyrulewidth]{1-3}
     \addlinespace[-\belowrulesep] 
    \end{tabular}
\end{table}

\noindent\textsl{\underline{The impact of discount factor $\discountfactor$.}}
Similar to the observation in
experiments over synthetic data, 
the performance of $\CFAlg(\discountfactor)$
is single-peaked in 
discount factor 
$\discountfactor\in\{0, 0.3, 0.5, 0.7, 1\}$.
In the low $\costconstructionfactor$ regime,
the best performance of $\CFAlg(\discountfactor)$
is attained at discount factor
$\discountfactor = 0.3$ for all four cities
(\Cref{table:numerical us cities ratio low}).
In the high $\costconstructionfactor$ regime,
the best performance of $\CFAlg(\discountfactor)$
is attained at discount factor $\discountfactor = 0.7$
for greater LA, and discount factor 
$\discountfactor = 0.5$ 
for other cities
(\Cref{table:numerical us cities ratio high}).

By combining with myopic pruning as 
the post-processing step,
$\CFAlgP(1)$ outperforms all other 
policies for all cities in both regimes.
Compared to the low $\costconstructionfactor$ regime,
the performance of $\CFAlgP(\discountfactor)$
is more sensitive in discount factor $\discountfactor$
in the high $\costconstructionfactor$ regime.
In particular,
in \Cref{table:numerical us cities ratio high},
the performance gap 
between $\CFAlgP(1)$ and $\CFAlgP(0)$
in the high $\costconstructionfactor$ regime
is 7.1\%, 5.4\%, 3.4\%, 5.6\% for four cities,
respectively.

\noindent\textsl{\underline{The value of mobility data.}}
Similar to the observation in 
experiments over synthetic data, 
$\CFAlgP(1)$ outperforms 
$\GDH$ and $\GDW$
for all four cities in both regimes.\footnote{Recall that {low $\costconstructionfactor$ regime} 
(resp.\ 
{high $\costconstructionfactor$ regime})
is defined 
such that the facilities are opened 
in 40\% to 80\%
(resp.\ 5\% to 20\%) 
of total locations 
in policy $\CFAlgP(1)$.
In the two extremes (i.e., 
$\costconstructionfactor$
goes to zero
and infinite),
the mobility data 
has no value. 
However,
theoretically speaking,
the value could be substantial
for $\costconstructionfactor$
in between.}
In the low $\costconstructionfactor$ regime,
the performance gap between $\CFAlgP(1)$
and $\GDH,\GDW$ is more than 22.3\%, 9.4\%,
respectively 
(\Cref{table:numerical us cities ratio low}).
% More interestingly,
In the high $\costconstructionfactor$ regime,
the performance gap between $\CFAlgP(1)$
and $\GDH$ is still more than 12.7\%,
but the performance gap between $\CFAlgP(1)$
and $\GDW$ reduces to less than 4.1\%
(\Cref{table:numerical us cities ratio high}).
% \footnote{Recall that {low $\costconstructionfactor$ regime} 
% (resp.\ 
% {high $\costconstructionfactor$ regime})
% is defined 
% such that the facilities are opened 
% in 40\% to 80\%
% (resp.\ 5\% to 20\%) 
% of total locations 
% in policy $\CFAlgP(1)$.
% In the two extremes (i.e., 
% }
% One important factor in the good performance 
% of $\GDW$
% is the relatively high concentration for 
% employments in all four cities.
% See \Cref{fig:numerical us cities PE}.
% In particular, 
% 20\% of locations covers 
% 61.8\%, 62.0\%, 85.9\%, 71.7\%
% of total employments
% in NYC, greater LA, greater DC, Research Triangle,
% respectively.


% \begin{figure}[ht]
%   \centering
%        \subfloat[NYC]
%       {\includegraphics[width=0.45\textwidth]{Paper/figs/numerical/NYC-PE-hist.png}}
%       ~~~~
%       ~~~~
%       \subfloat[greater LA]
%       {\includegraphics[width=0.45\textwidth]{Paper/figs/numerical/LA-PE-hist.png}}
%       \\
%        \subfloat[greater DC]
%       {\includegraphics[width=0.45\textwidth]{Paper/figs/numerical/DC-PE-hist.png}}
%       ~~~~
%       ~~~~
%       \subfloat[Research Triangle]
%       {\includegraphics[width=0.45\textwidth]{Paper/figs/numerical/ResearchTri-PE-hist.png}}
%   \caption{Histogram
%   of number of individuals 
%   who reside/work in each location.}
%    \label{fig:numerical us cities PE}
% \end{figure}

% To summarize our discussion, 
% the mobility data $\{\flowi\}$
% is important when 
% the facility opening cost is relatively low 
% compared to the individual connection cost 
% (i.e., low $\costconstructionfactor$ regime).
% In contrast,
% when the facility opening cost is relatively high
% (i.e., high $\costconstructionfactor$ regime),
% due to the concentration of employments,
% policy $\GDW$ which
% solves the single-location facility problem with 
% employment data   
% achieves similar performance 
% as $\CFAlgP(1)$ which requires 
% the mobility data $\{\flowi\}$.


==> Paper/facility-location-greedy-old.tex <==

\section{A $\greedyapprox$-Approximation Algorithm for 
the \TWOLFLP}

In this section,
we present the first contribution of the paper
--
a $\greedyapprox$-approximation
algorithm (\Cref{alg:greedy modified}) for the \TWOLFLP.
\Cref{alg:greedy modified} is a modified version
of the greedy algorithm (\Cref{alg:greedy}) designed in \citet{JMMSV-02}
for the (single-location) MFLP.
In \Cref{sec:greedy single location},
we present \Cref{alg:greedy}
and explain with examples 
why it does not guarantee 
constant approximation for the \TWOLFLP.
We then present our modified greedy algorithm
(\Cref{alg:greedy modified})
and discuss its $\greedyapprox$-approximation guarantee 
in \Cref{sec:greedy two location}.

\subsection{Failure of Classic Greedy Algorithm}
\label{sec:greedy single location}
In this subsection, we revisit the greedy algorithm (\Cref{alg:greedy})
introduced
in \citet{JMMSV-02},
where authors show a 1.861-approximation of 
\Cref{alg:greedy} for 
the (single-location) MFLP.
% Since the connection cost in our model is not a 
% metric, in \Cref{claim:log(n) bound} we show that 
% \Cref{alg:greedy} is a $\Omega(\log(n))$-approximation 
% in our model. 
% On the other side, we show a modified version
% of the greedy algorithm (\Cref{alg:greedy modified})
% is a $3.722$-approximation.




We use $\plus{x}$
to denote $\max\{x, 0\}$.

\begin{algorithm}[H]
 	\caption{GREEDY \citep{JMMSV-02}}
 	\label{alg:greedy}
 	\vspace{2mm}
 	
%  	Initialize $\dual(j) \gets 0$ for each individual $j\in[n]$
 	
%  	\vspace{1mm}
 	
%  	Initialize $\currentset \gets [n]$
 	
%  	\While{$U \not= \emptyset$}{ 
%  	    \vspace{1mm}
 	    
%  	    Continuously increase $\dual(j)$
%  	    with the same rate 
%  	    for all individuals $j\in \currentset$
 	    
%  	    \While{there exists an unopened store $i$ s.t.\
%  	    $\sum_{j\in \currentset} 
%  	    \plus{\dual(j) - \connectioncost(i, j)} = \opencost(i)$
%  	    }{
%  	    \vspace{1mm}
 	    
%  	    Open store $i$
 	    
%  	    \vspace{1mm}
 	    
%  	    \For{each individual $j\in \currentset$}{
%  	    \vspace{1mm}
%  	    \If{$\dual(j) - \connectioncost(i, j)\geq 0$}{
%  	    \vspace{1mm}
 	    
%  	    Connect individual $j$ with store $i$
 	    
%  	    \vspace{1mm}
%  	    Remove $j$ from $\currentset$, i.e., 
%  	    $\currentset \gets \currentset \backslash \{j\}$
%  	  %  \vspace{1mm}
%  	    }
%  	    }
%  	    }
 	    
%  	    \While{there exists an individual $j\in \currentset$ 
%  	    s.t.\ $\dual(j) = \connectioncost(i, j)$ 
%  	    for some opened store $i$
%  	    }
%  	    {
%  	    \vspace{1mm}
 	    
%  	    Connect individual $j$ with store $i$
%  	    and remove $j$ from $\currentset$ 
 	    
%  	  %  \vspace{1mm}
%  	    }
 	    
%  	    \vspace{1mm}
%  	}
\end{algorithm}

\begin{theorem}[\citealp{JMMSV-02}]
In the (single-location) MFLP,
\Cref{alg:greedy} is a $1.861$-approximation.
\end{theorem}

\begin{claim}
\label{claim:log(n) bound}
In the \TWOLFLP,
\Cref{alg:greedy} is a $\Omega(\log(n))$-approximation.
\end{claim}
\begin{proof}{\textsl{Proof.}}
Consider the following instance of home-workplace facility 
location problem.
There are $n$ individuals and $n + 1$ possible locations for 
stores.

All individual have the same home location
which is also the location of store $n + 1$.
The workplace of each individual $j\in [n]$ 
is also the location of store $j$.
The distance between any two stores is at least $1+\epsilon$
where $\epsilon > 0$ is a sufficiently small constant.
Note that in this instance, for each individual $j\in[n]$,
$$\connectioncost(i, j) \geq (1 + \epsilon)\cdot \indicator{i\not= j}
\;\;\mbox{for every $i\in[n]$; and }
\connectioncost(n + 1, j) = 0
$$

The opening cost $\opencost(i) = \frac{1}{n - i + 1} - \epsilon$
for each store $i \in [n]$;
and $\opencost(n + 1) = 1$.

The optimal solution is opening store $n + 1$ (with total cost 1);
while \Cref{alg:greedy}
opens the first $n$ stores (with total cost $\sum_{i\in [n]}(\frac{1}{i}-\epsilon) = 
\Omega(\log(n))$.
 \ 
\end{proof}

\subsection{2-Chance Greedy Algorithm}
\label{sec:greedy two location}
As we discussed in the previous subsection, 
\Cref{alg:greedy}
fails to achieve constant approximation
in the \TWOLFLP,
since it not only greedily determines
location for facilities, but also 
greedily determines how individuals 
are connected to facilities 
(i.e., through 
their home or workplace)
for every edge $\edge$.
To resolve this issue, 
we introduce a modified version (\Cref{alg:greedy modified})
of \Cref{alg:greedy},
which we name it as 2-chance greedy algorithm.
The main modification
behind \Cref{alg:greedy modified}
is that after we connect individuals on edge $\edge$
to a facility
(suppose we connect their home $\edgehome$ to 
this facility),
we will leave individuals on edge $\edge$ 
the second chance to connect their workplace 
$\edgework$ to facilities in the future.
See \Cref{alg:greedy modified} for a formal description.

\begin{theorem}
\label{thm:greedy modified}
In the \TWOLFLP, 
\Cref{alg:greedy modified}
is a $\greedyapprox$-approximation.
\end{theorem}


\input{Paper/alg-2-choice-greedy}


\begin{remark}Though \Cref{alg:greedy modified}
is described as a continuous procedure (due to the 
continuous update of $\{\greedycounter(\edge)\}$),
it is straightforward to see that 
it terminates deterministically by construction.
Furthermore, \Cref{alg:greedy modified} can be executed
in polynomial time. Note that the conditions in 
while loop (i.e., line 6, line 19) are satisfied 
$O(n^2)$ times. Thus, at any stage of the algorithm,
we can enumerate (in polynomial time) the closest time in which 
the conditions in while loop is satisfied, and
update (in polynomial time)
all variables (i.e, $\stores$, $\{\greedycounter(\edge)\}$,
$\firstchanceset$, $\secondchancesethome$, $\secondchancesetwork$)
accordingly.
\end{remark}

\begin{remark}
Explain the outcome of \Cref{alg:greedy modified} on Example XYZ.
\end{remark}

In the remaining of this section, 
we discuss how to prove the approximation guarantee 
of \Cref{alg:greedy modified}
in \Cref{thm:greedy modified}.
At a high-level, our analysis uses 
a three-step approach as follows.\footnote{
Our analysis extends the dual-fitting argument 
with factor-revealing program 
--
standard technique 
for greedy-style algorithm (e.g., \Cref{alg:greedy})
in the (single-location) MFLP
\citep[see, e.g.,][]{JMMSV-02,MYZ-06,zha-06}.}
In the first step, given an arbitrary instance $\instance$,
we 
lowerbound its optimal cost 
by a linear program~\ref{eq:lp relaxtion}
with exponential number of variables.
In the second step, 
we consider 
the dual program~\ref{eq:lp relaxtion dual}
of the primal program~\ref{eq:lp relaxtion},
and construct a dual assignment for program~\ref{eq:lp relaxtion dual}
whose objective value is weakly higher than the 
cost $\Cost{\stores}$ from solution $\stores$
computed by \Cref{alg:greedy modified}.
In the third step, we argue that this dual assignment 
approximately (i.e., up to a
multiplicative factor)
satisfies the dual constraints
in program~\ref{eq:lp relaxtion dual}.
Specifically, we analyze \Cref{alg:greedy modified}
in details
and introduce a factor-revealing program~\ref{eq:factor revealing program}
to show the aforementioned multiplicative factor is at most 
$\greedyapprox$.
Finally, invoking the weakly duality of linear program finishes 
our analysis. 

Below we provide detailed discussion and related lemmas for the above mentioned three steps. 
In the end of this subsection,
we combine all pieces together to conclude the proof of \Cref{thm:greedy modified}.

\paragraph{Step 1- lower bound of the optimal cost by linear program.} Given an arbitrary location $i\in[n]$,
a subset of edges $\Edge\subseteq[n]$, as well as 
a configuration
% \footnote{Configuration~$\config:
% \Edge\rightarrow\{h, w\}$ specifies that individuals on edge $\edge\in\Edge$
% are connected to location $i$ through $\edge_{\confige}$.} 
$\config:[n]^2\rightarrow\{h, w\}$,
we define \emph{star}  
$\starinstance = (i, \Edge, \config)$
as triple
where a facility is opened in location $i$
and serves individuals on edge $e$ through $\edge_\confige$
for each edge $\edge\in\Edge$.
Let $\starspace$ be the set of all possible stars.
In a slight abuse of notation, for every possible star $\starinstance = (i, \Edge, \config)\in\starspace$,
we define its cost 
$\cost(\starinstance)\triangleq {\opencost_i}
    +
    {
    \sum_{\edge\in\Edge}
    \flowe\cdot \distance(\edge_\confige, i)}$
    where the first term is the facility opening cost in location $i$,
    and the second term is the connection cost between edge $e$ and location $i$
    through $\edge_\confige$
    for each edge~$\edge\in\Edge$.
% $\cost(\starinstance)$ as 
% \begin{align*}
%     \cost(\starinstance) \triangleq \underbrace{\opencost_i}_{
%     \text{facility opening cost in location $i$}
%     }
%     +
%     \underbrace{
%     \sum_{\edge\in\Edge}\distance(\edge_\confige, i)}_{
%     \text{connection cost between edge $e$ and location $i$
%     through $\edge_\confige$}
%     }
% \end{align*}

Consider the following linear program~\ref{eq:lp relaxtion}
as well as its dual program~\ref{eq:lp relaxtion dual}.
\begin{align}
\tag{$\mathcal{P}_{\texttt{OPT-Primal}}$}
\label{eq:lp relaxtion}
    \arraycolsep=5.4pt\def\arraystretch{1}
    &\begin{array}{llll}
    \min\limits_{\mathbf\alloc\geq \mathbf{0}} &
    \displaystyle\sum\nolimits_{\starinstance\in\starspace} 
    \coststar \allocstar 
    & \text{s.t.} & \\
    & \displaystyle\sum\nolimits_{\starinstance=(i, \Edge, \config):
     \edge \in \Edge} 
     \allocstar \geq 1
     & 
     \edge \in [n]^2
     &
     \qquad\quad\qquad\langle\duale\rangle
    \end{array}
    \vspace{2mm}
    \\
\label{eq:lp relaxtion dual}
\tag{$\mathcal{P}_{\texttt{OPT-Dual}}$}
    &\begin{array}{llll}
    \max\limits_{\boldsymbol{\dual}\geq \mathbf{0}} &
    \displaystyle\sum\nolimits_{\edge\in[n]^2} 
    \duale
    & \qquad~\text{s.t.} & \\
    & \displaystyle\sum\nolimits_{
     \edge \in \Edge} 
     \duale \leq \coststar
     & 
     \qquad~\starinstance = (i, \Edge, \config)\in\starspace
     &
     \quad\langle\allocstar\rangle
    \end{array}
\end{align}
It is not hard to see that 
the optimal solution can be converted 
into a feasible solution of program~\ref{eq:lp relaxtion},
and thus 
the optimal objective value of program~\ref{eq:lp relaxtion}
is a lower bound of the optimal cost. 
We formalize this in \Cref{lem:lp relaxation} 
and defer its formal proof into Appendix XYZ.
\begin{lemma}
\label{lem:lp relaxation}
Given any problem instance
in the \TWOLFLP,
the optimal cost is at least the optimal objective value 
of program~\ref{eq:lp relaxtion}.
\end{lemma}

\paragraph{Step 2-
dual assignment construction.}
Let $\stores$ be the solution computed by \Cref{alg:greedy modified}.
Let $\{\greedycounter(\edge)\}$
and $\{\connectmapping(\edge,\edgehome),\connectmapping(\edge,\edgework)\}$
be the value of variables in \Cref{alg:greedy modified} 
when \Cref{alg:greedy modified} terminates.
We partition all edges $[n]^2$ into two disjoint subsets $\singlecountedgeset$
and $\doublecountedgeset$ where 
\begin{align*}
    \singlecountedgeset &\triangleq
    \{\edge\in[n]^2: \connectmapping(\edge,\edgehome) = -1 
    \lor 
    \connectmapping(\edge,\edgework) = -1\}
    \\
    \doublecountedgeset &\triangleq
    \{\edge\in[n]^2: \connectmapping(\edge,\edgehome) \in \stores
    \land 
    \connectmapping(\edge,\edgework) \in \stores\}
\end{align*}
Namely, $\singlecountedgeset$
contains all edges where each edge $\edge\in\singlecountedgeset$
is connected to some facilities in solution $\stores$ through either $\edgehome$ or $\edgework$,
while $\doublecountedgeset$
contains all edges where each edge $\edge\in\singlecountedgeset$
is connected to some facilities in solution $\stores$ 
through both $\edgehome$ and $\edgework$.\footnote{Equivalently, 
$\singlecountedgeset = \secondchancesethome\cup\secondchancesetwork$
where $\secondchancesethome$
and $\secondchancesetwork$ are 
(set) variables in \Cref{alg:greedy modified} when
\Cref{alg:greedy modified} terminates.}

Now consider the following dual assignment construction,
\begin{align}
\label{eq:dual assignment}
\begin{split}
    \edge\in\singlecountedgeset:&\qquad
    \duale \gets \greedycounter(\edge) \\
    \edge\in\doublecountedgeset:&\qquad
    \duale \gets 2\greedycounter(\edge) - 
    \flowe\cdot \max\{\distance(\edgehome, \connectmapping(\edge,\edgehome)),
    \distance(\edgework, \connectmapping(\edge,\edgework))
    \}
\end{split}
\end{align}
The construction of \Cref{alg:greedy modified}
ensures that the total cost of solution $\stores$
is upperbounded by the objective value of our constructed dual assignment.
We formalize this in \Cref{lem:dual assignment objective value}.
\begin{lemma}
\label{lem:dual assignment objective value}
Given any problem instance in the \TWOLFLP,
the total cost $\Cost{\stores}$
of solution $\stores$ computed by \Cref{alg:greedy modified}
is at most the objective value of dual assignment constructed in \eqref{eq:dual assignment},
i.e., $\Cost{\stores} \leq \sum_{\edge\in[n]^2}\duale$.
\end{lemma}
\begin{proof}
Consider a \emph{hypothetical} scenario where
the social planner (i)
opens facilities on every location in solution $\stores$;
(ii) \emph{forces} individuals on edge $\edge\in\singlecountedgeset$
to pay connection cost 
$\flowe\cdot \distance(\edgehome, \connectmapping(\edge,\edgehome))$
if $\connectmapping(\edge,\edgehome)\in\stores$,
or connection cost 
$\flowe\cdot \distance(\edgework, \connectmapping(\edge,\edgework))$ otherwise;
and 
(iii) \emph{forces} individuals on edge~$\edge\in\doublecountedgeset$
to pay connection cost 
$\flowe\cdot (\distance(\edgehome, \connectmapping(\edge,\edgehome))+
\distance(\edgework, \connectmapping(\edge,\edgework)))$.
Then, the total cost of the social planner
in this hypothetical scenario is at most $\sum_{\edge\in\singlecountedgeset}
\greedycounter(\edge) 
+
\sum_{\edge\in\doublecountedgeset}2\greedycounter(\edge)$
due to the construction of \Cref{alg:greedy modified}.

Now consider the \emph{realistic} scenario where the social planner (i)
opens facilities on every location in solution $\stores$;
and 
(ii) asks individuals to select their closest facilities.
In this case, the actual connection cost paid by individuals on edge~$\edge\in\singlecountedgeset$ is at most their connection cost 
in the hypothetical scenario;
and the actual connection cost paid by individuals on edge~$\edge\in\doublecountedgeset$
is at most $\flowe\cdot (\distance(\edgehome, \connectmapping(\edge,\edgehome))+
\distance(\edgework, \connectmapping(\edge,\edgework)))
-
\flowe \cdot 
\max\{\distance(\edgehome, \connectmapping(\edge,\edgehome)),
    \distance(\edgework, \connectmapping(\edge,\edgework))\}$.

Thus, by the comparison between the hypothetical scenario and 
realistic scenario, we have
\begin{align*}
    \Cost{\stores} \leq 
    \sum_{\edge\in\singlecountedgeset} \greedycounter(\edge) 
    +
    \sum_{\edge\in\doublecountedgeset} 2\greedycounter(\edge)
    -
    \sum_{\edge\doublecountedgeset} 
    \flowe \cdot 
\max\{\distance(\edgehome, \connectmapping(\edge,\edgehome)),
    \distance(\edgework, \connectmapping(\edge,\edgework))\}
    =
    \sum_{\edge\in[n]^2}\duale
\end{align*}
which finishes the proof.
\end{proof}

\paragraph{Step 3- approximate feasibility of dual assignment.}
It is straightforward to verify that $\duale \geq 0$
for every edge $\edge\in[n]^2$.
It is remaining to show that for each possible star $\starinstance
=(i, \Edge, \config)\in\starspace$,
the dual constraint associated with $\allocstar$
is approximately satisfied, i.e., 
\begin{align}
\label{eq:dual feasibility approx}
    \sum_{\edge\in\Edge}\duale \leq \dualapprox\cdot \coststar
\end{align}
where we will show $\dualapprox\leq \greedyapprox$
through a factor-revealing program~\ref{eq:factor revealing program}.



% Now we fix an arbitrary star $\starinstance
% =(i,\Edge,\config)\in\starspace$.
Fix an arbitrary natural number $\mHat\in \N_{\geq 1}$
and subset $\singlecountedgesetHat\subseteq[\mHat]$.
Define auxiliary variable $\doublecountedgesetHat \triangleq 
[\mHat]\backslash \singlecountedgesetHat$.
Consider the following optimization program, 
which is parameterized by $\mHat$,
$\singlecountedgesetHat$, $\doublecountedgesetHat$,
and has variables
$\costHat$, $\dualapproxHat$
$\{\muHat(\ell),\distanceHat(\ell),
\distanceHatStar(\ell)\}_{\ell\in[\mHat]}$:
% $\{\muHat(\ell)\}_{\ell\in[\mHat]}$,
% $\{\distanceHat(\ell)\}_{\ell\in[\mHat]}$,
% $\{\distanceHatStar(\ell)\}_{\ell\in[\mHat]}$.
\begin{align*}
\label{eq:factor revealing program}
\tag{$\mathcal{P}_{\texttt{FR}}$}
    \arraycolsep=5.4pt\def\arraystretch{1}
    &\begin{array}{clll}
    \max\limits_{\substack{\costHat, \dualapproxHat, \{\muHat(\ell),\distanceHat(\ell),
\distanceHatStar(\ell)\}_{\ell\in[\mHat]}}} &
    \dualapproxHat
    & \text{s.t.} & \\
    \langle\frcone\rangle
    & 
    \muHat(\ell') \leq \distanceHatStar(\ell) 
    + \distanceHat(\ell) + \distanceHat(\ell')
     & 
     \ell,\ell'\in[\mHat], \ell < \ell'
     &
     \\
    \langle\frctwo\rangle
     &
     \displaystyle\sum\nolimits_{\ell'\in[\ell:\mHat]}
     \plus{\min\{\muHat(\ell),\muHat(\ell')\} - 
     \distanceHat(\ell')}
     \leq 
     \costHat
     &
     \ell\in[\mHat]
     &
     \\
    \langle\frcthree\rangle
     &
     \displaystyle\sum\nolimits_{\ell\in\singlecountedgesetHat}
     \muHat(\ell) 
     +
     \displaystyle\sum\nolimits_{\ell\in\doublecountedgesetHat}
     2\muHat(\ell) - \distanceHatStar(\ell)
     \geq 
     \dualapproxHat\cdot
     \left(
     \costHat 
     +
     \displaystyle\sum\nolimits_{\ell\in[\mHat]}
     \distanceHat(\ell)
     \right)
     &
     \\
    \langle\frcfour\rangle
     &
     \distanceHatStar(\ell) \leq \muHat(\ell)
     &
     \ell\in[\mHat]
     &
     \\
    \langle\frcfive\rangle
     &
     \costHat\geq 0, \dualapproxHat\geq 0
     &&
     \\
    \langle\frcsix\rangle
     &
     \muHat(\ell) \geq 0, 
     \distanceHat(\ell)\geq 0,
     \distanceHatStar(\ell) \geq 0
     &
     \ell\in[\mHat]
     &
    \end{array}
\end{align*}
Below, we first show that any star $\starinstance=(i, \Edge, \config)\in\starspace$
can be converted into a feasible solution of program~\ref{eq:factor revealing program}
with $\dualapproxHat=
\frac{\sum_{\edge\in\Edge}\duale}{\coststar}$.
Then we upperbound the optimal objective value of program~\ref{eq:factor revealing program}
through a series of simplification.

\paragraph{Step 3.1- feasible assignment 
construction of
factor-revealing program.}
Fix an arbitrary star $\starinstance
=(i, \Edge, \config)\in\starspace$.
Let $\timeindex(\edge,\config)$
be the time at which edge $\edge$
is connected to some facility
through $\edge_\confige$ in \Cref{alg:greedy modified}.
If edge $\edge$ is not connected with any facility 
through $\edge_\confige$, we set 
$\timeindex(\edge,\config) = \infty$.
As a sanity check, note that $\timeindex(\edge,\config) \geq \greedycounter(\edge)$ for
all $\edge$ and $\config$.
When $\config$ is clear from the context,
we simplify the notation $\timeindex(\edge,\config)$
as $\timeindex(\edge)$.
Let $\permu$ be a bijection from $\Edge$
to $[|E|]$ such that
$\permu(\edge) \leq \permu(\edge')$
if 
% (a) 
$\timeindex(\edge) \leq \timeindex(\edge') < \infty$
or 
% (b) 
$\timeindex(\edge) = \timeindex(\edge') = \infty
\land 
\greedycounter(\edge) \geq \greedycounter(\edge')$.
For ease of presentation, 
we make the assumption\footnote{In the 
end of this part, 
we discuss why this assumption 
is without loss of generality.} 
that
$\flowe = 1$ for every edge $\edge \in \Edge$.


Now consider the following 
parameter and solution assignment construction
for program~\ref{eq:factor revealing program},
\begin{align*}
    &\qquad 
    \mHat \gets |\Edge|,
    \qquad 
    \singlecountedgesetHat \gets 
    \{\permu(\edge):\edge\in
    \Edge\cap\singlecountedgeset
    \},
    \qquad
    \doublecountedgesetHat \gets
    \{\permu(\edge):\edge\in
    \Edge\cap \doublecountedgeset
    \}
    \\
    &\qquad
    \costHat\gets \cost_i
    \qquad 
    \dualapproxHat
    \gets 
    \frac{\sum_{\edge\in\Edge} \duale}{\coststar}
    \\
    \edge\in\Edge:
    &\qquad
    \muHat(\permu(\edge)) \gets 
    \greedycounter(\edge),
    \qquad 
    \distanceHat(\permu(\edge)) \gets
    \distance(\edge_\confige, i),
    \\
    \edge \in \Edge\cap \singlecountedgeset:
    &\qquad
    \distanceHatStar(\permu(\edge)) \gets 
    \greedycounter(\edge)
    \\
    \edge \in \Edge\cap \doublecountedgeset:
    &\qquad
    \distanceHatStar(\permu(\edge)) \gets 
    \distance(\edge_\confige, \connectmapping(\edge,\edge_\confige))
\end{align*}
where subsets $\singlecountedgeset,\doublecountedgeset
\subseteq [n]^2$
are defined in the beginning of step 2,
and $\connectmapping(\edge,\edge_\confige)$ is defined 
in \Cref{alg:greedy modified}.
% We verify constraints \frcone-\frcsix\
% in a reverse order.

As a sanity check, constraints \frcfour,
\frcfive\ and \frcsix\ 
are satisfied by construction.
Additionally, constraint \frcthree\ 
can be verified by algebra,
\begin{align*}
    &~\sum_{\ell\in\singlecountedgesetHat}
     \muHat(\ell) 
     +
    \sum_{\ell\in\doublecountedgesetHat}
     2\muHat(\ell) - \distanceHatStar(\ell)\\
     =&
     \sum_{\edge\in \Edge\cap \singlecountedgeset} 
     \greedycounter(\edge)
     +
     \sum_{\edge \in \Edge\cap\doublecountedgeset}
     2\greedycounter(\edge) - 
     \distance(\edge_\config,\connectmapping(\edge,\edge_\config))
     \\
     \geq &
     \sum_{\edge\in \Edge\cap \singlecountedgeset} 
     \greedycounter(\edge)
     +
     \sum_{\edge \in \Edge\cap\doublecountedgeset}
     2\greedycounter(\edge) - 
     \max\{\distance(\edgehome,\connectmapping(\edge,\edgehome)),
     \distance(\edgework,\connectmapping(\edge,\edgework))
     \}
     \\
     =&~ 
     \sum_{\edge\in\Edge} \duale
    %  \\
     =
    %  &~ 
     \frac{\sum_{\edge\in\Edge}\duale}{\coststar}
     \cdot
     \coststar\\
     =& 
     ~\frac{\sum_{\edge\in\Edge}\duale}{\coststar}
     \cdot
     \left(\opencost_i + \sum_{\edge\in\Edge} 
     \distance(\edge_\confige,i)\right)
    %  \\
     = 
     \dualapproxHat\cdot \left(\costHat + 
     \sum_{\ell\in[\mHat]}\distanceHat(\ell)\right)
\end{align*}

Now we verify constraint \frcone.
Fix arbitrary edges $\edge, \edge'\in \Edge$ such that 
$\permu(\edge) < \permu(\edge')$. 
By definition, $\timeindex(\edge)\leq\timeindex(\edge')$.
We consider two subcases depending on the value of $\timeindex(\edge)$.
\begin{itemize}[label={-}]
    \item Suppose $\timeindex(\edge) = \infty$.
    In this case, we know that $\edge,\edge' \in \Edge\cap\singlecountedgeset$ due to the definition of $\timeindex(\cdot), \singlecountedgeset$,
    and $\greedycounter(\edge) \geq \greedycounter(\edge')$ due to the definition of $\permu(\cdot)$.
    Thus,
    \begin{align*}
        \muHat(\permu(\edge')) = 
        \greedycounter(\edge') 
        \leq 
        \greedycounter(\edge) 
        =
        \distanceHatStar(\permu(\edge))
        \leq
        \distanceHatStar(\permu(\edge))
        +
        \distanceHat(\permu(\edge)) + \distanceHat(\permu(\edge'))
    \end{align*}
    \item Suppose $\timeindex(\edge) < \infty$.
    Let $i\primed \triangleq\connectmapping(\edge, \edge_\confige)$.
    In this case, we know that edge $\edge$ is connected to 
    facility $i\primed\in\stores$
    through $\edge_\confige$.
    The construction of \Cref{alg:greedy modified}
    ensures that 
    location $i\primed$ is opened (i.e., added into solution $\stores$)
    before time $\timeindex(\edge)$.
    This further implies that $\distance(\edge'_{\config(\edge')}, i\primed) \geq 
    \greedycounter(\edge')$.\footnote{Otherwise, 
    edge $\edge'$ will be connected 
    to facility $i\primed$ through $\edge'_{\config(\edge')}$ before
    $\timeindex(\edge')$}
    Thus,
    \begin{align*}
        \muHat(\permu(\edge')) = 
        \greedycounter(\edge')
        \leq 
        \distance(\edge'_{\config(\edge')}, i\primed)
        &\overset{(a)}{\leq}
        \distance(\edge_\confige,i\primed) 
        +
        \distance(\edge_\confige, i)
        +
        \distance(\edge'_{\config(\edge')}, i)
        \\
        &\overset{(b)}{\leq}
        \distanceHatStar(\permu(\edge))
        +
        \distanceHat(\permu(\edge))
        +
        \distanceHat(\permu(\edge'))
    \end{align*}
    where inequality~(a) holds due to the triangle inequality;
    and inequality~(b) holds due to the assignment construction 
    and $\distance(\edge_\confige,i\primed) \leq \greedycounter(\edge)$.
\end{itemize}

Finally, we verify constraint~\frctwo\ 
by contradiction.
Suppose there exists $\ell\in[\mHat]$ such that
constraint~\frctwo\ is violated,
then we know that
\begin{align}
\label{eq:frctwo inequality}
    \sum_{\edge'\in\Edge:\permu(\edge') \geq \permu(\edge)}
    \plus{\min\{\greedycounter(\edge),\greedycounter(\edge')\}
    - \distance(\edge'_{\config(\edge')}, i)}
    >
    \opencost_i
\end{align}
where edge $\edge \triangleq \permu^{-1}(\ell)$.
Now consider \Cref{alg:greedy modified} at time $\timeindex(\edge)$.
By definition, no edge $\edge'\in\Edge$ 
such that
$\permu(\edge')\geq \permu(\edge)$
has been connected to any facility through its 
$\edge'_{\config(\edge')}$.
In a slight abuse of notation, let $\greedycounter_{\timeindex(\edge)}(\edge')$
be the value of variable $\greedycounter(\edge')$
in \Cref{alg:greedy modified} at time $\timeindex(\edge)$.
By construction, we know that 
$\greedycounter_{\timeindex(\edge)}(\edge')
\geq \min\{\timeindex(\edge),\greedycounter(\edge')\}$.
Thus, we claim that location $i$ is opened (i.e., added into solution $\stores$) no later than time $\timeindex(\edge)$, since
the while-loop condition (line 6) of \Cref{alg:greedy modified}
is satisfied for location $i$ at time $\timeindex(\edge)$,
i.e.,
\begin{align*}
    \sum_{\edge'\in\Edge:\permu(\edge') \geq \permu(\edge)}
    \plus{
    \greedycounter_{\timeindex(\edge)}(\edge')-
    \distance(\edge'_{\config(\edge')}, i)
    }
    &\geq 
    \sum_{\edge'\in\Edge:\permu(\edge') \geq \permu(\edge)}
    \plus{
     \min\{\timeindex(\edge),\greedycounter(\edge')\}-
    \distance(\edge'_{\config(\edge')}, i)
    }
    \\
    &\overset{(a)}{\geq}
    \sum_{\edge'\in\Edge:\permu(\edge') \geq \permu(\edge)}
    \plus{\min\{\greedycounter(\edge),\greedycounter(\edge')\}
    - \distance(\edge'_{\config(\edge')}, i)}
    \\
    &>
    \opencost_i
\end{align*}
where inequality~(a) holds due to the fact that $\timeindex(\edge) \geq 
\greedycounter(\edge)$.

Additionally, inequality~\eqref{eq:frctwo inequality} 
also guarantees that 
there exists $\edge'\in\Edge$ such that $\permu(\edge') 
\geq \permu(\edge)$
and 
\begin{align*}
    \greedycounter_{\timeindex(\edge)}(\edge')
-
\distance(\edge'_{\config(\edge')}, i)
&\geq \min\{\timeindex(\edge),\greedycounter(\edge')\}
- \distance(\edge'_{\config(\edge')}, i)
\\
&\geq \min\{\greedycounter(\edge),\greedycounter(\edge')\}
- \distance(\edge'_{\config(\edge')}, i)
\\
&> 0
\end{align*}
This implies that edge $\edge'$ 
is connected to location $i$ 
through its $\edge'_{\config(\edge')}$ 
no later than time $\timeindex(\edge)$,
which is a contradiction.

\paragraph{Step 3.2- upperbound of factor revealing program.}

The remaining analysis is currently in \Cref{apx:factor revealing program}.
\newpage


 \begin{comment}
Similar to \citet{JMMSV-02},
we define a \emph{star} $\starinstance = (i, L)$
as a pair of one store $i$ and a subset $L$ of locations.\footnote{
We only consider stars which consist 
subset of location where every individual 
has at most one corresponding location (i.e., home or workplace) in it.}
For every star $\starinstance=(i, L)$,
let $\cost(\starinstance) = \opencost(i) + \sum_{\ell\in L}
\distance(i, \ell)$.
It is easy to see that the optimal solution is lowerbounded by\footnote{In all programs, we omit the non-negativity 
constraints of variables for writing simplicity.}
\begin{align}
ss
\\
    \begin{array}{llll}
    \min     & 
    \sum_{\starinstance}
    \cost(\starinstance)\alloc(\starinstance)
    & \text{s.t.}&\\
         &
         \sum_{\starinstance:\home(j) \in \starinstance}
         \alloc(\starinstance)
         +
         \sum_{\starinstance:\workplace(j) \in \starinstance}
         \alloc(\starinstance)
         \geq 1 
         &
         j\in[n],
         ~~~~~
         &
         \langle\dual(j)\rangle
         \\
         \\
    \max     & 
    \sum_{j\in[n]}\dual(j)
    & \text{s.t.}&\\
         &
         \sum_{\ell\in L}\alpha(\ell) \leq \cost(\starinstance)
         ~~~~~
         &
         \starinstance=(i, L),
         &
         \langle\alloc(\starinstance)\rangle
    \end{array}
\end{align}
where we abuse the notation and define $\dual(\home(j)) = 
\dual(\workplace(j)) \triangleq \dual(j)$
for every individual $j\in[n]$.

\begin{claim}
\label{claim:optimal upperbound}
The optimal total cost is lowerbounded by 
program \eqref{eq:lp relaxtion}.
\end{claim}


Now, we consider $\{\dual(j)\}$ 
(or $\{\dual(\ell)\}$ equivalently)
constructed from \Cref{alg:greedy modified}.

\begin{claim}
\label{claim:greedy upperbound}
The total cost of \Cref{alg:greedy modified}
is at most $2\cdot \sum_{j\in[n]} \dual(j)$.
\end{claim}

Due to \Cref{claim:greedy upperbound},
if we show that the dual constraints in \eqref{eq:lp relaxtion}
is satisfied when its left hand side 
is scaling down by $\gamma = 1.861$,
then we finish the proof of \Cref{thm:greedy modified}.

Let $\timeindex(\ell)$
be the time stamp when location $\ell$
is connected to some store in \Cref{alg:greedy modified}.
If location $\ell$ does not get connected to any
store at the end, we set $\timeindex(\ell) = \infty$.

\begin{claim}
For every location $\ell$,
$\timeindex(\ell) \geq \dual(\ell)$.
\end{claim}

Without loss of generality, 
we assume $\timeindex(\ell)$ is weakly increasing
in $\ell$.
Next, we establish two lemmas to characterize 
$\{\dual(\ell)\}$ as follows.

\begin{lemma}
For every store $i\in [m]$, every 
pair of locations $\ell$ and 
$\ell\primed$,
if $\timeindex(\ell) < \timeindex(\ell\primed)$,
then 
\begin{align*}
    \dual(\ell\primed) \leq 
\dual(\ell) + \distance(i,\ell) 
+ \distance(i, \ell\primed).
\end{align*}
\end{lemma}
\begin{proof}
Let $i\primed$ be the store which location $\ell$
is
connected to (since $\timeindex(\ell) < \timeindex(\ell\primed) \leq \infty$, such store $i$ exists).
Note that \Cref{alg:greedy modified} ensures that 
\begin{itemize}
    \item $\dual(\ell)\geq \distance(i\primed, \ell)$
    \item store $i$ is opened weakly before time $\timeindex(\ell) < \timeindex(\ell\primed)$, 
    and thus $\dual(\ell\primed) \leq \distance(i\primed,\ell\primed)$
\end{itemize}
Hence, by triangle inequality,
\begin{align*}
    \dual(\ell\primed) \leq \distance(i\primed, \ell\primed)
    \leq 
    \distance(i\primed, \ell) + 
    \distance(i, \ell) +
    \distance(i, \ell\primed)
    \leq 
    \dual(\ell) + 
    \distance(i, \ell) +
    \distance(i, \ell\primed).
     \ 
\end{align*}
\end{proof}


\begin{lemma}
For every star $\starinstance = (i, L)$, and 
every location $\ell\in L$, 
\begin{align*}
    \sum_{\ell\primed\in L: \ell\primed \geq \ell} 
    \plus{\min\{\dual(\ell), \dual(\ell\primed)\} - \distance(i,\ell\primed)} 
    \leq
    \opencost(i).
\end{align*}
\end{lemma}
\begin{proof}
By contradiction, suppose there exists 
a star $\starinstance = (i, L)$, and 
a location $\ell\in L$
such that 
\begin{align}
\label{eq:contradiction}
    \sum_{\ell\primed\in L: \ell\primed \geq \ell} 
    \plus{\min\{\dual(\ell), \dual(\ell\primed)\} - \distance(i,\ell\primed)} 
    >
    \opencost(i).
\end{align}
Now consider the time stamp $\timeindex(\ell)$.
By definition, 
every location $\ell\primed\in L$ such that $\ell\primed \geq \ell$
is not connected to any store 
and its dual assignment is at least 
$\min\{\timeindex(\ell),\dual(\ell\primed)\}$
at this moment $\timeindex(\ell)$.
Therefore, we can conclude that store $i$
is opened strictly before time stamp $\timeindex(\ell)$,
since
\begin{align*}
    \opencost(i) < 
    \sum_{\ell\primed\in L: \ell\primed \geq \ell} 
    \plus{\min\{\dual(\ell), \dual(\ell\primed)\} 
    - \distance(i,\ell\primed)} 
    \leq 
    \sum_{s\in L: s \geq \ell} 
    \plus{\min\{\timeindex(\ell), \dual(\ell\primed)\} 
    - \distance(i,\ell\primed)} 
\end{align*}
On the other hand, 
\eqref{eq:contradiction} also implies that
there exists at least one location $\ell^* \in L$
such that $\ell^* \geq \ell$ and 
$\min\{\timeindex(\ell), \dual(\ell^*)\} - \distance(i,\ell^*) > 0$.
By the construction of \Cref{alg:greedy modified},
$\ell^*$ should be connected to location $i$ (or some other store)
strictly before time stamp 
$\timeindex(\ell)$ (i.e., $\timeindex(\ell^*) < \timeindex(\ell)$), which leads to a contradiction. 
\end{proof}

Using two lemmas above, we can upperbound $\gamma$ by the 
following factor revealing program parameterized by
a natural number $k\in \N_{\geq 1}$,
\begin{align}
% \label{eq:factor revealing program}\tag{$\mathcal{F}_k$}
    \begin{array}{lll}
    \max     & 
    \frac{\sum_{\ell\in [k]} \dual(\ell)}
    {\opencost + \sum_{\ell\in [k]} \distance(\ell)}
    & \text{s.t.} \\
         &
         \dual(\ell\primed) \leq \dual(\ell) + \distance(\ell)
         +
         \distance(\ell\primed)
         \qquad&
         \ell,\ell\primed\in[k], \ell < \ell\primed
         \\
         &
    \sum_{\ell\primed\in [\ell:k]} 
    \plus{\min\{\dual(\ell), \dual(\ell\primed)\} - \distance(\ell\primed)} 
    \leq
    \opencost
    \qquad
    &
    \ell\in[k]
    \end{array}
\end{align}
where for each dual constraint corresponded to 
star $\starinstance=(i, L)$, 
we can consider $k\gets |L|$,
$\opencost\gets \opencost(i)$,
$\distance(\ell) \gets \distance(i,\ell)$
and $\dual(\ell) \gets \in \dual(\ell)$;
and two constraints correspond to two 
characterization lemmas above.
\YF{This part is a little bit informal since the first lemma
also requires $\timeindex(\ell) < \timeindex(\ell\primed)$. However, it
can be verified that this factor revealing program is 
indeed correct.}

To rewrite program \eqref{eq:factor revealing program}
as a linear program, we 
consider all possible permutation $\permu$
for $[k]$ and define 
\begin{align}
\label{eq:factor revealing LP}\tag{$\mathcal{F}_{k,\permu}$}
    \begin{array}{lll}
    \max     & 
    \sum_{\ell\in [k]} \dual(\ell)
    & \text{s.t.} \\
    &
     \opencost + \sum_{\ell\in [k]} \distance(\ell) \leq 1
     &
    \\
    &
    \dual(\ell) \leq \dual(\ell\primed)
    &
    \ell,\ell\primed\in[k], \permu(\ell) <  \permu(\ell\primed)
    \\
         &
         \dual(\ell\primed) \leq \dual(\ell) + \distance(\ell)
         +
         \distance(\ell\primed)
         \qquad&
         \ell,\ell\primed\in[k], \ell < \ell\primed
         \\
         &
    \sum_{\ell\primed\in [\ell:k]} 
    \xi(\ell, \ell\primed)
    \leq
    \opencost
    \qquad
    &
    \ell\in[k]
    \\
    &
    \xi(\ell, \ell\primed)\geq \dual(\ell) - \distance(\ell\primed)
    &
    \ell,\ell\primed\in[k],
    \ell\leq \ell\primed,
    \permu(\ell) < \permu(\ell\primed)
    \\
    &
    \xi(\ell, \ell\primed)\geq \dual(\ell\primed) - \distance(\ell\primed)
    &
    \ell,\ell\primed\in[k],
    \ell\leq \ell\primed,
    \permu(\ell) > \permu(\ell\primed)
    \end{array}
\end{align}
\YF{The factor revealing LP \eqref{eq:factor revealing LP}
requires a parameter $\sigma$ 
to handle $\min\{\dual(\ell),\dual(\ell\primed)\}$.
Intuitively speaking, LP \eqref{eq:factor revealing LP}
should attain its worst ratio when $\sigma = (1, 2, \dots, k)$,
i.e., when
$\dual(\ell)$ is weakly increasing in $\ell$.
I numerically verified this intuition for $k \leq 8$
and it seems to be correct.
However, I cannot come up with a formal argument to proof 
this intuition at this moment. 
}
\YF{When $\sigma = (1, 2, \dots, k)$,
this is exactly the same LP in \citet{JMMSV-02}.}

\end{comment}

==> Paper/prelim-old.tex <==
\section{Preliminaries}
\label{sec:prelim}


In this paper, 
we study the cost-minimization
for the \emph{$2$-location (uncapacitated)
facility location problem (2-LFLP)} defined as follows.

There is a metric space 
$([n], \distance)$
with $n$ locations
indexed by $[n]\triangleq \{1,\dots, n\}$ and 
distance function (i.e., metric) $\distance:[n]\times[n] 
\rightarrow
\reals_+$.
For each location $i\in[n]$,
let $\popi$ denote
the number of individuals who reside 
in location~$i$,
and 
$\empj$ denote 
the number of individuals who work
in location~$j$.
For each pair of location $(i, j)\in[n]\times[n]$,
we denote $\flowi$ by the number of 
individuals who reside in location $i$
and work in location $j$.
By definition, we have 
$\popi = \sum_{j\in[n]}\flowi$
and $\empj = \sum_{i\in[n]}\flowi$
for every $i, j\in[n]$.

We also use 
terminology \emph{edge} $\edge = (\edgehome, \edgework)
\in[n]^2$
to denote individuals who reside in location~$\edgehome$ 
and work in location~$\edgework$.
In a slight abuse of notation, 
we define $\flowe \triangleq \flow_{\edgehome\edgework}$ 
as the number of individuals on edge $\edge$,
and $\distance(\edge, k) \triangleq 
\min\{\distance(\edgehome,k),\distance(\edgework,k)\}$
as the closest distance between location $k\in[n]$
and individuals on edge $\edge$.\footnote{It is easy to verify that 
$\{\distance(\edge, k)\}_{\edge\in[n]^2,k\in[n]}$ may not satisfy the triangle inequality.}
Throughout the paper, we use notation $(i, j)$
and $\edge$ interchangeably.


There is a social planner who
wants to choose a subset 
$\stores\subseteq[n]$
as the locations of her facilities 
to minimize the total cost.
Specifically, 
given an arbitrary solution $\stores\subseteq [n]$
as the location of facilities, 
the total cost $\Cost{\stores}$ is defined as
a combination of the facility opening cost and 
the
individual connection cost:\footnote{Namely, for each individual who resides in location $i$ and work in location $j$,
there is a connection cost which is equal to 
the minimum of the distances between her home or workplace to the closest 
facility in solution $\stores$.}
\begin{align*}
    \Cost{\stores}
    \triangleq
    \displaystyle\sum_{i\in\stores}\opencosti
    +
    \sum_{\edge\in[n]^2}
    \flowe \cdot 
    \min_{k\in\stores}
    \distance(e,k)
\end{align*}
where 
$\opencosti$ is the facility opening cost 
for location $i$.
Here the connection cost 
% , and 
% $\distance_\stores(i) \triangleq \min_{k\in\stores}
% \distance(i, k)$
% is the distance between location $i$ to the closest
% facility in solution $\stores$.


\paragraph{Mobility data.}
% In this paper we consider 
% the following two scenarios for the social planner
% --
% \emph{local data scenario} and 
% \emph{full data scenario},
% depending on whether she has access 
% to the mobility data.
% Specifically, 
Given an arbitrary problem instance 
$\instance = ([n], \distance, \pops, \emps, 
\flows, \opencosts)$,
we denote $\mobilitydata \triangleq \flows$ as the \emph{mobility data},
and $\partialdata \triangleq ([n], \distance, \pops, \emps,  \opencosts)$ as 
the \emph{local data}.
We say 
mobility data $\mobilitydata$
is consistent with 
local data $\partialdata$
if $\popi = \sum_{j\in[n]}\flowi$
and $\empj = \sum_{i\in[n]}\flowi$
for every location $i, j\in[n]$.


\paragraph{Approximation.}
Given a problem instance $\instance$,
we say a solution $\stores\subseteq[n]$
is a \emph{$\approxratio$-approximation} to the optimal solution $\OPT$
if 
\begin{align*}
    \Cost{\stores} \leq \approxratio \cdot 
    \Cost{\OPT}
\end{align*}
where optimal solution $\OPT \triangleq 
\argmin\limits_{\stores'\subseteq[n]}\Cost{\stores'}$
is the solution which minimizes the total cost.

We say an algorithm $\ALG$ is a \emph{$\approxratio$-approximation}
if for every problem instance $\instance$,
the solution $\ALG(\instance)$ computed from algorithm $\ALG$
is a $\approxratio$-approximation.

\paragraph{(Single-location) facility location problem.}
The \TWOLFLP\ generalizes 
the classical \emph{(single-location) metric facility location problem (MFLP)} \citep{STA-97}.
In particular, the former problem becomes 
the latter problem when we further impose 
the restriction on the problem instances such that
the home location of 
every individual
is the same as her workspace,
i.e., $\flowi = 0$ for every~$i\not= j$.

The \TWOLFLP\ can also be considered as 
a special case of 
the classical \emph{(single-location) non-metric facility location problem (NMFLP)} \citep{hoc-82}.
In particular, every problem instance 
in 
the \TWOLFLP\ is equivalent to a problem instance
in the NMFLP where we consider each edge $\edge$
as a new location
with opening cost $\infty$.\footnote{Recall that 
distance $\distance$ is defined as $
\distance(\edge, k) = \min\{\distance(\edgehome,k),
\distance(\edgework,k)\}$
which may not satisfy the triangle inequality. 
To complete the instance construction in NMFLP, 
we note that the distance $\distance(\edge,\edge')$
between location $\edge$ and $\edge'$
does not matter (and thus can be set arbitrarily), 
since
their opening costs are set to be $\infty$.}

The (single-location) MFLP as well as NMFLP
has been studied extensively in the literature. 
Under the standard computation complexity hardness assumption, 
it is known that there exists no polynomial-time algorithm
which can compute the optimal solution even for MFLP.
The approximation ratios achievable by polynomial-time algorithms 
are summarized in Figure XYZ.


==> Paper/weakly-factor-revealing-program.tex <==
\subsection{Construction of factor-revealing program~\ref{eq:weakly factor-revealing program}}
\label{sec:primal dual framework}

In this part,
we use the primal-dual analysis framework
(initially developed by \citealp{JMMSV-02}
for the JMMSV algorithm in the MFLP)
and 
provide  
%introduce 
three lemmas 
that shed light on the structure of  the 2-Chance Greedy Algorithm. We then leverage these to obtain our main approximation result  for \ref{eq:weakly factor-revealing program}, stated next:
\begin{lemma}
\label{lem:weakly factor-revealing program}
In the \TWOLFLP,
the approximation ratio of 
the 2-Chance Greedy Algorithm 
with discount factor $\discountfactor\in[0, 1]$
is 
at most equal to $\WFRapproxratio$ where
\begin{align*}
    \WFRapproxratio=
    \sup\limits_{\mHat\in\naturals, 
\permu
% \in[\mHat]^{\positivereals}
:[\mHat]\rightarrow\positivereals}
\Obj{\text{\ref{eq:weakly factor-revealing program}}}
\end{align*}
Here \ref{eq:weakly factor-revealing program}
is the maximization program parameterized by 
$\mHat\in\naturals$ 
and $\permu:[\mHat]\rightarrow\positivereals$
defined as follows:
\begin{align}
\tag{$\WFRP{\mHat,\permu,\discountfactor}$}
\label{eq:weakly factor-revealing program}
&\arraycolsep=1.4pt\def\arraystretch{2.2}
    \begin{array}{llll}
    \max\limits_{
    \substack{\costHat\geq 0,
    \\
    \muHatBf,
    \distanceHatBf,
    \distanceHatStarBf \geq 
    \zerobf
    }} &
     \displaystyle\sum\nolimits_{\ell\in[\mHat]}
     (1 + \discountfactor)
    \cdot
    \muHat(\ell) - 
    \discountfactor\cdot\distanceHatStar(\ell)
    & \text{s.t.} & \\
    \WFRCtriangleineq &
    \discountfactor\cdot \muHat(\ell') \leq 
    \distanceHatStar(\ell) + \distanceHat(\ell)
    +
    \distanceHat(\ell')
    &
    \ell,\ell'\in[\mHat],
    \permu(\ell) < \permu(\ell')
    &
    \\
    \WFRCcontribution &
    \displaystyle\sum\nolimits_{\ell'\in[\mHat]:
    \permu(\ell') \geq \permu(\ell)}
    \plus{\discountfactor\cdot 
    \min\left\{\muHat(\ell), \muHat(\ell')\right\} - \distanceHat(\ell')}
    \leq \costHat\quad
    &
    \ell \in[\mHat]
    \\
    \WFRCconnectcost &
    \distanceHatStar(\ell) \leq \muHat(\ell)
    &
    \ell\in[\mHat]
    \\
     \WFRCtotalcost &
     \costHat 
     +
     \displaystyle\sum\nolimits_{\ell\in[\mHat]}
     \distanceHat(\ell)
     \leq 1
     &
    \end{array}
\end{align}
\end{lemma}
In the above lemma,
program~\ref{eq:weakly factor-revealing program}
is parameterized by a natural number $\mHat\in\naturals$,
and function~$\permu\in\positivereals^{\mHat}$ which maps 
$[\mHat]$ to ${\positivereals}$.
It has non-negative variables 
$\costHat$, $\{\muHat(\ell),\distanceHat(\ell),
\distanceHatStar(\ell)\}_{\ell\in[\mHat]}$.
Function $\permu$ as a parameter of program~\ref{eq:weakly factor-revealing program}
essentially specifies 
a total preorder\footnote{Total preorder 
is a binary relation 
satisfying reflexivity, transitivity, and is total.}
over $[\mHat]$, each of which in turn correspond to different sets
of constraints in~\WFRCtriangleineq\ and \WFRCcontribution.
All
constraints other than
constraint~\WFRCcontribution
~are linear, as is  the  objective function.


As we discussed after \Cref{thm:greedy modified},
though \Cref{lem:weakly factor-revealing program}
already provides an upperbound on the approximation ratio
of the 2-Chance Greedy Algorithm, 
it is hard to evaluate it,  since it is the supremum of 
non-linear/non-quadratic/non-convex\footnote{Due to term $\min\{\muHat(\ell),\muHat(\ell')\}$,
it is hard to change 
constraint~\WFRCcontribution\ with a linear/quadratic constraint by 
introducing additional auxiliary variables and inequalities.
Furthermore, because of constraint~\WFRCcontribution, 
the set of feasible solution is not convex.}
programs~\{\ref{eq:weakly factor-revealing program}\}
over all possible $\mHat\in\naturals$ and $\permu\in \positivereals^{\mHat}$.
In \Cref{sec:strongly factor-revealing program},
we transform this family of factor-revealing 
programs
~\{\ref{eq:weakly factor-revealing program}\}
into the strongly factor-revealing programs~\{\ref{eq:strongly factor-revealing quadratic program}\},
which can be both analytically analyzed (albeit leading to loose bounds)
and numerically computed.

In the remaining of this part, we 
sketch the proof of \Cref{lem:weakly factor-revealing program}.
The proof uses an approach 
similar to that of \citet{JMMSV-02}
for the JMMSV algorithm in the MFLP.
At a high-level, the analysis 
proceeds in three steps:
In the first step, given an arbitrary \TWOLFLP\
instance,
we 
lowerbound its optimal cost 
via a linear program and its dual program~\ref{eq:lp relaxtion}.
In the second step, 
we construct a dual assignment for program~\ref{eq:lp relaxtion}
whose objective value is weakly higher than the 
total cost $\Cost{\stores}$ from solution $\stores$
computed by \Cref{alg:greedy modified}.
In the third step, we argue that this dual assignment 
approximately (i.e., up to a
multiplicative factor)
satisfies the dual constraints
in program~\ref{eq:lp relaxtion}.
Specifically, we present 
three structural lemmas on \Cref{alg:greedy modified}
and 
show that 
the aforementioned multiplicative factor 
can be captured by factor-revealing program~\ref{eq:weakly factor-revealing program}
for some parameters $\mHat$ and $\permu$.
Finally, invoking the weakly duality of linear program finishes 
our analysis. 


Below we provide a detailed discussion and  lemmas that formalize  the above mentioned three steps. 
In the end of this subsection,
we combine all pieces together to conclude the proof of \Cref{lem:weakly factor-revealing program}.

\paragraph{Step 1- lower bound of the optimal cost via linear program.} Given an arbitrary location $i\in[n]$,
a subset of edges $\EdgeTilde\subseteq\Edge$, as well as 
a configuration
$\config:\Edge\rightarrow\hwset$,
we define \emph{star} as the triple~$\starinstance = (i, \Edge, \config)$.
Here, $i$ is interpreted as the location where a facility is opened,
and this facility serves 
every edge $\edge\in\EdgeTilde$
through home/work location $\edge_{\confige}$.
Let $\starspace$ be the set of all possible stars.
With a slight abuse of notation, for every possible star $\starinstance = (i, \EdgeTilde, \config)\in\starspace$,
we define its cost as
$\cost(\starinstance)\triangleq {\opencost_i}
    +
    {
    \sum_{\edge\in\EdgeTilde}
    \flowe\cdot \distance(\edge_\confige, i)}$
    where the first term is the facility opening cost in location $i$,
    and the second term is the total 
    connection cost between edge $\edge$ and facility $i$
    through $\edge_\confige$
    over all edge~$\edge\in\EdgeTilde$.
% $\cost(\starinstance)$ as 
% \begin{align*}
%     \cost(\starinstance) \triangleq \underbrace{\opencost_i}_{
%     \text{facility opening cost in location $i$}
%     }
%     +
%     \underbrace{
%     \sum_{\edge\in\Edge}\distance(\edge_\confige, i)}_{
%     \text{connection cost between edge $e$ and location $i$
%     through $\edge_\confige$}
%     }
% \end{align*}

Consider the following linear program~\ref{eq:lp relaxtion}
as well as its dual program.
\begin{align}
\tag{$\mathcal{P}_{\texttt{OPT}}$}
\label{eq:lp relaxtion}
    \arraycolsep=5.4pt\def\arraystretch{1}
    &\begin{array}{llllll}
    \min\limits_{\mathbf\alloc\geq \zerobf} &
    \displaystyle\sum\nolimits_{\starinstance\in\starspace} 
    \coststar \allocstar 
    & \text{s.t.} &
    \quad
    \max\limits_{\boldsymbol{\dual}\geq \zerobf} &
    \displaystyle\sum\nolimits_{\edge\in\Edge} 
    \duale
    & \text{s.t.} \\
    & \displaystyle\sum\nolimits_{\starinstance=(i, \Edge, \config):
     \edge \in \Edge} 
     \allocstar \geq 1
     \quad
     & 
     \edge \in \Edge
     &
    &\displaystyle\sum\nolimits_{
     \edge \in \Edge} 
     \duale \leq \coststar
     \quad
     & 
     \starinstance = (i, \EdgeTilde, \config)\in\starspace
    \end{array}
\end{align}
It is not hard to see that 
the optimal solution $\OPT$ can be converted 
into a feasible solution of program~\ref{eq:lp relaxtion}, 
and thus 
the optimal objective value 
$\Obj{\text{\ref{eq:lp relaxtion}}}$
of program~\ref{eq:lp relaxtion}
is a lower bound on the optimal cost $\Cost{\OPT}$. 
We formalize this in \Cref{lem:lp relaxation} 
and defer its formal proof into \Cref{apx:lp relaxation}.
\begin{restatable}{lemma}{lprelaxation}
\label{lem:lp relaxation}
Given any \TWOLFLP\ instance,
the optimal cost $\Cost{\OPT}$ is at least equal to $\Obj{\text{\ref{eq:lp relaxtion}}}$.
\end{restatable}

\paragraph{Step 2-
dual assignment construction.}
Let $\stores$ be the solution computed by \Cref{alg:greedy modified}.
Let $\{\greedycounter(\edge)\}$
and $\{\connectmapping(\edge,\edgeindex)\}_{
\edge\in\Edge,\edgeindex\in\hwset}$
be the values of these variables at the termination of \Cref{alg:greedy modified}.
We partition all edges $\edge\in\Edge$ into two disjoint subsets  
$\singlecountedgeset$
and $\doublecountedgeset$ 
% and 
 as follows: 
\begin{align*}
    \doublecountedgeset &\triangleq
    \{\edge\in\Edge: \connectmapping(\edge,h) \not= \nullsymbol
    \land 
    \connectmapping(\edge,w)  \not= \nullsymbol
    \land 
    \connectmapping(\edge,h) \not = \connectmapping(\edge,w)\}
    \qquad
    \singlecountedgeset \triangleq
    \Edge\backslash\doublecountedgeset
\end{align*}
Namely, $\singlecountedgeset$
contains every edge $\edge\in\Edge$ 
that is either partially connected or fully connected to 
a single facility;
while $\doublecountedgeset$
contains every edges$\edge\in\Edge$ 
that is fully connected to 
two facilities.

Now consider the following dual assignment (which is not feasible in the dual problem in general),
\begin{align}
\label{eq:dual assignment}
\begin{split}
    \edge\in\singlecountedgeset:&\qquad
    \duale \gets \flowe\cdot \greedycounter(\edge) \\
    \edge\in\doublecountedgeset:&\qquad
    \duale \gets \flowe\cdot (1 + \discountfactor) \cdot \greedycounter(\edge) - 
    \flowe\cdot \discountfactor 
    \cdot \max\{
    \distance(\edgehome, \connectmapping(\edge,h)),
    \distance(\edgework, \connectmapping(\edge,w))
    \}
\end{split}
\end{align}
The construction of \Cref{alg:greedy modified}
ensures that the total cost of solution $\stores$
is upperbounded by the objective value of the constructed dual assignment.
We formalize this in \Cref{lem:dual assignment objective value}.
\begin{lemma}
\label{lem:dual assignment objective value}
Given any \TWOLFLP\ instance,
the total cost $\Cost{\stores}$
of solution $\stores$ computed by \Cref{alg:greedy modified}
with discount factor $\discountfactor\in[0, 1]$
is at most the objective value of 
the dual assignment constructed in \eqref{eq:dual assignment},
i.e., $\Cost{\stores} \leq \sum_{\edge\in\Edge}\duale$.
\end{lemma}
\begin{proof}
First, consider a \emph{hypothetical} scenario where
the social planner (i) opens
all facilities in solution $\stores$;
(ii) \emph{forces} individuals on edge $\edge\in\singlecountedgeset$
to pay connection cost 
$\flowe\cdot \distance(\edgehome, \connectmapping(\edge,h))$
if $\connectmapping(\edge,h)\in\stores$,
and connection cost 
$\flowe\cdot \distance(\edgework, \connectmapping(\edge,w))$ otherwise;
and 
(iii) \emph{forces} individuals on edge~$\edge\in\doublecountedgeset$
to pay connection cost 
$\flowe\cdot (\distance(\edgehome, \connectmapping(\edge,h))
+
\distance(\edgework, \connectmapping(\edge,w)))$.
It can be readily seen that  the total cost of the social planner
in this hypothetical scenario is at most $\sum_{\edge\in\singlecountedgeset}
\flowe\cdot \greedycounter(\edge) 
+
\sum_{\edge\in\doublecountedgeset}\flowe\cdot (1 +\discountfactor)\cdot \greedycounter(\edge)$.

Now consider the \emph{realistic} scenario where the social planner 
(i) opens
all facilities in solution $\stores$;
and 
(ii) asks individuals to select their closest facilities.
In this case, the actual connection cost paid by individuals on edge~$\edge\in\singlecountedgeset$ is at most their connection cost 
in the hypothetical scenario;
and the actual connection cost paid by individuals on edge~$\edge\in\doublecountedgeset$
is at most $\flowe\cdot (\distance(\edgehome, \connectmapping(\edge,h))+
\distance(\edgework, \connectmapping(\edge,w)))
-
\flowe \cdot 
\max\{\distance(\edgehome, \connectmapping(\edge,h)),
    \distance(\edgework, \connectmapping(\edge,w))\}$.

By the comparison between the hypothetical  and the
realistic scenarios, we have
\begin{align*}
    &~\Cost{\stores} 
    \\
    \leq& 
    \sum_{\edge\in\singlecountedgeset} \flowe \cdot 
    \greedycounter(\edge) 
    +
    \sum_{\edge\in\doublecountedgeset} 
    \flowe\cdot (1 + \discountfactor)
    \cdot \greedycounter(\edge)
    -
    \sum_{\edge\in\doublecountedgeset} 
    \flowe \cdot 
\max\{\distance(\edgehome, \connectmapping(\edge,h)),
    \distance(\edgework, \connectmapping(\edge,w))\}
    \\
    \leq&
    \sum_{\edge\in\singlecountedgeset} \flowe \cdot 
    \greedycounter(\edge) 
    +
    \sum_{\edge\in\doublecountedgeset} 
    \flowe\cdot (1 + \discountfactor)
    \cdot \greedycounter(\edge)
    -
    \sum_{\edge\in\doublecountedgeset} 
    \flowe \cdot 
    \discountfactor\cdot
\max\{\distance(\edgehome, \connectmapping(\edge,h)),
    \distance(\edgework, \connectmapping(\edge,w))\}
    \\
    =&
    \sum_{\edge\in\Edge}\duale
\end{align*}
which finishes the proof.
\end{proof}

\paragraph{Step 3- approximate feasibility of dual assignment.}
It is straightforward to verify that the constructed dual assignment is non-negative, i.e., 
$\duale \geq 0$
for every edge $\edge\in\Edge$.
It remains to show that for each possible star $\starinstance
=(i, \EdgeTilde, \config)\in\starspace$,
the dual constraint associated with primal variable 
$\allocstar$
is approximately satisfied (with an approximation factor of $\Gamma_{FR}$ defined in Lemma \ref{lem:weakly factor-revealing program}).  We formalize this
 in \Cref{lem:dual assignment approx feasible}.

\begin{restatable}{lemma}{dualassignmentapproxfeasible}
\label{lem:dual assignment approx feasible}
Given any \TWOLFLP\ instance,
the dual assignment constructed in \eqref{eq:dual assignment}
is $\WFRapproxratio$-approximately feasible, i.e., 
for each star $\starinstance
=(i, \EdgeTilde, \config)\in\starspace$,
\begin{align}
\label{eq:dual feasibility approx}
    \sum_{\edge\in\EdgeTilde}\duale \leq \WFRapproxratio\cdot \coststar
\end{align}
\end{restatable}

At a high level, we show that
for every \TWOLFLP\ instance, and every star $\starinstance$,
the components in $\duale$ and $\coststar$,
i.e., $\{\greedycounter(\edge), \distance(\edge_\confige, \connectmapping(\edge, \confige)),
\opencost_i, 
\distance(\edge_\confige, i)\}$
can be straightforwardly converted to
a feasible solution (after normalization)
of program~\ref{eq:weakly factor-revealing program}
with properly selected parameters $\mHat$ and $\permu$,
and ${\sum_{\edge\in \EdgeTilde} \duale}/{\coststar}$
is at most the objective value of this constructed solution.
In particular,  
let
$\edgetoellmappingconfig$ be an arbitrary bijection 
from $\EdgeTilde$ to $[\mHat]$.
We set 
$\mHat$ equal to the size of $\EdgeTilde$
(i.e., 
$\mHat = |\EdgeTilde|$),\footnote{For ease of presentation, in step 3 we make the assumption
that $\flowe \equiv 1$ for every edge $\edge\in\EdgeTilde$. 
This assumption is without loss of generality, since our argument
can be directly extended by resetting $\mHat$
equal to the total populations over all edges in $\EdgeTilde$,
i.e., $\mHat= \sum_{\edge\in\EdgeTilde}\flowe$, and treat each
of those individuals separately.}
and
$\permu(\edgetoellmappingconfig(\edge))$ 
equal to the time stamp when edge $\edge$
is connected to facility $\connectmapping(\edge, \confige)$
through home/work location $\confige$
for each edge $\edge\in\EdgeTilde$.
If $\connectmapping(\edge, \confige) = \nullsymbol$, 
we let $\permu(\edgetoellmappingconfig(\edge))$ 
be the time stamp of the
termination of the algorithm.
We construct a solution
$\{\costHat\primed,\muHat\primed(\ell),\distanceHat\primed(\ell),
\distanceHatStar\primed(\ell)\}$ for program~\ref{eq:weakly factor-revealing program} as follows:\footnote{Here we use superscript $\dagger$
to denote the solution in program~\ref{eq:weakly factor-revealing program}.}
\begin{align*}
    &\qquad\costHat\primed \gets \normalizefactor \cdot {\opencost_i},
    \\
    \edge\in\EdgeTilde:&
    \qquad
    \muHat\primed(\edgetoellmappingconfig(\edge)) \gets 
    \normalizefactor \cdot {\greedycounter(\edge)},
    \quad 
    \distanceHat\primed(\edgetoellmappingconfig(\edge)) \gets 
    \normalizefactor \cdot 
    {\distance(\edge_\confige, i)},
    \\
    % &\distanceHatStar\primed(\edgetoellmappingconfig(\edge)) \gets 
    % \left\{
    % \begin{array}{ll}
    %  \normalizefactor\cdot {\distance(\edge_\confige, \connectmapping(\edge, \confige))}
    %  & 
    %  \text{if $\connectmapping(\edge, \confige)\not=\nullsymbol$}\\
    %   \normalizefactor\cdot {\greedycounter(\edgetoellmappingconfig(\edge)) }
    %   & 
    %   \text{if $\connectmapping(\edge, \confige)=\nullsymbol$}
    % \end{array}
    % \right.
    \edge\in\EdgeTilde\cap \singlecountedgeset:
    &\qquad
    \distanceHatStar\primed(\edgetoellmappingconfig(\edge)) \gets 
    \normalizefactor\cdot {\greedycounter(\edge) },
    \\
    \edge\in\EdgeTilde\cap \doublecountedgeset:
    &\qquad
    \distanceHatStar\primed(\edgetoellmappingconfig(\edge)) \gets 
    \normalizefactor\cdot \distance(\edge_\confige, \connectmapping(\edge, \confige))
\end{align*}
where $\normalizefactor = \frac{1}{\opencost_i+\sum_{\edge\in\EdgeTilde}\distance(\edge_\confige, i)}$ is the normalization factor\footnote{If $\opencost_i+\sum_{\edge\in\EdgeTilde}\distance(\edge_\confige, i) = 0$, 
the algorithm construction ensures that $\greedycounter(\edge) = 0$
for every edge $\edge\in\EdgeTilde$ and thus the dual constraint is satisfied with equality trivially.} which guarantees the feasibility of 
constraint~\WFRCtotalcost.

The formal proof of \Cref{lem:dual assignment approx feasible}
using the above solution construction
is deferred to \Cref{apx:dual assignment approx feasible}.
Here we present a structure lemma of the 2-Chance Greedy Algorithm
with discount factor $\discountfactor\in[0, 1]$
that is used to show the feasibility of the first three constraints \WFRCtriangleineq
-\WFRCconnectcost\ 
in program~\ref{eq:weakly factor-revealing program}.
With a slight abuse of notation, in this lemma,
we simplify the notation $\permu(\edgetoellmappingconfig(\edge))$
as $\permu(\edge)$.

\begin{lemma}
\label{lem:structural lemma}
Given any \TWOLFLP\ instance, 
and any star $\starinstance 
= (i, \EdgeTilde, \config)\in\starspace$,
for the 2-Chance Greedy Algorithm with discount factor $\discountfactor\in
[0, 1]$,
\begin{enumerate}
\item [(i)]
for every $\edge,\edge'\in \EdgeTilde$, 
if $\permu(\edge) < \permu(\edge')$,
then $\connectmapping(\edge,\confige) \not=\nullsymbol$
and 
\begin{align*}
    \discountfactor\cdot \greedycounter(\edge') \leq 
\distance(\edge_\confige, \connectmapping(\edge,\confige))
+
\distance(\edge_\confige, i)
+
\distance(\edge'_{\config(\edge')}, i)
\end{align*}

\item [(ii)] 
for every $\edge\in \EdgeTilde$, 
\begin{align*}
    \sum_{\edge'\in\EdgeTilde:\permu(\edge') \geq \permu(\edge)}
    \plus{
    \discountfactor\cdot 
    \min\left\{
    \greedycounter(\edge),
    \greedycounter(\edge')
    \right\}
    -
    \distance(\edge'_{\config(\edge')}, i)
    }
    \leq
    \opencost_i
\end{align*}

\item [(iii)] for every $\edge\in\EdgeTilde$,
if $\connectmapping(\edge,\confige) \not=\nullsymbol$,
then 
\begin{align*}
\distance(\edge_\confige, \connectmapping(\edge,\confige))
\leq 
    \greedycounter(\edge)
\end{align*}
\end{enumerate}
\end{lemma}
\begin{proof}
We first show property~(i). By definition of $\permu(\cdot)$,
if $\permu(\edge) < \permu(\edge')$, 
$\connectmapping(\edge,\confige) \not=\nullsymbol$.
% By definition,
At time stamp $\permu(\edge)$,
facility~$\connectmapping(\edge,\confige)$ has been opened, and 
edge $\edge'$ has not been connected through its home/work location
$\edge'_{\config(\edge')}$ yet.
This implies that
$\discountfactor \cdot \greedycounter(\edge') < 
\distance(\edge'_{\config(\edge')}, \connectmapping(\edge,\confige))$.
Otherwise, edge $\edge'$ should be connected to
facility~$\connectmapping(\edge,\confige)$ through 
its home/work location
$\edge'_{\config(\edge')}$ weakly before time stamp $\permu(\edge)$, which
is a contradiction.
Therefore,
\begin{align*}
    \discountfactor \cdot \greedycounter(\edge') 
    < 
\distance(\edge'_{\config(\edge')}, \connectmapping(\edge,\confige))
\overset{}{\leq}
\distance(\edge_\confige, \connectmapping(\edge,\confige))
+
\distance(\edge_\confige, i)
+
\distance(\edge'_{\config(\edge')}, i)
\end{align*}
where the second inequality holds due to the triangle inequality.

Next we prove property~(ii) by contradiction. 
Suppose there exists an edge $\edge\in\EdgeTilde$
such that 
\begin{align*}
    \sum_{\edge'\in\EdgeTilde:\permu(\edge') \geq \permu(\edge)}
    \plus{
    \discountfactor\cdot 
    \min\left\{
    \greedycounter(\edge),
    \greedycounter(\edge')
    \right\}
    -
    \distance(\edge'_{\config(\edge')}, i)
    }
    >
    \opencost_i
\end{align*}
Now consider the algorithm at time stamp $\timeindex \triangleq \permu(\edge) - \epsilon$ for sufficiently small $\epsilon$.
By definition, none of edges $\edge'\in\Edge$ 
with 
$\permu(\edge')\geq \permu(\edge)$
has been connected to any facility through its 
home/work location $\edge'_{\config(\edge')}$.
In a slight abuse of notation, 
let $\greedycounter_{\timeindex}(\edge')$
be the value of variable $\greedycounter(\edge')$
in the algorithm at time stamp $t$.
By construction, we know that 
$\greedycounter_{\timeindex}(\edge')
\geq \min\{\timeindex,\greedycounter(\edge')\}$,
and $\timeindex \geq \greedycounter(\edge)$.
Thus, we claim that facility $i$ is opened 
weakly before time stamp $\timeindex$, 
since
the condition of opening facility $i$
is satisfied at time stamp $\timeindex$.
Moreover, there exists at least an edge $\edge'\in\Edge$ 
such that  
$\permu(\edge')\geq \timeindex$
and $\discountfactor\cdot  
\greedycounter_{\timeindex}(\edge') \geq \distance(\edge'_{\config(\edge')}, i)$.
This implies that edge $\edge'$ 
is connected to facility $i$ 
through its $\edge'_{\config(\edge')}$ 
weakly before time stamp $\timeindex$,
which is a contradiction.

Finally, property~(iii) is guaranteed by the construction of the algorithm,
and the assumption that $\discountfactor \in[0, 1]$.
\end{proof}

Putting all pieces together, we are ready to prove \Cref{lem:weakly factor-revealing program}.
\begin{proof}[Proof of \Cref{lem:weakly factor-revealing program}]
Consider linear program~\ref{eq:lp relaxtion}.
Invoking \Cref{lem:lp relaxation}, \Cref{lem:dual assignment objective value}
\Cref{lem:dual assignment approx feasible},
and duality of linear programming finishes the proof.
\end{proof}

% \paragraph{Structural lemma of the JMMSV algorithm in the MFLP.}

% \begin{remark}
In the MFLP, \citet{JMMSV-02} also identify a 
structural lemma with similar properties~(i) and (ii)
for the JMMSV algorithm (a.k.a., 2-Chance Greedy Algorithm with discount factor $\discountfactor = 0$).
The main difference, which becomes 
a new significant technical challenge  in our setting,
is the \emph{misalignment between 
$\greedycounter(\edge)$ and
$\permu(\edgetoellmappingconfig(\edge))$}.
Specifically, 
when we implement the 2-Chance Greedy Algorithm
with strictly positive discount factor $\discountfactor \in (0, 1]$ in the \TWOLFLP,
each edge $\edge$ may be connected to two facilities,
and thus $\greedycounter(\edge)$
is not monotone with respect to the total preorder
specified by 
$\permu(\edgetoellmappingconfig(\edge))$.
Due to the non-monotonicity of $\greedycounter(\edge)$,
the property~(ii) in the structural lemma and
constraint \WFRCcontribution\ in the factor-revealing program~\ref{eq:weakly factor-revealing program}
include
a non-linear term $\min\{\muHat(\ell), \muHat(\ell')\}$.
Consequently, program~\ref{eq:weakly factor-revealing program}
becomes harder to analyze.
We side step this difficulty
through a major technical contribution of~\Cref{sec:strongly factor-revealing program},
which allows us to obtain a
 strongly factor-revealing quadratic  program~\ref{eq:strongly factor-revealing quadratic program} that can be both analytically analyzed and numerically computed.
By contrast, 
the JMMSV algorithm
only connects each edge to a single facility,
and thus $\greedycounter(\edge) \equiv
\permu(\edgetoellmappingconfig(\edge))$.
Therefore, the monotonicity of $\greedycounter(\edge)$
with respect to $\permu(\edgetoellmappingconfig(\edge))$
is guaranteed, and the non-linear term 
$\min\{\muHat(\ell), \muHat(\ell')\}$ simply becomes the linear term $\muHat(\ell)$.
Consequently, 
both relatively simple analytical analysis and numerically-aided
analysis are possible.
% \begin{lemma}[adopted from \citealp{JMMSV-02}]
% Given any MFLP instance, and any star $\starinstance$, for the 2-Chance Greedy
% Algorithm with discount factor and any star $\starinstance 
% = (i, \EdgeTilde, \config)\in\starspace$,
% for the 2-Chance Greedy Algorithm with discount factor $\discountfactor\in
% [0, 1]$,
% \end{lemma}

It is also worth mentioning the \emph{degeneracy of 
property~(i)} for 2-Chance Greedy Algorithm
with discount factor~$\discountfactor = 0$.
Namely, in this case, 
property~(i) is trivially satisfied since 
its left-hand side becomes zero.
The proof of property~(i) mainly utilizes
the fact that distance function $\distance$
satisfies the triangle inequality 
over all locations.
However,
as we discussed at the end of \Cref{sec:greedy two location},
 the \TWOLFLP~  algorithm with discount factor~$\discountfactor = 0$,
essentially treats each edge as a new location, resulting in distances 
 between the new locations and facilities that no longer satisfy the triangle inequality.
Nonetheless, this degeneracy of 
property~(i) can be overcome in the MFLP.
Recall that
the JMMSV algorithm
is equivalent to the 2-Chance Greedy Algorithm
with an arbitrary discount factor~$\discountfactor \in[0, 1]$
(\Cref{ob:JMMSV equivalence MFLP}) in the MFLP.
This enables us to consider
the factor-revealing program~\ref{eq:weakly factor-revealing program}
with $\discountfactor = 1$,
which 
recovers the factor-revealing program from \citet{JMMSV-02}
and
guarantees
the $\greedyapproxMFLP$-approximation  
the JMMSV algorithm in the MFLP.
% \end{remark}

